SERENADE: A Parallel Randomized Algorithm Suite for Crossbar Scheduling in Input-Queued Switches

Most of today's high-speed switches and routers adopt an input-queued crossbar switch architecture. Such a switch needs to compute a matching (crossbar schedule) between the input ports and output ports during each switching cycle (time slot). A key research challenge in designing large (in number of input/output ports $N$) input-queued crossbar switches is to develop crossbar scheduling algorithms that can compute "high quality" matchings -- i.e., those that result in high switch throughput (ideally $100\%$) and low queueing delays for packets -- at line rates. SERENA is one such algorithm: it outputs excellent matching decisions that result in $100\%$ switch throughput and reasonably good queueing delays. However, since SERENA is a centralized algorithm with $O(N)$ computational complexity, it cannot support switches that both are large and have a very high line rate per port. In this work, we propose SERENADE (SERENA, the Distributed Edition), a parallel iterative algorithm that emulates SERENA in only $O(\log N)$ iterations between input ports and output ports, and hence has a time complexity of only $O(\log N)$ per port. We prove that SERENADE can exactly emulate SERENA. We also propose an early-stop version of SERENADE, called O-SERENADE, to only approximately emulate SERENA. Through extensive simulations, we show that O-SERENADE can achieve 100\% throughput and that it has similar as or slightly better delay performance than SERENA under various load conditions and traffic patterns.

==> figures/bs-v1/bs-analogy.tex <==
\begin{tikzpicture}[
hlist/.style={
    very thin,
    rectangle split,
    rectangle split parts=11, draw, % change from 9 to 7, removing the nodes before head & after tail
    rectangle split horizontal, 
    minimum height= 0.6cm,
    % minimum width = 1.6em,
    % minimum text width = 1.5 em,
    text centered,
    inner sep=5pt, 
    text=black, 
    rectangle split part align={north}
}]

\node[draw, circle,inner sep=0.1cm, label=below:{$\mathcal{L}$}] (Leader) at (0,0) {};
\node[draw, circle,inner sep=0.1cm, label=below:{$\sigma^{(2^{k_0-1})}(\mathcal{L})$}] (Leader1) at (3cm,0) {};
\node[draw, circle,inner sep=0.1cm, label=below:{$\sigma^{2^{k_0}}(\mathcal{L})$}] (Leader2) at (6cm,0) {};



\draw[->,->=latex] (Leader) -- (Leader1);
\draw[->,->=latex] (Leader1) -- (Leader2);

\node[draw=red, fill=white, circle,inner sep=0.08cm, label=above:{$\mathcal{L}$}, dotted, thick] (Lea) at (4.1cm,0) {};

% %% draw array
\node [hlist,above=1cm of Leader.north, anchor=west](array)
{ 
  \nodepart{one} / 
  \nodepart{two}$0$  
  \nodepart{three} $0$  
  \nodepart{four}$\cdots$ 
  \nodepart{five} $0$  
  \nodepart{six} {\color{red}$\mathbf{1}$}
  \nodepart{seven} $1$
  \nodepart{eight} $1$
  \nodepart{nine} $\cdots$
  \nodepart{ten} $1$
  \nodepart{eleven} /
};

\draw[dashed,->] (Leader1) -- (array.one south);
\draw[dashed,->] (Lea) -- (array.six south);
\draw[dashed,->] (Leader2) -- (array.eleven south);

\end{tikzpicture}

==> figures/bs-v1/bs-illus-v1.tex <==
\subfigure[View of a cycle]{
\input{figures/bs-v1/cycle-demo}
\label{subfig: cycle-demo}
}
\subfigure[Analogy to an ordered array]{
\input{figures/bs-v1/bs-analogy}
\label{subfig: bs-analogy}
}

==> figures/bs-v1/cycle-demo.tex <==
\begin{tikzpicture}

\def \n {3}
\def \radius {2cm}
\def \Radius {2.25cm}
\def \RRadius {2.4cm}
\def \RRRadius {3cm}
\def \margin {5} % margin in angles, depends on the radius



\node[draw, circle,label={[label distance=0.01cm]-90:$\mathcal{L}$}] (Leader0) at ({90}:\radius) {};

\node[draw, circle,label={[label distance=0.01cm]60:$\sigma^{(2^{k_0-1})}(\mathcal{L})$}] (Leader1) at ({-130}:\radius) {};

\node[draw, circle,label={[label distance=0.01cm]220:$\sigma^{2^{k_0}}(\mathcal{L})$}] (Leader2) at ({-350}:\radius) {};

\draw[->, >=latex] ({-270 - \margin}:\radius) arc ({-270 - \margin}:{-350 + \margin}:\radius);
\draw[->, >=latex] ({-350 - \margin}:\radius) arc ({-350 - \margin}:{-490 + \margin}:\radius);    
\draw[->, >=latex] ({-490 - \margin}:\radius) arc ({-490 - \margin}:{-630 + \margin}:\radius); 


\node[draw=none,fill=none,inner sep=0] (Leader0Above) at ({90}:\Radius) {};
\node[draw=none,fill=none,inner sep=0] (Leader1Above) at ({-130}:\Radius) {};


% \draw (Leader0) -- (Leader0Above);
% \draw (Leader1) -- (Leader1Above);

\draw[->, >=latex, dotted, thick] (Leader0Above) arc ({-270}:{-490}:\Radius);


\node[draw=none,fill=none,inner sep=0] (Leader0AAbove) at ({90}:\RRadius) {};
\node[draw=none,fill=none,inner sep=0] (Leader2Above) at ({-350}:\RRRadius) {};

% \bonusspiral[black](0,0)(90:10)({\RRadius}:{\RRRadius})[2];

\draw[domain={0}:{7.68},variable=\t,samples=440,smooth,->, >=latex, dashed, thick]
        plot({(-\t+1.5708) r}:{\RRadius + \t/1.2 + 1.1*\t/(0.1+\t)});
        
% \draw [domain=90:-33, variable=\t, smooth, samples=75, ->] plot ({\t r}: {0.008*\t*\t});

% \foreach \s in {1,...,\n}
% {
% %   \node[draw, circle,label={[label distance=0.08cm]30:label}] ({\s}) at ({360/\n * (\s - 1) - 30 }:\radius) {};
%   \draw[->, >=latex] ({360/\n * (\s) - 30 - \margin}:\radius) 
%     arc ({360/\n * (\s) - 30 -\margin}:{360/\n * (\s - 1) - 30 + \margin}:\radius);
% }



% \node[draw=none] (LeaderAbove) at ({120 * (- 1) - 30 }:\Radius) {};
% \node[draw=none] (LeaderDownO) at ({120 * (- 1) - 30 }:\Radius) {};

% \draw[->, >=latex] ({90}:\Radius) arc ({90}:{-150}:\Radius);
    
% \bonusspiral[black](0,0)(180:270)(-1:-5)[2];
\end{tikzpicture}

==> figures/bs-v2/bs-illus-v2.tex <==
\begin{tikzpicture}[
vertex/.style={circle, draw, inner sep=2pt}]

\def \margin{2pt}

\node[vertex,label=below:$\mathcal{L}$] (v0) at (0,0) {};
\node[vertex,label=below:$\sigma^{N}(\mathcal{L})$] (v1) at (8.0cm,0) {};


\node[vertex,label=below:$\sigma^{N/2}(\mathcal{L})$] (v2) at (4.0cm,0) {};

\draw[->,->=latex,dashed, thick] (v1.north) arc (0:180:2.0cm);

\node[vertex,label=below:$\sigma^{3N/4}(\mathcal{L})$] (v3) at (6.0cm,0) {};

\draw[->,->=latex,thick] (v1.north) arc (0:180:1.0cm);

\node[vertex] (v4) at (5.0cm,0) {};

\draw[->,->=latex,thick] (v3.north) arc (0:180:0.5cm);

\node[vertex,fill=red] (v5) at (4.5cm,0) {};
\draw[->,->=latex,thick] (v4.north) arc (0:180:0.25cm);

\draw[thick] (v0) -- (v2) -- (v5) -- (v4) -- (v3) -- (v1);

\end{tikzpicture}

==> figures/merge-elaboration/cycle-graphs-h.tex <==
\subfigure[Cycles in $S_r\bigcup S_g$]{
\input{figures/merge-elaboration/sigma-new-small-h}
\label{subfig: cycle-io}
}
% \hspace{0.5em}
\subfigure[{\it I}-to-{\it I} cycles (cycles in $\sigma=\sigma_g^{-1}\circ\sigma_r$)]{
\input{figures/merge-elaboration/sigma-ii-new-small-h}
\label{subfig: cycle-ii}
}

==> figures/merge-elaboration/cycle-graphs.tex <==
\subfigure[Original]{
\input{figures/merge-elaboration/sigma-new-small}
\label{subfig: cycle-io}
}
% \hspace{0.5em}
\subfigure[{\it I}-to-{\it I}]{
\input{figures/merge-elaboration/sigma-ii-new-small}
\label{subfig: cycle-ii}
}

==> figures/merge-elaboration/merge-demo-new-small-v2.tex <==
\subfigure[$\sigma_r$]{
\input{figures/merge-elaboration/sigma-1-small-v2}
\label{subfig: sigma-1}
}
%
\subfigure[$\sigma^{-1}_g$]{
\input{figures/merge-elaboration/sigma-2-small-v2}
\label{subfig: sigma-2}
}
%
\subfigure[$S_1 \cup S_2$]{
\input{figures/merge-elaboration/union-graph}
\label{subfig: union}
}

==> figures/merge-elaboration/merge-demo-new-small.tex <==

% \subfigure[$\sigma_r$]{
\subfigure[Red matching]{
\input{figures/merge-elaboration/sigma-1-small}
\label{subfig: sigma-1}
}
\hspace{1.2em}
% \subfigure[$\sigma^{-1}_g$]{
\subfigure[Green matching]{
\input{figures/merge-elaboration/sigma-2-small}
\label{subfig: sigma-2}
}
% \hspace{-0.9em}
% \subfigure[$\sigma$]{
% \input{figures/merge-elaboration/sigma-new-small}
% \label{subfig: sigma}
% }
% \end{figure}

% \end{document}


==> figures/v2/cycle-ww.tex <==
\begin{tikzpicture}
\def \n {6}
\def \radius {0.65cm}
\def \margin {19} % margin in angles, depends on the radius
\def \cmargin {0.4cm}
\def \labeldist {-2pt}
\def \minsize {5mm}
\def \innersep {0pt}
\def \myrotate {45}
\def \myyshift {0}

\renewcommand{\n}{6}
\renewcommand{\myrotate}{0}
\newcommand{\Radius}{1.1cm}
\renewcommand{\margin} {14}

\tikzstyle{vertex}=[draw, fill=none, circle,inner sep=
{\innersep}, minimum
size={\minsize}]
% {rgb:green,1;red,1}
\tikzstyle{IO}=[->, >=latex,draw=black]
% {rgb:green,1;red,1}
\tikzstyle{OI}=[->, >=latex,draw=black]
\tikzstyle{dummyvertex}=[draw=none,fill=none]
% {rgb:green,1;red,1}
\tikzstyle{NIO}=[draw=black]

\foreach \s/\i/\p/\w in {6/3/above/1,5/8/above/1,4/4/below/6,3/6/below/3,2/7/above/1,1/1/below/3}
{
  \pgfmathparse{int(mod(\s,2))}

  \ifthenelse{0 = \pgfmathresult}
  {\draw[OI] ({360/\n * (\s + 1) - \myrotate - \margin}:\Radius) 
    arc ({360/\n * (\s + 1) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate +
    \margin}:\Radius) node[midway,\p, sloped]{$w_g\,=\,\w$}} 
  {\draw[NIO] ({360/\n * (\s) - \myrotate - \margin}:\Radius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 2) - \myrotate + \margin}:\Radius) node[midway,\p,sloped]{$w_r\,=\,\w$}}
  ;%% cannot remove

  \ifthenelse{0 = \pgfmathresult}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\Radius) {$\i$};}
      {}
}

% \renewcommand{\n}{3}
% \foreach \s/\i/\p/\w in {6/3/below/1,5/8/below/1,4/4/below/6,3/6/above/3,2/7/above/1,1/1/above/3}
% {
%   \pgfmathparse{int(mod(\s,2))}

%   \ifthenelse{\s > 3}
%   {\draw[OI] ({360/\n * (\s - 3) - \myrotate}:\Radius) 
%     arc ({360/\n * (\s - 3) - \myrotate }:{360/\n * (\s - 4) - \myrotate +
%     \margin}:\Radius) node[midway,\p, sloped]{$w_g\,=\,\w$};}
%   {} 
%   % {\draw[NIO] ({360/\n * (\s) - \myrotate - \margin}:\Radius) 
%   %   arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate }:\Radius) node[midway,\p,sloped]{$w_r\,=\,\w$}}
%   % ;%% cannot remove

%   \ifthenelse{0 = \pgfmathresult}
%       {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\Radius) {$\i$};}
%       {}
% }

\end{tikzpicture}

==> figures/v2/cycles-in-union.tex <==
\begin{tikzpicture}[scale=0.9]
\def \n {4}
\def \radius {0.65cm}
\def \margin {20} % margin in angles, depends on the radius
\def \cmargin {0.4cm}
\def \labeldist {-2pt}
\def \minsize {5mm}
\def \innersep {0pt}
\def \myrotate {45}
\def \myyshift {0}
% {rgb:black,1;white,3}
\tikzstyle{vertex}=[draw, fill=none, circle,inner sep=
{\innersep}, minimum
size={\minsize}]
% ,red
\tikzstyle{IO}=[->, >=latex, draw=black]
% ,green
\tikzstyle{OI}=[->, >=latex, draw=black]


% \begin{scope}[shift={(0,1.3cm)}]
% \node[draw=none] at (0,0) {\Large \textbf{I}-to-\textbf{I}};
% \end{scope}
%% cycle 1
\begin{scope}
\foreach \s/\i in {4/1,3/4,2/5,1/3}
{
  \pgfmathparse{int(mod(\s,2))}

  \ifthenelse{0 = \pgfmathresult}
  {\draw[OI] ({360/\n * (\s) - \myrotate - \margin}:\radius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate +
    \margin}:\radius)} 
  {\draw[IO] ({360/\n * (\s) - \myrotate - \margin}:\radius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate +
    \margin}:\radius)}
  ;%% cannot remove

  \ifthenelse{0 = \pgfmathresult}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\radius) {$I_\i$}}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\radius) {$O_\i$}}
  ;%% cannot remove
}
\end{scope}

%% cycle 2
\renewcommand{\n}{4}

\begin{scope}[shift={({2 * (\radius) + (\cmargin)},0)}]
\foreach \s/\i in {4/2,3/5,2/6,1/7}
{
  \pgfmathparse{int(mod(\s,2))}

  \ifthenelse{0 = \pgfmathresult}
  {\draw[OI] ({360/\n * (\s) - \myrotate - \margin}:\radius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate +
    \margin}:\radius)} 
  {\draw[IO] ({360/\n * (\s) - \myrotate - \margin}:\radius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate +
    \margin}:\radius)}
  ;%% cannot remove

  \ifthenelse{0 = \pgfmathresult}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\radius) {$I_\i$}}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\radius) {$O_\i$}}
  ;%% cannot remove
}
\end{scope}

%% cycle 3
\renewcommand{\n}{6}
\newcommand{\Radius}{1.2cm}
\renewcommand{\margin} {12}
\begin{scope}[shift={({4 * (\radius)  + 4 * (\cmargin)}, 0)}]
\foreach \s/\i in {6/3,5/8,4/4,3/6,2/7,1/1}
{
  \pgfmathparse{int(mod(\s,2))}

  \ifthenelse{0 = \pgfmathresult}
  {\draw[OI] ({360/\n * (\s) - \myrotate - \margin}:\Radius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate +
    \margin}:\Radius)} 
  {\draw[IO] ({360/\n * (\s) - \myrotate - \margin}:\Radius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate +
    \margin}:\Radius)}
  ;%% cannot remove

  \ifthenelse{0 = \pgfmathresult}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\Radius) {$I_\i$}}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\Radius) {$O_\i$}}
  ;%% cannot remove
}
\end{scope}

\renewcommand{\n}{2}
\newcommand{\rradius}{0.4cm}
\renewcommand{\margin}{34}
\renewcommand{\myrotate}{90}

\begin{scope}[shift={({4 * (\radius) + 2 * (\Radius) + 4 * (\cmargin)}, 0)}]
\foreach \s/\i in {2/8,1/2}
{
  \pgfmathparse{int(mod(\s,2))}

  \ifthenelse{0 = \pgfmathresult}
  {\draw[OI] ({360/\n * (\s) - \myrotate - \margin}:\rradius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate +
    \margin}:\rradius)} 
  {\draw[IO] ({360/\n * (\s) - \myrotate - \margin}:\rradius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate +
    \margin}:\rradius)}
  ;%% cannot remove

  \ifthenelse{0 = \pgfmathresult}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\rradius) {$I_\i$}}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\rradius) {$O_\i$}}
  ;%% cannot remove
}
\end{scope}

\end{tikzpicture}

==> figures/v2/permutation-cycles.tex <==
\begin{tikzpicture}[scale=0.9]
\def \n {4}
\def \radius {0.65cm}
\def \margin {20} % margin in angles, depends on the radius
\def \cmargin {0.4cm}
\def \labeldist {-2pt}
\def \minsize {5mm}
\def \innersep {0pt}
\def \myrotate {45}
\def \myyshift {0}

% {rgb:black,1;white,3}
\tikzstyle{vertex}=[draw, fill=none, circle,inner sep=
{\innersep}, minimum
size={\minsize}]
% {rgb:green,1;red,1}
\tikzstyle{IO}=[->, >=latex,draw=black]
% {rgb:green,1;red,1}
\tikzstyle{OI}=[->, >=latex,draw=black]
\tikzstyle{dummyvertex}=[draw=none,fill=none]
% {rgb:green,1;red,1}
\tikzstyle{NIO}=[draw=black]
% \begin{scope}[shift={(0,1.3cm)}]
% \node[draw=none] at (0,0) {\Large \textbf{I}-to-\textbf{I}};
% \end{scope}
%% cycle 1
\begin{scope}
\foreach \s/\i in {4/1,3/4,2/5,1/3}
{
  \pgfmathparse{int(mod(\s,2))}

  \ifthenelse{0 = \pgfmathresult}
  {\draw[OI] ({360/\n * (\s) - \myrotate }:\radius) 
    arc ({360/\n * (\s) - \myrotate }:{360/\n * (\s - 1) - \myrotate +
    \margin}:\radius)} 
  {\draw[NIO] ({360/\n * (\s) - \myrotate - \margin}:\radius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate }:\radius)}
  ;%% cannot remove

  \ifthenelse{0 = \pgfmathresult}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\radius) {$\i$};}
      {}

}
\end{scope}

%% cycle 2
\renewcommand{\n}{4}

\begin{scope}[shift={({2 * (\radius) + (\cmargin)},0)}]
\foreach \s/\i in {4/2,3/5,2/6,1/7}
{
  \pgfmathparse{int(mod(\s,2))}

  \ifthenelse{0 = \pgfmathresult}
  {\draw[OI] ({360/\n * (\s) - \myrotate}:\radius) 
    arc ({360/\n * (\s) - \myrotate }:{360/\n * (\s - 1) - \myrotate +
    \margin}:\radius)} 
  {\draw[NIO] ({360/\n * (\s) - \myrotate - \margin}:\radius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate }:\radius)}
  ;%% cannot remove

  \ifthenelse{0 = \pgfmathresult}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\radius) {$\i$};}
      {}
}
\end{scope}

%% cycle 3
\renewcommand{\n}{6}
\renewcommand{\myrotate}{0}
\newcommand{\Radius}{1.2cm}
\renewcommand{\margin} {12}
\begin{scope}[shift={({4 * (\radius) + 4 * (\cmargin)},0)}]
\foreach \s/\i in {6/3,5/8,4/4,3/6,2/7,1/1}
{
  \pgfmathparse{int(mod(\s,2))}

  \ifthenelse{0 = \pgfmathresult}
  {\draw[OI] ({360/\n * (\s) - \myrotate}:\Radius) 
    arc ({360/\n * (\s) - \myrotate }:{360/\n * (\s - 1) - \myrotate +
    \margin}:\Radius)} 
  {\draw[NIO] ({360/\n * (\s) - \myrotate - \margin}:\Radius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate }:\Radius)}
  ;%% cannot remove

  \ifthenelse{0 = \pgfmathresult}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\Radius) {$\i$};}
      {}
}
\end{scope}

\renewcommand{\n}{2}
\newcommand{\rradius}{0.4cm}
\renewcommand{\margin}{34}
\renewcommand{\myrotate}{90}

\begin{scope}[shift={({4 * (\radius) + 2 * (\Radius) + 4 * (\cmargin)},0)}]
\foreach \s/\i in {2/8,1/2}
{
  \pgfmathparse{int(mod(\s,2))}

  \ifthenelse{0 = \pgfmathresult}
  {\draw[OI] ({360/\n * (\s) - \myrotate}:\rradius) 
    arc ({360/\n * (\s) - \myrotate}:{360/\n * (\s - 1) - \myrotate +
    \margin}:\rradius)} 
  {\draw[NIO] ({360/\n * (\s) - \myrotate - \margin}:\rradius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate }:\rradius)}
  ;%% cannot remove

  \ifthenelse{0 = \pgfmathresult}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\rradius) {$\i$};}
      {}
}
\end{scope}

\end{tikzpicture}

==> figures/v2/two-full-matchings.tex <==
% \subfigure[$\sigma_r$]{
\subfigure[$S_r(I\rightarrow O)$]{
\input{figures/merge-elaboration/sigma-1-small}
\label{subfig: sigma-1}
}
\hspace{1.2em}
% \subfigure[$\sigma^{-1}_g$]{
\subfigure[$S_g(O\rightarrow I)$]{
\input{figures/merge-elaboration/sigma-2-small}
\label{subfig: sigma-2}
}

==> libs/double_quotes_relax.tex <==
%% These two packages are included to handle 
%% double quotes issues (`` ")
\usepackage[english]{babel}
\usepackage[autostyle]{csquotes}

==> libs/font_warning_fixer.tex <==
% \usepackage{lmodern}% http://ctan.org/pkg/lm does not work
\usepackage{anyfontsize}

==> libs/macros/autoref_fixer_acmart.tex <==
\def\definitionautorefname{Definition}

==> libs/macros/highlight.tex <==
% highlight by Long
\def\glong#1{\textcolor{blue}{#1}}

==> libs/macros/utils.tex <==
%% default log
%% inspired by https://tex.stackexchange.com/questions/33381/how-to-redefine-an-existing-command-using-futurelet-scanning-for-number-and-type
%% if user provides a base then use the base, otherwise use the default base (i.e., 2)
% \usepackage{etoolbox}

% \makeatletter
% \expandafter\def\csname  logalias \endcsname
% \expandafter\def\csname  logtwo \endcsname
% \let\logalias\log
% \def\logtwo{{\qopname\relax{no}{log}}_2}
% \def\log{\@ifnextchar_ {\csname logalias\endcsname} {\csname logtwo\endcsname}}
% \makeatother

==> sections/figures/bs-v1/bs-analogy.tex <==
\begin{tikzpicture}[
hlist/.style={
    very thin,
    rectangle split,
    rectangle split parts=11, draw, % change from 9 to 7, removing the nodes before head & after tail
    rectangle split horizontal, 
    minimum height= 0.6cm,
    % minimum width = 1.6em,
    % minimum text width = 1.5 em,
    text centered,
    inner sep=5pt, 
    text=black, 
    rectangle split part align={north}
}]

\node[draw, circle,inner sep=0.1cm, label=below:{$\mathcal{L}$}] (Leader) at (0,0) {};
\node[draw, circle,inner sep=0.1cm, label=below:{$\sigma^{(2^{k_0-1})}(\mathcal{L})$}] (Leader1) at (3cm,0) {};
\node[draw, circle,inner sep=0.1cm, label=below:{$\sigma^{2^{k_0}}(\mathcal{L})$}] (Leader2) at (6cm,0) {};



\draw[->,->=latex] (Leader) -- (Leader1);
\draw[->,->=latex] (Leader1) -- (Leader2);

\node[draw=red, fill=white, circle,inner sep=0.08cm, label=above:{$\mathcal{L}$}, dotted, thick] (Lea) at (4.1cm,0) {};

% %% draw array
\node [hlist,above=1cm of Leader.north, anchor=west](array)
{ 
  \nodepart{one} / 
  \nodepart{two}$0$  
  \nodepart{three} $0$  
  \nodepart{four}$\cdots$ 
  \nodepart{five} $0$  
  \nodepart{six} {\color{red}$\mathbf{1}$}
  \nodepart{seven} $1$
  \nodepart{eight} $1$
  \nodepart{nine} $\cdots$
  \nodepart{ten} $1$
  \nodepart{eleven} /
};

\draw[dashed,->] (Leader1) -- (array.one south);
\draw[dashed,->] (Lea) -- (array.six south);
\draw[dashed,->] (Leader2) -- (array.eleven south);

\end{tikzpicture}

==> sections/figures/bs-v1/bs-illus-v1.tex <==
\subfigure[View of a cycle]{
\input{figures/bs-v1/cycle-demo}
\label{subfig: cycle-demo}
}
\subfigure[Analogy to an ordered array]{
\input{figures/bs-v1/bs-analogy}
\label{subfig: bs-analogy}
}

==> sections/figures/bs-v1/cycle-demo.tex <==
\begin{tikzpicture}

\def \n {3}
\def \radius {2cm}
\def \Radius {2.25cm}
\def \RRadius {2.4cm}
\def \RRRadius {3cm}
\def \margin {5} % margin in angles, depends on the radius



\node[draw, circle,label={[label distance=0.01cm]-90:$\mathcal{L}$}] (Leader0) at ({90}:\radius) {};

\node[draw, circle,label={[label distance=0.01cm]60:$\sigma^{(2^{k_0-1})}(\mathcal{L})$}] (Leader1) at ({-130}:\radius) {};

\node[draw, circle,label={[label distance=0.01cm]220:$\sigma^{2^{k_0}}(\mathcal{L})$}] (Leader2) at ({-350}:\radius) {};

\draw[->, >=latex] ({-270 - \margin}:\radius) arc ({-270 - \margin}:{-350 + \margin}:\radius);
\draw[->, >=latex] ({-350 - \margin}:\radius) arc ({-350 - \margin}:{-490 + \margin}:\radius);    
\draw[->, >=latex] ({-490 - \margin}:\radius) arc ({-490 - \margin}:{-630 + \margin}:\radius); 


\node[draw=none,fill=none,inner sep=0] (Leader0Above) at ({90}:\Radius) {};
\node[draw=none,fill=none,inner sep=0] (Leader1Above) at ({-130}:\Radius) {};


% \draw (Leader0) -- (Leader0Above);
% \draw (Leader1) -- (Leader1Above);

\draw[->, >=latex, dotted, thick] (Leader0Above) arc ({-270}:{-490}:\Radius);


\node[draw=none,fill=none,inner sep=0] (Leader0AAbove) at ({90}:\RRadius) {};
\node[draw=none,fill=none,inner sep=0] (Leader2Above) at ({-350}:\RRRadius) {};

% \bonusspiral[black](0,0)(90:10)({\RRadius}:{\RRRadius})[2];

\draw[domain={0}:{7.68},variable=\t,samples=440,smooth,->, >=latex, dashed, thick]
        plot({(-\t+1.5708) r}:{\RRadius + \t/1.2 + 1.1*\t/(0.1+\t)});
        
% \draw [domain=90:-33, variable=\t, smooth, samples=75, ->] plot ({\t r}: {0.008*\t*\t});

% \foreach \s in {1,...,\n}
% {
% %   \node[draw, circle,label={[label distance=0.08cm]30:label}] ({\s}) at ({360/\n * (\s - 1) - 30 }:\radius) {};
%   \draw[->, >=latex] ({360/\n * (\s) - 30 - \margin}:\radius) 
%     arc ({360/\n * (\s) - 30 -\margin}:{360/\n * (\s - 1) - 30 + \margin}:\radius);
% }



% \node[draw=none] (LeaderAbove) at ({120 * (- 1) - 30 }:\Radius) {};
% \node[draw=none] (LeaderDownO) at ({120 * (- 1) - 30 }:\Radius) {};

% \draw[->, >=latex] ({90}:\Radius) arc ({90}:{-150}:\Radius);
    
% \bonusspiral[black](0,0)(180:270)(-1:-5)[2];
\end{tikzpicture}

==> sections/figures/bs-v2/bs-illus-v2.tex <==
\begin{tikzpicture}[
vertex/.style={circle, draw, inner sep=2pt}]

\def \margin{2pt}

\node[vertex,label=below:$\mathcal{L}$] (v0) at (0,0) {};
\node[vertex,label=below:$\sigma^{N}(\mathcal{L})$] (v1) at (8.0cm,0) {};


\node[vertex,label=below:$\sigma^{N/2}(\mathcal{L})$] (v2) at (4.0cm,0) {};

\draw[->,->=latex,dashed, thick] (v1.north) arc (0:180:2.0cm);

\node[vertex,label=below:$\sigma^{3N/4}(\mathcal{L})$] (v3) at (6.0cm,0) {};

\draw[->,->=latex,thick] (v1.north) arc (0:180:1.0cm);

\node[vertex] (v4) at (5.0cm,0) {};

\draw[->,->=latex,thick] (v3.north) arc (0:180:0.5cm);

\node[vertex,fill=red] (v5) at (4.5cm,0) {};
\draw[->,->=latex,thick] (v4.north) arc (0:180:0.25cm);

\draw[thick] (v0) -- (v2) -- (v5) -- (v4) -- (v3) -- (v1);

\end{tikzpicture}

==> sections/figures/bs-v2/bs-illus-v2s1.tex <==
\begin{tikzpicture}[
vertex/.style={circle, draw, inner sep=2pt},
post/.style={->,shorten >=1pt,>=stealth',semithick}]

\def \margin{0pt}

\node[vertex,label=below:$\mathcal{L}$] (v0) at (0,0) {};
\node[vertex,label=below:$\sigma^{N}(\mathcal{L})$] (v1) at (8.0cm,0) {};


\node[vertex,label=below:$\sigma^{N/2}(\mathcal{L})$] (v2) at (4.0cm,0) {};

\draw[post,dashed, thick] (v1.north) arc (60:120:4.0cm);

\node[vertex,label=below:$\sigma^{3N/4}(\mathcal{L})$] (v3) at (6.0cm,0) {};

\draw[post,thick] (v1.north) arc (60:120:2.0cm);

\node[vertex] (v4) at (5.0cm,0) {};

\draw[post,thick] (v3.north) arc (60:120:1.0cm);

\node[vertex,fill=red] (v5) at (4.5cm,0) {};
\draw[post,thick] (v4.north) arc (60:120:0.5cm);

\draw[thick] (v0) -- (v2) -- (v5) -- (v4) -- (v3) -- (v1);

\end{tikzpicture}

==> sections/figures/merge-elaboration/cycle-graphs-h.tex <==
\subfigure[Cycles in $S_r\bigcup S_g$]{
\input{figures/merge-elaboration/sigma-new-small-h}
\label{subfig: cycle-io}
}
% \hspace{0.5em}
\subfigure[{\it I}-to-{\it I} cycles (cycles in $\sigma=\sigma_g^{-1}\circ\sigma_r$)]{
\input{figures/merge-elaboration/sigma-ii-new-small-h}
\label{subfig: cycle-ii}
}

==> sections/figures/merge-elaboration/cycle-graphs.tex <==
\subfigure[Original]{
\input{figures/merge-elaboration/sigma-new-small}
\label{subfig: cycle-io}
}
% \hspace{0.5em}
\subfigure[{\it I}-to-{\it I}]{
\input{figures/merge-elaboration/sigma-ii-new-small}
\label{subfig: cycle-ii}
}

==> sections/figures/merge-elaboration/merge-demo-new-small-v2.tex <==
\subfigure[$\sigma_r$]{
\input{figures/merge-elaboration/sigma-1-small-v2}
\label{subfig: sigma-1}
}
%
\subfigure[$\sigma^{-1}_g$]{
\input{figures/merge-elaboration/sigma-2-small-v2}
\label{subfig: sigma-2}
}
%
\subfigure[$S_1 \cup S_2$]{
\input{figures/merge-elaboration/union-graph}
\label{subfig: union}
}

==> sections/figures/merge-elaboration/merge-demo-new-small.tex <==

% \subfigure[$\sigma_r$]{
\subfigure[Red matching]{
\input{figures/merge-elaboration/sigma-1-small}
\label{subfig: sigma-1}
}
\hspace{1.2em}
% \subfigure[$\sigma^{-1}_g$]{
\subfigure[Green matching]{
\input{figures/merge-elaboration/sigma-2-small}
\label{subfig: sigma-2}
}
% \hspace{-0.9em}
% \subfigure[$\sigma$]{
% \input{figures/merge-elaboration/sigma-new-small}
% \label{subfig: sigma}
% }
% \end{figure}

% \end{document}


==> sections/figures/v2/cycle-ww.tex <==
\begin{tikzpicture}
\def \n {6}
\def \radius {0.65cm}
\def \margin {19} % margin in angles, depends on the radius
\def \cmargin {0.4cm}
\def \labeldist {-2pt}
\def \minsize {5mm}
\def \innersep {0pt}
\def \myrotate {45}
\def \myyshift {0}

\renewcommand{\n}{6}
\renewcommand{\myrotate}{0}
\newcommand{\Radius}{1.1cm}
\renewcommand{\margin} {14}

\tikzstyle{vertex}=[draw, fill=none, circle,inner sep=
{\innersep}, minimum
size={\minsize}]
% {rgb:green,1;red,1}
\tikzstyle{IO}=[->, >=latex,draw=black]
% {rgb:green,1;red,1}
\tikzstyle{OI}=[->, >=latex,draw=black]
\tikzstyle{dummyvertex}=[draw=none,fill=none]
% {rgb:green,1;red,1}
\tikzstyle{NIO}=[draw=black]

\foreach \s/\i/\p/\w in {6/3/above/1,5/8/above/1,4/4/below/6,3/6/below/3,2/7/above/1,1/1/below/3}
{
  \pgfmathparse{int(mod(\s,2))}

  \ifthenelse{0 = \pgfmathresult}
  {\draw[OI] ({360/\n * (\s + 1) - \myrotate - \margin}:\Radius) 
    arc ({360/\n * (\s + 1) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate +
    \margin}:\Radius) node[midway,\p, sloped]{$w_g\,=\,\w$}} 
  {\draw[NIO] ({360/\n * (\s) - \myrotate - \margin}:\Radius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 2) - \myrotate + \margin}:\Radius) node[midway,\p,sloped]{$w_r\,=\,\w$}}
  ;%% cannot remove

  \ifthenelse{0 = \pgfmathresult}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\Radius) {$\i$};}
      {}
}

% \renewcommand{\n}{3}
% \foreach \s/\i/\p/\w in {6/3/below/1,5/8/below/1,4/4/below/6,3/6/above/3,2/7/above/1,1/1/above/3}
% {
%   \pgfmathparse{int(mod(\s,2))}

%   \ifthenelse{\s > 3}
%   {\draw[OI] ({360/\n * (\s - 3) - \myrotate}:\Radius) 
%     arc ({360/\n * (\s - 3) - \myrotate }:{360/\n * (\s - 4) - \myrotate +
%     \margin}:\Radius) node[midway,\p, sloped]{$w_g\,=\,\w$};}
%   {} 
%   % {\draw[NIO] ({360/\n * (\s) - \myrotate - \margin}:\Radius) 
%   %   arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate }:\Radius) node[midway,\p,sloped]{$w_r\,=\,\w$}}
%   % ;%% cannot remove

%   \ifthenelse{0 = \pgfmathresult}
%       {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\Radius) {$\i$};}
%       {}
% }

\end{tikzpicture}

==> sections/figures/v2/cycles-in-union.tex <==
\begin{tikzpicture}
\def \n {4}
\def \radius {0.65cm}
\def \margin {20} % margin in angles, depends on the radius
\def \cmargin {0.4cm}
\def \labeldist {-2pt}
\def \minsize {5mm}
\def \innersep {0pt}
\def \myrotate {45}
\def \myyshift {0}
% {rgb:black,1;white,3}
\tikzstyle{vertex}=[draw, fill=none, circle,inner sep=
{\innersep}, minimum
size={\minsize}]
% ,red
\tikzstyle{IO}=[->, >=latex, draw=black]
% ,green
\tikzstyle{OI}=[->, >=latex, draw=black]


% \begin{scope}[shift={(0,1.3cm)}]
% \node[draw=none] at (0,0) {\Large \textbf{I}-to-\textbf{I}};
% \end{scope}
%% cycle 1
\begin{scope}
\foreach \s/\i in {4/1,3/4,2/5,1/3}
{
  \pgfmathparse{int(mod(\s,2))}

  \ifthenelse{0 = \pgfmathresult}
  {\draw[OI] ({360/\n * (\s) - \myrotate - \margin}:\radius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate +
    \margin}:\radius)} 
  {\draw[IO] ({360/\n * (\s) - \myrotate - \margin}:\radius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate +
    \margin}:\radius)}
  ;%% cannot remove

  \ifthenelse{0 = \pgfmathresult}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\radius) {$I_\i$}}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\radius) {$O_\i$}}
  ;%% cannot remove
}
\end{scope}

%% cycle 2
\renewcommand{\n}{4}

\begin{scope}[shift={({2 * (\radius) + (\cmargin)},0)}]
\foreach \s/\i in {4/2,3/5,2/6,1/7}
{
  \pgfmathparse{int(mod(\s,2))}

  \ifthenelse{0 = \pgfmathresult}
  {\draw[OI] ({360/\n * (\s) - \myrotate - \margin}:\radius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate +
    \margin}:\radius)} 
  {\draw[IO] ({360/\n * (\s) - \myrotate - \margin}:\radius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate +
    \margin}:\radius)}
  ;%% cannot remove

  \ifthenelse{0 = \pgfmathresult}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\radius) {$I_\i$}}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\radius) {$O_\i$}}
  ;%% cannot remove
}
\end{scope}

%% cycle 3
\renewcommand{\n}{6}
\newcommand{\Radius}{1.2cm}
\renewcommand{\margin} {12}
\begin{scope}[shift={({4 * (\radius)  + 4 * (\cmargin)}, 0)}]
\foreach \s/\i in {6/3,5/8,4/4,3/6,2/7,1/1}
{
  \pgfmathparse{int(mod(\s,2))}

  \ifthenelse{0 = \pgfmathresult}
  {\draw[OI] ({360/\n * (\s) - \myrotate - \margin}:\Radius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate +
    \margin}:\Radius)} 
  {\draw[IO] ({360/\n * (\s) - \myrotate - \margin}:\Radius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate +
    \margin}:\Radius)}
  ;%% cannot remove

  \ifthenelse{0 = \pgfmathresult}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\Radius) {$I_\i$}}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\Radius) {$O_\i$}}
  ;%% cannot remove
}
\end{scope}

\renewcommand{\n}{2}
\newcommand{\rradius}{0.4cm}
\renewcommand{\margin}{34}
\renewcommand{\myrotate}{90}

\begin{scope}[shift={({4 * (\radius) + 2 * (\Radius) + 4 * (\cmargin)}, 0)}]
\foreach \s/\i in {2/8,1/2}
{
  \pgfmathparse{int(mod(\s,2))}

  \ifthenelse{0 = \pgfmathresult}
  {\draw[OI] ({360/\n * (\s) - \myrotate - \margin}:\rradius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate +
    \margin}:\rradius)} 
  {\draw[IO] ({360/\n * (\s) - \myrotate - \margin}:\rradius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate +
    \margin}:\rradius)}
  ;%% cannot remove

  \ifthenelse{0 = \pgfmathresult}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\rradius) {$I_\i$}}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\rradius) {$O_\i$}}
  ;%% cannot remove
}
\end{scope}

\end{tikzpicture}

==> sections/figures/v2/permutation-cycles.tex <==
\begin{tikzpicture}
\def \n {4}
\def \radius {0.65cm}
\def \margin {20} % margin in angles, depends on the radius
\def \cmargin {0.4cm}
\def \labeldist {-2pt}
\def \minsize {5mm}
\def \innersep {0pt}
\def \myrotate {45}
\def \myyshift {0}

% {rgb:black,1;white,3}
\tikzstyle{vertex}=[draw, fill=none, circle,inner sep=
{\innersep}, minimum
size={\minsize}]
% {rgb:green,1;red,1}
\tikzstyle{IO}=[->, >=latex,draw=black]
% {rgb:green,1;red,1}
\tikzstyle{OI}=[->, >=latex,draw=black]
\tikzstyle{dummyvertex}=[draw=none,fill=none]
% {rgb:green,1;red,1}
\tikzstyle{NIO}=[draw=black]
% \begin{scope}[shift={(0,1.3cm)}]
% \node[draw=none] at (0,0) {\Large \textbf{I}-to-\textbf{I}};
% \end{scope}
%% cycle 1
\begin{scope}
\foreach \s/\i in {4/1,3/4,2/5,1/3}
{
  \pgfmathparse{int(mod(\s,2))}

  \ifthenelse{0 = \pgfmathresult}
  {\draw[OI] ({360/\n * (\s) - \myrotate }:\radius) 
    arc ({360/\n * (\s) - \myrotate }:{360/\n * (\s - 1) - \myrotate +
    \margin}:\radius)} 
  {\draw[NIO] ({360/\n * (\s) - \myrotate - \margin}:\radius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate }:\radius)}
  ;%% cannot remove

  \ifthenelse{0 = \pgfmathresult}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\radius) {$\i$};}
      {}

}
\end{scope}

%% cycle 2
\renewcommand{\n}{4}

\begin{scope}[shift={({2 * (\radius) + (\cmargin)},0)}]
\foreach \s/\i in {4/2,3/5,2/6,1/7}
{
  \pgfmathparse{int(mod(\s,2))}

  \ifthenelse{0 = \pgfmathresult}
  {\draw[OI] ({360/\n * (\s) - \myrotate}:\radius) 
    arc ({360/\n * (\s) - \myrotate }:{360/\n * (\s - 1) - \myrotate +
    \margin}:\radius)} 
  {\draw[NIO] ({360/\n * (\s) - \myrotate - \margin}:\radius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate }:\radius)}
  ;%% cannot remove

  \ifthenelse{0 = \pgfmathresult}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\radius) {$\i$};}
      {}
}
\end{scope}

%% cycle 3
\renewcommand{\n}{6}
\renewcommand{\myrotate}{0}
\newcommand{\Radius}{1.2cm}
\renewcommand{\margin} {12}
\begin{scope}[shift={({4 * (\radius) + 4 * (\cmargin)},0)}]
\foreach \s/\i in {6/3,5/8,4/4,3/6,2/7,1/1}
{
  \pgfmathparse{int(mod(\s,2))}

  \ifthenelse{0 = \pgfmathresult}
  {\draw[OI] ({360/\n * (\s) - \myrotate}:\Radius) 
    arc ({360/\n * (\s) - \myrotate }:{360/\n * (\s - 1) - \myrotate +
    \margin}:\Radius)} 
  {\draw[NIO] ({360/\n * (\s) - \myrotate - \margin}:\Radius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate }:\Radius)}
  ;%% cannot remove

  \ifthenelse{0 = \pgfmathresult}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\Radius) {$\i$};}
      {}
}
\end{scope}

\renewcommand{\n}{2}
\newcommand{\rradius}{0.4cm}
\renewcommand{\margin}{34}
\renewcommand{\myrotate}{90}

\begin{scope}[shift={({4 * (\radius) + 2 * (\Radius) + 4 * (\cmargin)},0)}]
\foreach \s/\i in {2/8,1/2}
{
  \pgfmathparse{int(mod(\s,2))}

  \ifthenelse{0 = \pgfmathresult}
  {\draw[OI] ({360/\n * (\s) - \myrotate}:\rradius) 
    arc ({360/\n * (\s) - \myrotate}:{360/\n * (\s - 1) - \myrotate +
    \margin}:\rradius)} 
  {\draw[NIO] ({360/\n * (\s) - \myrotate - \margin}:\rradius) 
    arc ({360/\n * (\s) - \myrotate - \margin}:{360/\n * (\s - 1) - \myrotate }:\rradius)}
  ;%% cannot remove

  \ifthenelse{0 = \pgfmathresult}
      {\node [vertex] at ({360/\n * (\s - 1) - \myrotate}:\rradius) {$\i$};}
      {}
}
\end{scope}

\end{tikzpicture}

==> sections/figures/v2/two-full-matchings.tex <==
% \subfigure[$\sigma_r$]{
\subfigure[$S_r(I\rightarrow O)$]{
\input{figures/merge-elaboration/sigma-1-small}
\label{subfig: sigma-1}
}
\hspace{1.2em}
% \subfigure[$\sigma^{-1}_g$]{
\subfigure[$S_g(O\rightarrow I)$]{
\input{figures/merge-elaboration/sigma-2-small}
\label{subfig: sigma-2}
}

==> sections/schemes_new.tex <==
%% serenade_schemes.tex
%%
\section{SERENADE}
\label{sec: serenade}

In this section, we describe SERENADE, a parallel iterative algorithm for exactly emulating SERENA.  
SERENADE is consisted of two stages: the knowledge-discovery stage and the binary search stage. 
First, we will present the details of the knowledge-discovery stage, which consists of $1\!+\!\log_2N$ iterations of 
the knowledge-discovery procedure. Then, we will show why the $1\!+\!\log_2N$ iterations is selected and motivate 
the necessity of the binary search stage. 
After that, we will detail the binary search stage. Finally, we 
prove that SERENADE can emulate SERENA exactly. 


\begin{theorem}[Exact Emulation]
The SERENADE can exactly emulate SERENA~\cite{GiacconePrabhakarShah2003SerenaJSAC} with 
$O(\log_2 N)$ iterations, more precisely, at most $1\!+\!\log_2N$ iterations of the knowledge-discovery 
procedure and $\log_2 N$ iterations of the distributed binary search.
\end{theorem}

\RestyleAlgo{ruled}

\begin{algorithm}[t]

\caption{SERENADE.}\label{alg:serenade}

\SetKwFor{ParFor}{parfor}{do}{endparfor}

% \SetNlSty{texttt}{(}{)}
% \SetAlgoNlRelativeSize{0}
% \SetNlSkip{2pt}

\Indm \nonl {\bf The Knowledge-Discovery Stage:}

\Indp \nonl {\it IN PARALLEL} vertex $i$ runs the knowledge-discovery procedure for up to $1\!+\!\log_2 N$ iterations\;

\Indm \nonl {\bf The Distributed Binary Search Stage:}

\Indp \nonl (1) {\it IN PARALLEL} vertex $i$ checks its identity, if it is:
    \begin{itemize}
         \item the leader of a non-ouroboros cycle, then notify the switch controller by registering its identity\; 
         \item the initial search administrator of a non-ouroboros cycle, then start a distributed binary search\;
    \end{itemize}

\nonl (2) The switch controller broadcast the decisions of registered vertices to all the $N$ vertices\;

\end{algorithm}
\RestyleAlgo{boxed}

\subsection{The Knowledge-Discovery Stage}\label{subsec:knowledge-discovery}

As mentioned above, SERENADE starts with a knowledge-discovery stage that consists of $1 \!+\! \log_2 N$ 
iterations. For ease of presentation (\textit{e.g.,} no need to put floors or ceilings around each 
occurrence of $\log_2 N$), we have assumed that $N$
is a power of $2$ throughout this paper;  SERENADE works just as well when $N$ is not. 

The knowledge-discovery stage uses the standard technique of two-directional exploration with
successively doubled distance in distributed computing~\cite{Lynch1996Distributed}, the communication pattern of 
which is very similar to that of the dissemination algorithm~\cite{Hensgen1988Dissemination}. 
The basic idea of the algorithm is for each vertex $i$ to exchange information, 
with vertices ``$(\pm 2^{k-1})$ $\sigma$-hops" away (\ie $\sigma^{2^{k-1}}(i)$ and $\sigma^{-(2^{k-1})}(i)$) 
in the $k^{th}$ iteration.   
In the example shown in~\autoref{fig: comb-cycles}, vertex $3$ communicates with 
vertices $4\!=\!\sigma(3)$ and $12\!=\!\sigma^{-1}(3)$ in the $1^{st}$ iteration,
with vertices $14\!=\!\sigma^{2}(3)$ and $10\!=\!\sigma^{-2}(3)$ in the $2^{nd}$ 
iterations, with vertices $11=\sigma^{4}(3)$ and $5\!=\!\sigma^{-4}(3)$ in the $3^{nd}$ 
iteration, and with vertices $16\!=\!\sigma^{8}(3)$ and $7\!=\!\sigma^{-8}(3)$ 
in the $4^{th}$ iteration.


\subsubsection{Knowledge Sets}\label{subsubsec:knowledge-sets}

We will show next that, for $k = 0, 1, 2, \cdots, \log_2 N$ (there is a $0^{th}$ iteration at the beginning), after the $k^{th}$ iteration, each vertex $i$ learns the following two 
knowledge sets:  $\phi^{(i)}_{k+}$ and $\phi^{(i)}_{k-}$.
Knowledge set $\phi^{(i)}_{k+}$ contains three quantities concerning the 
vertex (input port)
that is $2^k$ $\sigma$-hops ``downstream"
({\it w.r.t.} the ``direction'' of $\sigma$), relative to vertex $i$, in the cycle decomposition graph of $\sigma$:
\begin{spenumerate}
    \item $\sigma^{2^k}(i)$, the identity of that vertex,
    \item $w_r(i\leadsto\sigma^{2^k}(i))$, the red weight of the $2^k$-edge-long walk from $i$ to that 
    vertex, and
    \item $w_g(i\leadsto\sigma^{2^k}(i))$, the green weight of the walk.
\end{spenumerate}
% For notational convenience, we define the three functions: $\code{id}(\cdot)$, $\code{red\_weight}(\cdot)$ and 
% $\code{green\_weight}(\cdot)$ on the knowledge set to extract its three fields respectively. 

Similarly, knowledge set $\phi^{(i)}_{k-}$ contains the three quantities concerning the 
vertex that is $2^k$ $\sigma$-hops ``upstream" relative to vertex $i$, namely
$\sigma^{-2^k}(i)$, $w_r(\sigma^{-2^k}(i)\leadsto i)$, and $w_g(\sigma^{-2^k}(i)\leadsto i)$.  
For example, after the $3^{rd}$ iteration, vertex $3$ learns the identities of $16\!=\!\sigma^8(3)$ and $7\!=\!\sigma^{-8}(3)$ (vertices ``$(\pm 8)$ $\sigma$-hops" away) and the green and the red weights of the walks $3\!\leadsto\!\sigma^8(3)$ and $\sigma^{-8}(3)\!\leadsto \!3$.

\addedHL{Note the information, {\it i.e.,} the at most $2\!+\! 2\log_2 N$ knowledge sets each vertex $i$  
learns after the $1 \!+\!\log_2 N$ iterations of the augmented knowledge-discovery procedure are a tiny percentage of information
the switch controller has under SERENA:  the former scales as $O(\log N)$ whereas the latter scales as $O(N)$.  
For example, in~\autoref{fig: comb-cycles}, vertex $3$ knows only the values the permutation
function $\sigma(\bigdot)$ takes on argument values $3$, $4$, and $12$, whereas under SERENA the (central) switch controller would know that on all $N \!=\! 16$ argument values.  
In general, 
different vertices have very different sets of such partial knowledges.  For example, vertex $2$ knows only the values the permutation
function $\sigma(\bigdot)$ takes on argument values $2$, $8$, and $11$.     
However, despite this ``blind men (different vertices) and an elephant ($\sigma$ and the green and the red weights of all walks
on the combinatorial cycles of $\sigma$)'' situation, these vertices manage to collaboratively perform the approximate or the exact  
MERGE operation ({\it i.e.}, making do with less).}
% [{\color{red}{\bf !!!!!!!! Move to the leader election section !!!!!}}]

% \addedHL{Note these $2+ 2\log_2 N$ knowledge sets each vertex $i$ learns after the $1 + \log_2 N$ iterations of SERENADE-common are a tiny percentage of information
% the switch controller has under SERENA:  the former scales as $O(\log N)$ whereas the latter scales as $O(N)$.  
% For example, in~\autoref{fig: comb-cycles}, vertex $3$ knows only the values the permutation
% function $\sigma(\bigdot)$ takes on argument values $3$, $4$, and $12$, whereas under SERENA the (central) switch controller would know that on all $N = 16$ argument values.  
% In general, 
% different vertices have very different sets of such partial knowledges.  For example, vertex $2$ knows only the values the permutation
% function $\sigma(\bigdot)$ takes on argument values $2$, $8$, and $11$.     
% However, despite this ``blind men (different vertices) and an elephant ($\sigma$ and the green and the red weights of all walks
% on the combinatorial cycles of $\sigma$)'' situation, these vertices manage to collaboratively perform the approximate or the exact  
% MERGE operation ({\it i.e.}, making do with less).}

%% 
\subsection{The Knowledge-Discovery Procedure}\label{subsubsec:knowledge-discover}

In this section, we detail the algorithmic steps of the knowledge-discovery procedure in the knowledge-discovery stage 
of SERENADE. First, we introduce the following definition and an important fact of it.

\begin{definition}\label{def:disc}
We say vertex $i$ {\bf discovers} vertex $j$ if $i$ learns the identity of $j$ and 
the weights of any walk from $i$ to $j$. Note that by this definition, every vertex 
$i$ discovers itself via a zero-length walk.
\end{definition}

\begin{fact}\label{fact:disc}
Given any two vertices $i$ and $j$ ($i,j$ could be the same) on a combinatorial cycle of $\sigma$, if vertex $i$ discovers the 
vertex $j$ twice via two different walks, then vertex $i$ can know precisely whether the green weight or the red weight 
of the cycle is larger. In particular, if $i,j$ are the same vertex, then vertex $i$ can do so if it discovers itself once via 
a walk with a positive length.
\end{fact}

It is obvious that the vertices can make the exact same matching decisions in SERENADE as they would 
in SERENA, if every vertex can discover  twice some vertex on the same cycle. That is the guideline 
of the SERENADE algorithm. 

We now describe the $1 \!+\! \log_2 N$ iterations of the knowledge-discovery procedure in detail and explain how
these iterations allow every vertex $i$ to concurrently discover its knowledge sets 
$\phi^{(i)}_{k+}$ and $\phi^{(i)}_{k-}$ 
for $k \!=\! 0, 1, 2, \cdots, \log_2 N$.

\begin{algorithm}[t]
\caption{The $k^{th}$ iteration of the knowledge-discovery procedure at input port $i$.}
\label{alg: serenade-general}
\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
\SetKwInOut{Input}{global}\SetKwInOut{Output}{out} 


\Input{Knowledge sets $\phi^{(i)}_{\xi+}$ and $\phi^{(i)}_{\xi-}, 0\!\leq\!\xi\!\leq\! k\!-\!1$, Array of pointers $\mathcal{B}$ of size $N$}


$i_D\leftarrow \sigma^{2^{k-1}}(i)$\;
$i_U\leftarrow \sigma^{-2^{k-1}}(i)$\;

Send to $i_U$ the knowledge set $\phi^{(i)}_{(k-1)+}$\;
\label{serenade: send-up}

Receive from $i_D$ the knowledge set $\phi^{(i_D)}_{(k-1)+}$\;
\label{serenade: receive-down}

Send to $i_D$ the knowledge set $\phi^{(i)}_{(k-1)-}$\;
\label{serenade: send-down}

Receive from $i_U$ the knowledge set $\phi^{(i_U)}_{(k-1)-}$\;
\label{serenade: receive-up}

Compute knowledge set $\phi^{(i)}_{k}$ with $\phi^{(i)}_{(k-1)+}$ and $\phi^{(i_D)}_{(k-1)+}$ by~\autoref{eq:comp-know}
\label{serenade: compute-knowledge-set}


Compute knowledge set $\phi^{(i)}_{k-}$ similarly with $\phi^{(i)}_{(k-1)-}$ and $\phi^{(i_U)}_{(k-1)-}$
\label{serenade: compute-knowledge-set-minus}

Halt if: (I) $\sigma^{2^k}(i)\!=\!\sigma^{-2^k}(i)$ or (II) $i$ has already discovered $\sigma^{2^k}(i)$ or $\sigma^{-2^k}(i)$ in the previous iterations, {\it i.e.,} $\mathcal{B}[\sigma^{2^k}(i)] \!\neq\!$ \texttt{NULL} 
or $\mathcal{B}[\sigma^{-2^k}(i)] \!\neq\!$ \texttt{NULL}\;
\label{serenade: halt-check}

$\mathcal{B}[\sigma^{2^k}(i)] \leftarrow \&\phi^{(i)}_{k+}$\;

$\mathcal{B}[\sigma^{-2^k}(i)] \leftarrow \&\phi^{(i)}_{k-}$\;


\end{algorithm}


\subsubsection{The \texorpdfstring{$k^{th}\,(k\geq 1)$}{kth} Iteration}\label{subsubsec: subsequent-iterations}

We first describe the $k^{th}$ iteration for $k\!\ge\!1$, since  
these iterations are extremely simple when described ``inductively" (recursively) whereas the 
$0^{th}$ iteration ({\it i.e.,} base case) is slightly different. \autoref{alg: serenade-general} shows 
the operations of the $k^{th}$ iteration at input port $i$, the operations 
of all other input ports are identical. Note that the global variables, {\it i.e.,} the knowledge sets and an array $\mathcal{B}$ 
that points to those knowledge sets that used for quickly checking whether a vertex is discovered 
twice, are private variables for each vertex, {\it i.e.}, each vertex has its own knowledge sets and array $\mathcal{B}$, 
which are initialized and updated as follows. The knowledge sets are set to empty initially and new knowledge sets learned 
after each iteration are inserted into it. The array $\mathcal{B}$ is initialized as all pointers pointing to \texttt{NULL}, 
and updated according to the last two lines of~\autoref{alg: serenade-general}. 

Suppose after iteration $k\!-\!1$ (for any $1\!\le\! k\!\le\! \log_2 N$), every input port $i$ discovers 
its upstream vertex $i_U \!=\! \sigma^{-2^{k-1}}(i)$ and its downstream vertex $i_D \!=\! \sigma^{2^{k-1}}(i)$ 
(\ie the ``induction hypothesis").
\autoref{alg: serenade-general} shows how input port $i$ discovers 
$\sigma^{2^{k}}(i)$ and $\sigma^{-2^{k}}(i)$ via two rounds of message exchanges of the 
iteration $k$ (\ie the ``inductive step"). More specifically, input port $i$ receives from $i_D$ 
the knowledge set $\phi^{(i_D)}_{(k-1)+}$ (\autoref{serenade: receive-down}), which, 
as explained earlier, contains the values of 
$\sigma^{2^{k-1}}(i_D)$, $w_r(i_D \!\leadsto\! \sigma^{2^{k-1}}(i_D))$, 
and $w_g(i_D \!\leadsto\! \sigma^{2^{k-1}}(i_D))$. With the knowledge sets $\phi^{(i_D)}_{(k-1)+}$ 
and $\phi^{(i)}_{(k-1)+}$ which, by the ``induction hypothesis", is learned by input port $i$ after the 
$(k-1)^{th}$ iteration, it then computes the knowledge set $\phi^{(i)}_{k+}$ (\autoref{serenade: compute-knowledge-set}) as follows.
\setlength{\belowdisplayskip}{0pt} \setlength{\belowdisplayshortskip}{0pt}
\setlength{\abovedisplayskip}{4pt} \setlength{\abovedisplayshortskip}{4pt}
\begin{equation}\label{eq:comp-know}\resizebox{0.913\hsize}{!}{
$\begin{cases}
\sigma^{2^k}(i) &\leftarrow \sigma^{2^{k-1}}\bigParenthes{i_D}\\
w_r\bigParenthes{i \leadsto \sigma^{2^k}(i)} &\leftarrow
w_r\bigParenthes{i \leadsto \sigma^{2^{k-1}}(i)} + w_r\bigParenthes{i_D \leadsto \sigma^{2^{k-1}}(i_D)}\\
w_g\bigParenthes{i \leadsto \sigma^{2^k}(i)} &\leftarrow
w_g\bigParenthes{i \leadsto \sigma^{2^{k-1}}(i)} + w_g\bigParenthes{i_D \leadsto \sigma^{2^{k-1}}(i_D)}
\end{cases}$
}\end{equation}

Similarly, input port $i$ discovers $\phi_{k-}^{(i)}$ by computing the knowledge set $\phi^{(i)}_{k-}$ 
(\autoref{serenade: compute-knowledge-set-minus}) with $\phi^{(i)}_{(k-1)-}$, which, 
by the ``induction hypothesis", is learned by input port $i$ after the 
$(k-1)^{th}$ iteration and $\phi^{(i_U)}_{(k-1)-}$, which is obtained at~\autoref{serenade: receive-up}. 
Therefore, vertex $i$ discovers $\sigma^{2^k}(i)$ and $\sigma^{-2^k}(i)$, more precisely, obtaining 
the knowledge sets $\phi_{k+}^{(i)}$ and $\phi_{k-}^{(i)}$ after the $k^{th}$ iteration.


\begin{figure}
\centering
\includegraphics[width=0.495\textwidth]{example_figures/v2/knowledge-discovery-example}
\caption{Illustration of the knowledge-discovery procedure at input $3$ of~\autoref{fig: comb-cycles}: 
The contents in each row of rectangle are the messages transmitted during each iteration, 
where the left one is sending from input $3$, and 
the right one is received by input $3$.}
\label{fig:knowledge-disc}
\end{figure}
Note that the knowledge-discovery procedure might stop before finishing the $(1\!+\!\log_2 N)$ iterations. 
As shown in~\autoref{serenade: halt-check} of~\autoref{alg: serenade-general}, the procedure will halt 
if input port $i$ discovers some vertex twice. By~\autoref{fact:disc}, 
we can conclude that vertex $i$ can make the exact same matching decision as it would in SERENA. We will 
prove later all other vertices on the same cycle as vertex $i$ can also do so. We will show later that if the 
knowledge-discovery procedure halts at~\autoref{serenade: halt-check}, vertex $i$ can use $O(1)$ operations to 
decide which is heaver between the green weight and the red weight of the cycle that vertex $i$ is on, and 
so can other vertices on the same cycle.

\begin{lemma}[All or nothing]\label{lemma:all-or-nothing}
During the execution of the knowledge-discovery procedure in SERENADE, if any vertex $i$ halts before 
reaching the $(\log_2 N)^{th}$ iteration, then all the other vertices on the same cycle as $i$ does will 
also halt at the same time. More specifically, if any vertex $i$ on a combinatorial cycle of $\sigma$ discovers 
a vertex on the same cycle twice during the knowledge-discover stage of SERENADE, all the other vertices 
also discover some vertex twice at the same iteration as $i$ does.
\end{lemma}

\begin{IEEEproof}
Suppose that vertex $i$ discovers vertex $j$ after the $k_1^{th}$ and $k_2^{th}$ iteration respectively. 
Then we have $\sigma^{m_1}(i)\!=\!\sigma^{m_2}(i)\!=\!j$ where $m_1\!=\!2^{k_1}$ if $i$ discovers $j$ 
through~\autoref{serenade: compute-knowledge-set} during the $k_1^{th}$ iteration, otherwise $m_1\!=\!-2^{k_1}$. 
Similarly, $m_2\!=\!\pm2^{k_2}$. Thus, we have $i\!=\!\sigma^{m_2-m_1}(i)$. Therefore, there exists 
some positive integer $\kappa$ such that $\abs{m_2-m_1} \!=\!\kappa \ell$ where $\ell$ is the length of 
the cycle. 

For any other vertex $x$ on the same cycle, we have $x\!=\!\sigma^{m_2-m_1}(x)$. Thus, 
$\sigma^{m_2}(x)\!=\!\sigma^{m_1}(x)\triangleq y$. Therefore, $x$ also discovers $y$ twice.
\end{IEEEproof}

\subsubsection{The \texorpdfstring{$0^{th}$}{0th} Iteration}\label{subsubsec: iteration-0}

Now we describe the the $0^{th}$ iteration, as mentioned before, the operation of which is slightly different than that of subsequent iterations
in that whereas messages are exchanged only between input ports in all subsequent iterations, they are
also between input ports and output ports in the $0^{th}$ iteration.  We explain the operations carried out at output port $j$;  those carried out at any other output port
are identical.
Suppose output port $j$ is paired with input port $i_r$ in the (red) full matching $S_r$ and with
input port $i_g$ in the (green) full matching $S_g$.
The $0^{th}$ iteration contains two rounds of message exchanges. In the first round, each output port $j$ sends
a message to the input port $i_g$,
informing it of the identity $i_r$ and
the (red) weight of the edge $i_r \rightarrow j$ in the (red) matching $S_r$. 
Note that $\sigma(i_r) = i_g$ by the definition of $\sigma$.  In the second round, the input port $i_g$ relays the following
information to the input port $i_r$: $w_g(i_r\rightarrow i_g)$ and $w_r(i_r\rightarrow i_g)$.
Clearly after this $0^{th}$ iteration, each input port $i$ discovers $\sigma(i)$ and $\sigma^{-1}(i)$. 
More specifically, it obtains the knowledge sets $\phi^{(i)}_{0+}$ and $\phi^{(i)}_{0-}$.

\subsubsection{Discussions}\label{subsubsec: logical_bypass}
\modifiedHL{Note that, in describing %the SERENADE common part 
SERENADE-common 
and all SERENADE variants,
we assume that input ports
can communicate directly with each other.  This is a %very 
realistic assumption, because in most 
real-world switch products, each line card $i$ is full-duplex in the sense
the logical input port $i$ and the logical output port $i$ are 
co-located in the same physical line card $i$.  In this case, for example, an input port $i_1$
can communicate with another input port $i_2$ by sending information to output port $i_2$, which then relays it to 
the input port $i_2$ through the ``local bypass", presumably at little or no communication 
costs.  However, the SERENADE algorithms can also work for the type of switches that do not have such a ``local bypass," 
by letting an output port to serve as a relay, albeit at twice the communication costs.  More precisely, in the example above, the input port $i_1$ can send the 
information first to the output port $i_1$, which then relays the information 
to the input port $i_2$.}  

\subsubsection{Complexities of The Knowledge-Discovery Procedure}
\label{subsec: complexity-common}

%\footnote{We do not use the ``big $O$" notation here to emphasize the constant factor $1$.}

\modifiedHL{The time complexity of the knowledge-discovery procedure is $1 \!+\! \log_2 N$ iterations, 
and that of each iteration is %clearly
several operations for local computation for computing knowledge sets (\autoref{serenade: compute-knowledge-set} of \autoref{alg: serenade-general}) and checking for the halt condition  
(\autoref{serenade: halt-check} of \autoref{alg: serenade-general}). Clearly, those operations can be performed 
in $O(1)$. 
The total message complexity of the knowledge-discovery procedure is $O(\log N)$ messages per vertex, since 
every vertex needs to send (and receive) two messages 
during each iteration.}


\subsection{Why \texorpdfstring{$(1\!+\!\log_2 N)$}{1+logN} iterations?}\label{subsec:ouroboros-theory}

In the above section, we take the $1\!+\!\log_2N$ iterations for granted. In this section, we show the 
reasons behind $1\!+\!\log_2N$ iterations. For ease of presentation, in this section, we assume that 
the knowledge-discovery procedure can run ant number of iterations until it halts at~\autoref{serenade: halt-check} 
of~\autoref{alg: serenade-bsearch} unless explicitly stated.

First, the following theorem shows that the knowledge-discovery procedure halts  
after at most $N/2$ iterations.

\begin{theorem}\label{thm:stop}
The knowledge-discovery procedure described in~\autoref{subsubsec:knowledge-discover} will halt after at most $N/2$ iterations.
\end{theorem}

\begin{IEEEproof}
By~\autoref{lemma:all-or-nothing}, it is clear that during each iteration of the knowledge-discovery procedure, each vertex 
either discovers two new vertices or the procedure halts 
at~\autoref{serenade: halt-check} of~\autoref{alg: serenade-bsearch}. Therefore, if the procedure does not halt after the 
$k^{th}$ iteration, then vertex $i$ has discovered $2k+1$ different vertices (including itself). 
Since there are at most $N$ different vertices in a combinatorial cycle, by Pigeonhole principle~\cite{Brualdi2009}, 
some vertex has to be discovered twice after $N/2$ iterations.
\end{IEEEproof}

Note that~\autoref{thm:stop} only provides an upper bound for the number of iterations required by 
the knowledge-discovery procedure. The number of iterations 
required by the knowledge-discovery procedure could be much less than $N/2$. Clearly, 
it is determined by the length $\ell$ of the combinatorial cycle that the vertex is on.  
To calculate the exact number of iterations for an arbitrary $\ell$ 
is outside the scope of this work, 
% because whether the knowledge-discovery procedure requires $N/2$ iterations 
% us to solve the Artin's Conjecture~\cite{stein2008elementary} 
% with restricted to the integer $2$. Fortunately, 
as the cycle length $\ell$ in the context of SERENADE is 
usually at most several thousand, for which the number of iterations is amenable to compute naively. 
\autoref{fig:number-of-iterations} shows the number of iterations for $\ell\!\le 64\!$. 
\autoref{tab:max-iter} presents the maximum number of iterations for all possible combinatorial cycles under the 
cases of $N\!=\!64,128,\cdots,1024$, as we can 
see the maximum number of iterations required by the knowledge-discovery procedure is very close to $N/2$, which 
exceeds SERENADE's budget.

Therefore, we only run the knowledge-discovery procedure for $1\!+\!\log_2 N$ iterations as the leader election  
required by the distributed binary search procedure in the binary search stage needs at least $1\!+\!\log_2 N$. 

\begin{figure}
\centering 
\includegraphics[width=0.49\textwidth]{figures/ouroborous/number-of-iterations}
\caption{Number of iterations for different cycle lengths.}\label{fig:number-of-iterations}
\end{figure}

\begin{table}
\centering
\caption{Maximum number of iterations.}\label{tab:max-iter}
\begin{tabular}{@{}rccccc@{}}
\toprule
N & 64 & 128 & 256 & 512 & 1024 \\\midrule
Maximum number of iterations & 31 & 56 & 114 & 255 & 510\\\bottomrule
\end{tabular}
\end{table}

%%%

% \subsection{Complexities of SERENADE-common}
% \label{subsec: complexity-common}

% %\footnote{We do not use the ``big $O$" notation here to emphasize the constant factor $1$.}

% \modifiedHL{The time complexity of SERENADE-common is $1 + \log_2 N$ iterations, 
% and that of each iteration is %clearly
% several CPU instructions:  roughly $4$ instructions for computing knowledge sets (\autoref{serenade: compute-knowledge-set} of \autoref{alg: serenade-general}) and another $4$ for checking for the ouroboros condition  
% (\autoref{serenade: halt-check} of \autoref{alg: serenade-general}) to be more precise.   
% %Hence its total time complexity is $3 + 2 \log_2 N$ instructions, including the comparison between the green and the red weights.  
% % \glong{For interest of space, we defer the description of how $i$ can check 
% % whether or not it is on an ouroboros cycle (\ie \autoref{serenade: halt-check} of \autoref{alg: serenade-general}) in $O(1)$ to \autoref{subsec: check-for-ouroboros}.} 
% The total message complexity of SERENADE-common is 
% %$O(N \log N)$ messages, or 
% $O(\log N)$ messages per vertex, since 
% every vertex needs to send (and receive) two messages 
% % comparable to
% during each iteration.}

%This message complexity is asymptotically smaller than that of iSLIP~\cite{McKeown99iSLIP}, 
%in which the $N$ input ports need to send, among other things, a total of $N^2$ bits, indicating whether each of the
%$N^2$ VOQs is empty or not, to the switch controller.  

\subsection{Leader Election}
\label{subsec: leader-election}

\addedHL{
% As analyzed in~\autoref{subsec:ouroboros-theory}, by using the knowledge-discovery procedure alone, SERENADE needs roughly up to $N/2$ iterations 
% to let every vertex to make the same matching decision as it would do in SERENA. We need some strategy to reduce 
% the number of iterations. 
As explained in~\autoref{subsec: merge}, every vertex in a combinatorial 
cycle will select the same sub-matching, {\it i.e.,} making the same decision on 
selecting the red or green edge, in SERENA. A straightforward, economical and commonly used strategy 
to save messages that need to be transmitted in distributed computing is to select 
a designated vertex, {\it i.e.,} a master or a leader, to make decision for all the vertices. 
The process for identifying the ``leader'' 
is called {\bf leader election}, which is commonly used in various distributed systems, 
such as Apache ZooKeeper~\cite{zookeeper2018} and Kubernetes~\cite{kubernetes2016}. 
Although leader election is in general a relatively expensive operation~\cite{attiya2004distributed,Lynch1996Distributed}, 
it is much less so in SERENADE, since leader 
election can be seamlessly embedded into the knowledge-discovery procedure, and leader elections on distinct cycles 
can be computed in parallel within $1\!+\!\log_2N$ iterations, as we will show shortly.} 

Now we describe 
how to embed the leader election process into the knowledge-discovery procedure of SERENADE. 
We explain this process on an arbitrary combinatorial cycle of $\sigma$, 
focusing on the actions of an arbitrary vertex $i$ that belongs to this cycle.  
We follow the standard practice~\cite{Perlman2000:leaderelection} of making the vertex with the
smallest identity (an integer between $1$ and $N$) on this cycle the leader.  
Recall that in the knowledge-discovery procedure, after each (say $k^{th}$) iteration,
vertex $i$ discovers $\sigma^{-2^{k}}(i)$ that is ``$2^k$ $\sigma$-hops away" from it on the cycle. 
Our goal is to augment this $k^{th}$ iteration to learn the vertex with the smallest identity on 
this walk $\sigma^{-2^k}(i)\!\leadsto\! i$, which we denote as $\calL(\sigma^{-2^k}(i)\!\leadsto\! i)$
and call a level-$k$ ``precinct leader."  
% It is clear that this augmented knowledge-discovery procedure 
% requires $1\!+\!\log_2 N$ iterations (including the $0^{th}$ iteration) to make all vertices learn the 
% identity of the leader. Because the length of any cycle is no larger than $N$, the
% length of the precinct (walk) $\sigma^{-N}(i)\!\leadsto\! i$, of which the precinct leader 
% $\mathcal{L}(\sigma^{-N}(i)\!\leadsto\! i)$ learned during the $(\log_2 N)^{th}$ iteration 
% must be $\calL_0$, the leader of the entire cycle. 


Like in the knowledge-discovery procedure, we explain this augmentation ``inductively."
The case of $k\!=\!0$ ({\it i.e.}, the $0^{th}$ iteration) is trivial:  Each vertex $i$ considers 
the one with smaller identity between itself and $\sigma^{-1}(i)$ 
to be the leader of its respective level-0 precinct.

For the $k^{th}$ ($k\!\ge\!1$) iteration, each vertex $i$ only needs to augment the knowledge set it 
sends downstream to $i_D\!=\!\sigma^{2^{k-1}}(i)$ with the leadership information $\mathcal{L}(\sigma^{(-2^{k-1})}(i)\!\leadsto\!i)$ 
at~\autoref{serenade: send-down} of~\autoref{alg: serenade-general}. Clearly, it will 
receives, from $i_U\!=\!\sigma^{(-2^{k-1})}(i)$, the vertex $2^{k\!-\!1}$ $\sigma$-hops upstream, 
its level-$(k-1)$ precinct leader information at~\autoref{serenade: receive-up} of~\autoref{alg: serenade-general}, 
as $i_U$ also augments its knowledge set. In addition, each vertex $i$ also adds the following local computation 
at~\autoref{serenade: compute-knowledge-set-minus} of~\autoref{alg: serenade-general}.
\setlength{\belowdisplayskip}{0pt} \setlength{\belowdisplayshortskip}{0pt}
\setlength{\abovedisplayskip}{4pt} \setlength{\abovedisplayshortskip}{4pt}
\[\resizebox{0.95\hsize}{!}{
$\mathcal{L}(\sigma^{-2^{k}}(i) \leadsto i) \!\leftarrow\! \min\big{\{}\mathcal{L}(\sigma^{(-2^{k-1})}(i_U)\!\leadsto\!i_U), \mathcal{L}(\sigma^{(-2^{k-1})}(i)\!\leadsto\!i)\big{\}}$
}
\]

The following theorem concerns the correctness of and the minimum number of iterations required by 
the above embedded leader election process. Its proof is straightforward, we omit 
it in this paper.

\begin{theorem}\label{thm:leader-election}
Each vertex $i$ will learn, through the augmented knowledge-discovery procedure, the identity of the leader for the cycle vertex $i$ is on, 
after at most $1\!+\!\log_2N$ iterations, 
if the knowledge-discovery procedure executed at vertex $i$ does not halt at~\autoref{serenade: halt-check}. 
Besides, there exists some cycle such that some of its vertices need at least $1\!+\!\log_2N$ iterations to 
learn the identity of the leader.
\end{theorem}

Once the leader of a cycle is decided, through a distributed binary search procedure, the leader will discover itself 
(through a walk with positive length). 
According to~\autoref{fact:disc}, the leader now can make the same matching decision as it would in SERENA. Then, 
the leader $\calL_0$ informs the switch controller of its decision on whether to 
choose the green or the red sub-matching, and the switch controller then broadcast decisions of ``all leaders'' to 
the $N$ vertices. As we explained in~\autoref{subsec:ouroboros-theory}, 
not all cycles need its leader to make the matching decisions. 
We call those cycles, which do not need the leader to make the matching 
decision for, the ouroboros cycles. The formal definition will be presented shortly. Similarly, we call the others 
the non-ouroboros cycles. 
% Given a permutation, the number of iterations, which the knowledge-discovery procedure runs for, determines 
% the number of non-ouroboros cycles.

As explain above, the switch controller has to broadcast the leaders' decisions. 
The size of this broadcast, equal to the number of {\it non-ouroboros} cycles in $\sigma$, 
is small (with overwhelming probability).
% as small as possible. 
% It is obvious the more iterations the knowledge-discovery procedure runs for, the smaller 
% the size of this broadcast, whereas the more messages are transmitted during the knowledge-discovery stage. 
% If we could know the distribution of all the permutations ({\it e.g.}, by profiling 
% historical data), then we can formulate an optimization problem for the number of iterations to obtain the optimal 
% number of iterations to minimize the communication complexity. This is however outside the scope of this paper.  
% In this paper, we simply let the number of iterations be $1\!+\!\log_2N$. We find, through simulations, the size of 
% broadcast when SERENADE runs the knowledge-discovery procedure for $1\!+\!\log_2N$ iterations, is small (with overwhelming probability). 
For example, even when $N \!=\! 1,024$, the average 
number of non-ouroboros cycles is only $2.667$ for a uniform random permutation.
Since each vertex on a non-ouroboros cycle knows the identity of its leader by~\autoref{thm:leader-election},
it will follow the decision made by its leader in choosing between the red and the green edges. 
Note that when there are many non-ouroboros cycles, albeit is rare 
empirically, the above broadcast approach would not scale. Under such a case, 
the switch controller, after getting the decisions from all the leaders, can simply 
broadcast a bitmap with length $N$. The $i^{th}$ bit equals $1$ indicates that 
the vertex $i$ picks the red sub-matching, otherwise, the green sub-matching is 
picked by $i$. Clearly, this broadcast scheme, costing more bits when there are 
few non-ouroboros cycles, has a fixed size of $N$ bits and every vertex on 
a non-ouroboros cycle can read its leader's decision in one operation.


% We claim that after iteration $k\!-\!1$, every input port $i$ gets two things done (This claim is ``the induction hypothesis").  
% First, $i$ learns the identity of $\mathcal{L}(\sigma^{(-2^{k\!-\!1})}(i) 
% \!\leadsto\!i)$, the leader of the level-($k\!-\!1$) precinct right-ended at
% $i$ (Part I of the claim). Second, $i$
% receives, from $i_U\!=\!\sigma^{(-2^{k-1})}(i)$, the vertex $2^{k\!-\!1}$ $\sigma$-hops upstream, its level-$(k-1)$ precinct leader information (Part II of the claim).
% However, the union of these two level-$(k\!-\!1)$ precincts $\mathcal{L}(\sigma^{(-2^{k\!-\!1})}(i) \!\leadsto\! i)$ and $\mathcal{L}(\sigma^{(-2^{k\!-\!1})}(i_U) \!\leadsto\! i_U)$ is precisely the level-$k$ precinct $\mathcal{L}(\sigma^{-2^{k}}(i) \!\leadsto\! i)$. 
% Hence, in iteration $k$,  input port $i$ simply computes 
% %
% %$... \leftarrow \min\big{\{}\mathcal{L}(\sigma^{(-2^{k-1})}(i_U)\!\leadsto\!i_U), \mathcal{L}(\sigma^{(-2^{k-1})}(i)\!\leadsto\!i)\big{\}}.$
% $ \mathcal{L}(\sigma^{-2^{k}}(i) \leadsto i) \!\leftarrow\! \min\big{\{}\mathcal{L}(\sigma^{(-2^{k-1})}(i_U)\!\leadsto\!i_U), \mathcal{L}(\sigma^{(-2^{k-1})}(i)\!\leadsto\!i)\big{\}}$, so part I of the above claim is fulfilled;  this local computation is added to \autoref{alg: serenade-general} as ``Line 5.5".
% In addition, (each) vertex $i$ sends the information $\mathcal{L}(\sigma^{(-2^{k-1})}(i)\!\leadsto\!i)$ downstream to $i_D=\sigma^{2^{k-1}}(i)$, so part II of the above claim is fulfilled;  this information is appended to the message
% that $i$ sends to $i_D$ in \autoref{serenade: send-down} of \autoref{alg: serenade-general} and hence does not require a separate message exchange.  Therefore, the ``inductive step is proved''.

% \addedHL{To summarize, the leader election process incurs only a small additional message complexity: 
% a $\log_2 N$-bit-long ``precinct leader'' field needs to be added,
% in each iteration of SERENADE-common, to one of the two messages sent by each vertex. 
% Note however this 
% field 
% has to be included in these messages from 
% % round $0$
% the $0^{th}$ iteration 
% onwards, if the switch intends to execute O-SERENADE in this time slot.
% This is the reason why the switch controller is required to declare this intention at the beginning of the time slot 
% (mentioned in $\autoref{sec: serenade-algorithms}$). }




\subsection{The Ouroboros Cycles}\label{subsec:ouroborous-cycle}

\begin{figure}
\centering
\includegraphics[width=0.498\textwidth]{example_figures/v2/ouroboros-number}
\caption{Illustration of three cases corresponding to the three forms of the ouroboros numbers.}
\label{fig:ouroboros-numbers}
\end{figure}
In the previous sections, we have shown that after the (at most) $1\!+\!\log_2N$ iterations of the knowledge-discovery procedure, 
vertices on some cycles, more precisely, vertices that halt at~\autoref{serenade: halt-check} of~\autoref{alg: serenade-general}, 
can immediately make the exact same matching decisions as they would in SERENA. In this section, we will make it clearer vertices 
on which cycles can do so. 
% As mentioned before, we call those cycles as ouroboros cycles. We will show in this section that a  
% cycle is ouroboros if its length is one of certain special numbers, which we call ouroboros numbers. 

\modifiedHL{
% Fix a vertex $i$, we have just shown that after the (at most) $1\!+\!\log_2 N$ iterations 
% of the knowledge-discovery procedure, vertex $i$ either discovers some vertex twice or has learned the following 
% knowledge sets: $\phi_{k+}^{(i)}$ and $\phi_{k-}^{(i)}$ for $k=0,1,\cdots,\log_2 N$. 
% Armed with these knowledge sets, vertex $i$ can immediately determine whether any of the following three ideal situations occurs:
% \begin{spenumerate}
%     % \item $\sigma^{2^j}(i)$, the index/identity of the vertex (input port) that is the
%     % ending point of the walk $\mathcal{W}_{i}(2^j)$,
% %    \item there is a nonnegative integer $n\le \log_2 N$, such that $i = \sigma^{2^n}(i)$, since $\sigma^{2^n}(i) \in \phi^{(i)}_{n+}$;
% \item $i = \sigma^{2^n}(i)$ for some nonnegative integer $n\le \log_2 N$ (since $\sigma^{2^n}(i) \in \phi^{(i)}_{n+}$);
%     % \item $\sigma^{-2^j}(i)$, the index/identity of the vertex (input port)
%     % that is starting point of the walk $\mathcal{W}_{i}(-2^j)$,
%     % \item $\sigma^{-2^j}(i)$, the index/identity of the vertex (input port) that is $2^j$ steps
%     % (edges) ``upstream",
%     %\item The red weight $w_r(i \leadsto \sigma^{2^k}(i))$ and the green weight $w_g(i \leadsto \sigma^{2^k}(i))$ of the walk $i \leadsto \sigma^{2^k}(i)$.
%     \item $\sigma^{2^n}(i) = \sigma^{2^m}(i)$ for some nonnegative integers $n < m \le \log_2 N$ (since $\sigma^{2^m}(i) \in \phi^{(i)}_{m+}$);
%     \item $\sigma^{-2^n}(i) = \sigma^{2^m}(i)$ for some nonnegative integers $n < m \le \log_2 N$ (since $\sigma^{-2^n}(i) \in \phi^{(i)}_{n-}$).
%     % \item The green weights of the walks $\mathcal{W}_{i}
%     % (\pm 2^j)$.
% \end{spenumerate}

% Let $l$ be the length of the cycle to which vertex $i$ belongs.  
% %Note that $l$ is the smallest positive integer such that $\sigma^l(i) = i$.
% The three situations above are considered ideal because, as we 
% % will show in~\autoref{sec: explanation-three-ideal}, 
% have shown in~\cite{Gong2017arXivSERENADE},
% whenever one of them occurs, the vertex $i$ -- and all other vertices on the same cycle $i\leadsto \sigma^l(i)$ --
% know precisely whether $w_g(i\leadsto \sigma^l(i))$,
% the green weight of the cycle, or $w_r(i\leadsto \sigma^l(i))$, the red weight of the cycle, is larger (but do not generally know the exact weights). 
% Therefore, with this knowledge, every vertex on this cycle will select, under SERENADE, the same 
% sub-matching, as under SERENA.  
% %Note that, in general, $i$ knows the exact 
% %value of neither $w_g(i\leadsto \sigma^l(i))$ nor $w_r(i\leadsto \sigma^l(i))$ in the second and the third situations. 
% We will show that one or more of the three situations above 
% would happen, 
Fix a vertex $i$, we will show next that the knowledge-discovery procedure at vertex $i$ can halt at~\autoref{serenade: halt-check} because of 
discovering some vertex twice, if and only if $i$ is on an {\it ouroboros cycle}, defined next. 
\begin{definition}[Ouroboros Cycle]\label{fact: ouroboros-numbers}\label{def: ouroboros-cycle}
A cycle is {\bf ouroboros} if and only if its length $l$ is an {\it ouroboros number} ({\it w.r.t.} $N$), 
defined as a positive divisor of a number that takes one of the following three forms: 
(I) $2^\alpha$, (II) $2^\beta \!-\! 2^\gamma$, and (III) $2^\beta \!+\! 2^\gamma$, where $\alpha$, 
$\beta$ and $\gamma$ are nonnegative integers that satisfy $\alpha\!\leq\!\lceil\!\log_2 N \rceil$ and 
$\gamma\!<\!\beta\!\leq\!\lceil\!\log_2 N \rceil$.
\end{definition}

It is easy to check that, in~\autoref{fig: comb-cycles}, the leftmost cycle (of length $11$) 
is not ouroboros ({\it i.e.}, non-ouroboros), but the other two are. 
% Once a vertex $i$ finds out that it is on an ouroboros cycle -- and so 
% do other vertices on this cycle at this point -- they can all halt their computations immediately. 
Now, we prove that vertex $i$ on an {\it ouroboros cycle} will halt 
at~\autoref{serenade: halt-check} of~\autoref{alg: serenade-general}, 
which is summarized as the following lemma.
\begin{lemma}[Ouroboros Lemma]\label{lemma:ouroboros-lemma}
Vertex $i$ will discover twice some vertex, if it is on an ouroboros cycle.
\end{lemma}
The proof of this lemma is straightforward, here we only show the proof sketch for brevity. 
It is not hard to show that if the cycle, on which vertex $i$ is, has a length of an ouroboros numbers 
in the three forms defined in~\autoref{def: ouroboros-cycle}, 
then vertex $i$ will discover twice another vertex in the same iteration 
({\it i.e.,} halting because of condition (I) at~\autoref{serenade: halt-check} 
of~\autoref{alg: serenade-general}), another vertex along two different walks with 
the same direction, and another vertex along 
two different walks with the opposite direction, respectively. \autoref{fig:ouroboros-numbers} 
illustrates the three different cases. Note that for (II) and (III) in~\autoref{fig:ouroboros-numbers}, 
both the two walks can coil around the cycle for one or more times, and the directions of the two 
walks can be reversed. For example, for (III) in~\autoref{fig:ouroboros-numbers}, the two walks could also 
be $\sigma^{-2^\gamma}(i)\!\leadsto\!i$ and $i\!\leadsto\!\sigma^{2^\beta}(i)$, and both of them could 
coil around the cycle for one or more times, {\it i.e.,} they are longer than the cycle.

% For example, in~\autoref{fig: comb-cycles}, the leftmost cycle (of length $11$) 
% is not ouroboros ({\it i.e.}, non-ouroboros), but the other two are.} 
% \modifiedHL{Once a vertex $i$ finds out that it is on an ouroboros cycle -- and so 
% do other vertices on this cycle at this point -- they can all halt their computations immediately, 
% as shown in~\autoref{serenade: halt-check} of~\autoref{alg: serenade-general}. 
% We have shown in~\cite{Gong2017arXivSERENADE} that, with a simple data structure, 
% checking the ouroboros condition has $O(1)$ time complexity.
}

%% Procedure version
\begin{algorithm}[tb]
\caption{Distributed binary search at vertex $i$.}
\label{alg: serenade-bsearch}
\SetKwRepeat{Do}{do}{while}
\SetKwProg{Proc}{Procedure}{}{end}
\SetKwFunction{algo}{\small BinarySearch}

% \tcc{After ($i$) receiving the baton }
%\tcc{\small $l$: precinct level, $w_g$: $w_g(\calL\leadsto i)$, $w_r$: $w_r(\calL\leadsto i)$}
% \Proc{BinarySearch($i$, $d$, $w_g$, $w_r$)}{

\Proc{BinarySearch($i$, $k$, $w_g$, $w_r$)}{\label{bsearch: entrance}

    If $i$ (self) is $\mathcal{L}_0$ then halt\;
    \label{code: exit-check}

    % Update depth of the search: $d \leftarrow d + 1$\;
    % \label{code: depth-update}

    % \eIf{$\sigma^{(-N/2^{d + 1})}(i)=\sleader$}
    \eIf{$\sigma^{(-2^{k-1})}(i)=\sleader_0$}
    {\label{code: endpoint-check}\label{code: middle-check}

        % \algo{$\sigma^{(-N/2^{d +1})}(i)$, $d + 1$}\;
        % $w_g \leftarrow w_g - w_g\bigParenthes{\sigma^{(-N/2^{d+1})}(i) \leadsto i}$\;
        $w_g \leftarrow w_g - w_g\bigParenthes{\sigma^{(-2^{k-1})}(i) \leadsto i}$\;
        \label{code: green-weight-update}

        % $w_r \leftarrow w_r - w_r\bigParenthes{\sigma^{(-N/2^{d+1})}(i) \leadsto i}$\;
        $w_r \leftarrow w_r - w_r\bigParenthes{\sigma^{(-2^{k-1})}(i) \leadsto i}$\;
        \label{code: red-weight-update}

        % \algo{$\calL$, $d + 1$, $w_g$, $w_r$}\;
        \algo{$\calL_0,k \!-\! 1,w_g,w_r$}\;
        \label{code: final-passing}



    }
    {


        % \eIf{$\mathcal{L}$ is on the walk $\sigma^{(-N/2^{d+1})}(i) \leadsto i$} {\label{code: walk-leader-check}
        \eIf{$\mathcal{L}_0=\calL(\sigma^{(-2^{k-1})}(i) \leadsto i$)} {\label{code: walk-leader-check}

            % \algo{$i$, $d + 1$, $w_g$, $w_r$}\;
            \algo{$i$, $k - 1$, $w_g$, $w_r$}\;
            \label{code: dummy-passing}
        }
        {

            % $w_g \leftarrow w_g - w_g\bigParenthes{\sigma^{(-N/2^{d+1})}(i) \leadsto i}$\;
            % \label{code: green-weight-update}

            % $w_r \leftarrow w_r - w_r\bigParenthes{\sigma^{(-N/2^{d+1})}(i) \leadsto i}$\;
            % \label{code: red-weight-update}
            % $w_g \leftarrow w_g - w_g\bigParenthes{\sigma^{(-N/2^{d+1})}(i) \leadsto i}$\;
            $w_g \leftarrow w_g - w_g\bigParenthes{\sigma^{(-2^{k-1})}(i) \leadsto i}$\;
            \label{code: green-weight-update-}

            % $w_r \leftarrow w_r - w_r\bigParenthes{\sigma^{(-N/2^{d+1})}(i) \leadsto i}$\;
            $w_r \leftarrow w_r - w_r\bigParenthes{\sigma^{(-2^{k-1})}(i) \leadsto i}$\;
            \label{code: red-weight-update-}

            % \algo{$\sigma^{(-N/2^{d +1})}(i)$, $d + 1$, $w_g$, $w_r$}\;
            \algo{$\sigma^{(-\!2^{k \!-\!1})}(i){,}k \!-\! 1{,}w_g{,}w_r$}\;
            \label{code: intermediate-passing}
        }
    }

} % end procedure
\end{algorithm}

\subsection{Binary Search Stage}\label{subsec:bs}

As mentioned above, only vertices on ouroboros cycles can make the exact same decisions as they would in SERENA, for vertices 
on non-ouroboros cycles, SERENADE needs the an extra binary search stage. In this section, we will describe the binary search stage 
focusing on an arbitrary non-ouroboros cycle.

\subsubsection{Distributed Binary Search}\label{subsubsec: b-search}  
% It suffices to describe this distributed algorithm on an arbitrary non-ouroboros cycle,
% since every non-ouroboros cycle runs an (distinct) instance of the same
% algorithm.  Hence, w
Without loss of generality, we assume that $\calL_0$ is the leader of, and $i$ a
vertex on, this non-ouroboros cycle. The objective of this distributed algorithm is 
to let its leader $\calL_0$ discovers itself 
twice by searching a repetition ({\it i.e.,} other than its first occurrence as the starting point of the walk) of $\calL_0$ 
along the walk $\mathcal{L}_0\!\leadsto\!\sigma^N(\mathcal{L}_0)$, the level-($\log_2 N$) precinct 
right-ended at $\sigma^N(\mathcal{L}_0)$;  this repetition must exist
because $N$, the length of the walk $\mathcal{L}_0 \leadsto \sigma^N(\mathcal{L}_0)$, is no smaller than
the length of this cycle.   
\modifiedHL{To this end, vertices on this non-ouroboros cycle perform a distributed binary search, guided by the
aforementioned 
% ``intermediate" and ``final products" %(\ie the identities of the level-$0$ to level-$N$ precinct leaders right-ended at $i$) 
leadership information 
each vertex obtains through the leader
election process.} \addedHL{In the following, we describe the high-level ideas of this binary search algorithm
%  while referring readers to~\cite{Gong2017arXivSERENADE} for its pseudocode and detailed
% descriptions.
% whose pseudo-code is shown in~\autoref{alg: serenade-bsearch}.
, in which the detailed actions of a vertex $i$ is captured in~\autoref{alg: serenade-bsearch}. 
} Unlike the knowledge-discovery procedure, during each iteration of the distributed binary search, only one 
vertex on this non-ouroboros cycle will perform the search task, which we call {\it the search administrator}. 

This binary search is initiated by the vertex
$\sigma^{N}(\calL_0)$, who learns ``who herself is" (\ie that herself is $\sigma^{N}(\calL_0)$) during the last iteration 
of the knowledge-discovery procedure;  in other words, the initial {\it search administrator} is $\sigma^{N}(\calL_0)$.
The initial {\it search interval} is the entire walk $\calL_0\leadsto\sigma^{N}(\calL_0)$, also the level-$(\log_2 N)$ precinct right-ended at $\sigma^{N}(\calL_0)$.
%, which consists of $N$ edges (\ie is of length $N$).  
The search administrator $\sigma^{N}(\calL_0)$ first checks whether itself or $\sigma^{N/2}(\calL_0)$, the middle point 
of the search interval, is a repetition of $\calL_0$. If so, the entire search mission is accomplished, so the 
search ends. Otherwise, it checks 
whether there is a repetition of $\calL_0$ in the right half of the search interval (\ie the walk
$\sigma^{-N/2}(i)\leadsto i$) by checking whether
$\calL(\sigma^{N/2}(\calL_0)\leadsto\sigma^{N}(\calL_0))$ is equal to $\calL_0$;  note the identity of $\calL(\sigma^{N/2}(\calL_0)\leadsto\sigma^{N}(\calL_0))$, 
the leader of the level-$(\log_2 (N) - 1)$ precinct right-ended at $\sigma^{N}(\calL_0)$,
is known to $\sigma^{N}(\calL_0)$, since it is one of the aforementioned leadership information $\sigma^{N}(\calL_0)$ learns through the leader election
process.
If so, the same search administrator $\sigma^{N}(\calL_0)$ carries on this binary search in the right half of the search interval.  
Otherwise, the ``middle point" of the search interval $\sigma^{N/2}(\calL_0)$ becomes the new search administrator and carries on this binary search in the left half.  
%Clearly, it takes at most $\log_2 N$ steps for this binary search to end (with finding a repetition of $\calL_0$).
%This way, with each step of this binary search, the search interval is halved (and becomes a precinct that is one level lower), 
%and if needed, a different vertex that is at least twice as close to the target becomes the new search administrator.

As mentioned above, the detailed actions of any search administrator $i$ is captured by~\autoref{alg: serenade-bsearch}. 
Initially $i$ is $\sigma^{N}(\calL_0)$ who assigns $\log_2 N$ to $k$, the $2^{nd}$ argument 
of~\autoref{alg: serenade-bsearch}, which indicates the search interval is $\sigma^{-2^k}\!\leadsto\!i$. To ensure that 
$\calL_0$ can discover itself, {\it i.e.,} learning the green and red weights of a walk of positive length from 
$\calL_0$ to itself, search administrator $i$ also maintains the weight information $w_g$, $w_r$ (the $3^{rd}$ and $4^{th}$ 
arguments of~\autoref{alg: serenade-bsearch}), 
which are the green and red weights 
of the walk from $\calL_0$ to $i$. We will not describe~\autoref{alg: serenade-bsearch} line-by-line, 
since the actions of search administrator $i$ is straightforward after we describe the high-level ideas.

\begin{figure}[t]
\centering
\includegraphics[width=0.49\textwidth]{example_figures/v2/bs-example}
\caption{Distributed binary search on the leftmost cycle in~\autoref{fig: comb-cycles}.}
\label{fig:bs-example}
\end{figure}

\noindent
{\bf An Illustrative Example.} 
\autoref{fig:bs-example} shows an example of the distributed binary search procedure by using the non-ouroboros cycle 
in~\autoref{fig: comb-cycles}. In~\autoref{fig:bs-example}, the dotted line indicates that the vertex $i$ only checks 
whether the leader of the corresponding walk is $\calL_0$, {\it i.e.,} there are no message exchanges, whereas the solid 
line with arrow indicates that the changing of the search administrator, {\it i.e.,} message exchanges occur. 
It is clear that vertex $2$ is the leader and $12\!=\!\sigma^{2^4}(2)$ is the initial search 
administrator in this cycle. 
Vertex $12$ first checks whether $14\!=\!\sigma^{-2^3}(12)$ is the leader and 
gets a negative answer. Then it finds that the leader of the walk $\sigma^{-2^3}(12)\!\leadsto\!12$ equals $2$, thus it 
continues to carry on this binary search in the next search interval. 
Now it finds that the leader of the walk 
$\sigma^{-2^2}(12)\!\leadsto\!12$ is not $2$, so $8\!=\!\sigma^{-2^2}(12)$ becomes the new search 
administrator. Eventually, the binary search halts at vertex $2$ ({\it i.e.,} the leader), 
so it discovers itself twice.

\subsubsection{Complexities of The Distributed Binary Search}\label{subsubsec:comp-bs}

The time complexity ({\it i.e.,} number of iterations) of the distributed binary search 
is upper-bounded by $\lceil\log_2 \eta\rceil$ ($\le\! \log_2 N$) iterations, where $\eta$ is the length of the longest non-ouroboros cycle. 
\addedHL{Hence, it can be as large as $\log_2 N$ iterations, each of which contains roughly $3$ operations ($2$ additions and $1$ comparison), in the worst case.} 

In the distributed binary search, the average number of additional iterations is, however, much smaller than $\log_2 N$ for the following reason.   It takes practically no time 
for a search administrator $i$ to narrow the search interval to the smallest precinct right-ended at $i$, since $i$ can remember this information 
(when the vertex with the smallest identity among those ``seen" so far first becomes a precinct leader) during the SERENADE-common iterations.
Hence, a unit of time complexity is incurred only when the search administrator has to move from one vertex to another, which happens often much less than 
$\lceil\log_2 \eta'\rceil$ on a non-ouroboros cycle of length $\eta'$.  
\addedHL{For example, the average time complexity as a function of $N$,
when $\sigma$ is a uniform random permutation, 
varies narrowly between $0.46 \log_2 N$ and $0.48 \log_2 N$, 
for $N \!\in\! \{ 64, 128, 256, 512, 1024\}$. 
Therefore, we consider E-SERENADE to be $1.5$ times more expensive empirically, in terms of time complexity, than C-SERENADE and O-SERENADE.}

%(\autoref{code: intermediate-passing} in \autoref{alg: serenade-bsearch}) 

\addedHL{As explained in~\autoref{subsubsec: b-search}, 
during the binary search process, on each non-ouroboros cycle a message 
(to maintaining the weight information) 
is transmitted only when the search administrator moves from one vertex to another, 
so the message complexity of the binary search process, in the worst-case, 
is $1$ message per vertex.
It can be
shown that the average additional message complexity per vertex is bounded by $O(\frac{\log^2 N}{N})$, which is even smaller asymptotically. } 

% \subsubsection{``Bookkeeping" the Weight Information}\label{subsubsec: bookkeep}  
% \modifiedHL{We highlight the following important invariant this binary search algorithm maintains.
% Whenever a vertex (say $\sigma^u(\mathcal{L}_0)$) becomes the new search administrator,
% the search algorithm maintains the red and the green weights of the walk
% $\mathcal{L}_0\leadsto\sigma^u(\mathcal{L}_0)$.  This way, when the search administrator finally reaches a repetition of $\calL_0$ (say $\sigma^v(\calL_0)$ ), 
% we have also obtained the red and the green weights of the walk $\mathcal{L}_0\leadsto\sigma^v(\mathcal{L}_0)$.   
% Comparing these two weights allows us to tell precisely whether the green weight or 
% the red weight of the cycle is heavier because, the walk $\mathcal{L}_0\leadsto\sigma^v(\mathcal{L}_0)$  
% coils around the cycle for an integer number of times (since the endpoint $\sigma^v(\mathcal{L}_0)$ is a repetition of 
% the starting point $\calL_0$).}




%% remarks

% \subsubsection{Registration Requirement} 
% \modifiedHL{Note that the leader of each non-ouroboros cycle needs to ``register" its identity with the switch controller, at the end 
% of the leader-election-augmented 
% knowledge-discovery procedure. The leader informs the switch controller, of its determination (as to which sub-matching is heavier)
% only after the %collaborative 
% distributed binary search completes on the non-ouroboros cycle. As mentioned above, 
% The switch controller then broadcasts the aforementioned list of leaders and their determinations to all vertices only after hearing from all ``registered" leaders.  
% The ``registration" process is important for minimizing the average additional delay of E-SERENADE because, without it, the switch would have to 
% conservatively wait the maximum amount of time it would possibly take for 
% the distributed binary search process to complete on every non-ouroboros cycle.}  
================{\bf Stop Here}=================

\section{Approximation}
\label{subsec: o-serenade}

In the previous sections, we show that SERENADE can make full 
of the knowledge sets each vertex learned during the knowledge discovery to let every vertex makes the exact same 
decision as it would in SERENA. However, the cost is up to $\log_2N$ additional iterations of a distributed binary 
search. In this section, we present an approximation version to SERENADE without the distributed binary search, in which 
vertices on any such non-ouroboros cycle make a
decision based on the (insufficient) information at hand after the augmented knowledge-discovery stage. 

\medskip
\noindent
{\bf Decision Rule.}
The decision rule of this approximation is for the leader $\calL_0$ on this cycle to compare the green
and the red weights of the longest such walk 
$\calL_0\!\leadsto\!\sigma^N(\calL_0)$,
and pick, on behalf of the whole cycle, the green or the red matching according to the outcome of this comparison; note we cannot simply let every vertex $i$ on this cycle to pick the green or the red 
edge individually based on its local view (of $w_r\big{(}i\leadsto\sigma^N(i)\big{)}$ vs. $w_g\big{(}i\leadsto\sigma^N(i)\big{)}$) since these local views can be inconsistent as we have shown in~\cite{Gong2017arXivSERENADE}. [{\bf Add the example back if having enough space eventually}] Note that like SERENADE, this approximation also needs the switch controller to broadcast the decisions of all the leaders to the $N$ vertices.
% This strategy is opportunistic as it does not hesitate to pick 
% a sub-matching that appears to be larger, even though there is a small chance this appearance is incorrect.  
% Empirically this strategy performs better than the 
% conservative strategy of C-SERENADE (as we will show in~\autoref{sec:evaluation}), for the following reason.}

\medskip
\noindent
{\bf Rationale.}
The rationale behind the heuristic decision rule is as follows. 
When the weight difference between the red and the
green sub-matchings is small, 
it matters little which sub-matching
is picked.  When the difference is large, however, this ``longest ouroboros walk'' likely will further inflate the already large difference and hence result in the correct sub-matching being picked. 






==> sections/serenade-algorithms/c_serenade.tex <==
\section{The SERENADE Variants}
\label{sec: serenade-algorithms}

In this section, we describe in detail the three 
%(pure) 
variants of SERENADE, namely C-SERENADE (\autoref{subsec: c-serenade}), O-SERENADE (\autoref{subsec: o-serenade}), and E-SERENADE (\autoref{subsec: E-serenade}).
%(\autoref{subsec: c-serenade})
%For each variant,
% focus on their operations during an arbitrary time slot $t$, 
%We again assume that the ``union-ed" permutation
%during an arbitrary time slot is $\sigma$.  
Recall that E-SERENADE emulates SERENA exactly, and C-SERENADE and O-SERENADE do so approximately.  
\modifiedHL{As explained earlier, 
%Recall that if the ``union-ed" permutation 
% \deletedHL{if the ``union-ed" permutation $\sigma$ happens to be {\it ouroboros}, all input ports will find out this fact during or after executing the $1 + \log_2 N $ 
% iterations of %the SERENADE common stage, 
% SERENADE-common,
% %and no further communication is needed (\ie mission accomplished) beyond this point 
% %because the input ports already have sufficient information
% %to 
% %individually simultaneously [need to explain that = collective decision] earlier
% and decide on the same ``merged"
% matching $S$ as they would under SERENA (given the same $\sigma$). 
% %However, more often than not, this ouroboros situation does not happen (see row ? of Table ?), and in this case
% Otherwise,} 
input ports on any {\it non-ouroboros cycle} do not know for sure, 
 % at this point, 
after executing the $1 + \log_2 N $ 
iterations of %the SERENADE common stage, 
SERENADE-common, 
between the
red or the green sub-matchings that collapse into the cycle, which one is heavier.} 
The three variants of SERENADE branch off from this point onwards.

Note that the switch has the freedom to choose, for each time slot, which SERENADE variant is to be used.
If the switch intends to exercise this freedom, however, the switch controller needs to inform all input ports of its choice at the beginning of the time slot;
or all input ports will execute the pre-determined default SERENADE variant.
This freedom makes possible the aforementioned hybrid variants such as ``mixing $1\%$ E-SERENADE with $99\%$ C-SERENADE," which we will
motivate and elaborate on in \autoref{sec: stabilization}.

\subsection{C-SERENADE}\label{subsec: c-serenade}
In C-SERENADE, %(C for conservative), 
input ports on any such non-ouroboros cycle will each make an individual
decision at this point (\ie without any additional communication and/or computation), according to the following simple rule:  
any input port on this non-ouroboros cycle will
stay with the green sub-matching (the one used for the previous time slot)
and pair again with the output port it paired with in the previous time slot.  The logic behind this decision rule is a conservative 
one:  these input ports ``stay put" unless they are certain that the alternative is better ({\it i.e.}, the red sub-matching is heavier).
%-- based on the (insufficient) information at hand -- that 
Clearly, the final matching resulting from these individual decisions may or may not be the same as
the input ports would decide on under SERENA.   



==> sections/serenade-algorithms/complexities_serenade_variants.tex <==
\subsection{Complexities of SERENADE Variants}
\label{subsec: complexity-variants}



%% handle counter issues
\newcounter{savefootnote}% Get current counters
\setcounter{savefootnote}{\value{footnote}}% Store footnote counter
\stepcounter{savefootnote} %% increase the counter
\setcounter{footnote}{\value{savefootnote}}% write back footnote counter
%% please make sure the above several lines
%% appear before the following table
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htb]
\centering\caption{Complexities of SERENADE variants.}\label{tab: complexities}
\begin{tabular}{@{}*{4}{c}@{}}
\toprule 
 & Iterations & Message complexity per vertex \\ \midrule
C-SERENADE &   $1 + \log_2 N$    & \addedHL{$O(\log N)$ messages} \\ \midrule
O-SERENADE &  \addedHL{$2 + \log_2 N$}    & \addedHL{$O(\log N)$  messages} \\ \midrule
E-SERENADE &  \addedHL{$2 + 2 \log_2 N$} & \addedHL{$O(\log N)$ messages} \\ 
\bottomrule
\end{tabular}
\end{table}

%\footnotemark[\value{savefootnote}] 
%\footnotetext[\value{savefootnote}]{Note that, O-SERENADE and E-SERENADE need a broadcast (per cycle) to distribute 
%the decision of the leader to all nodes in the corresponding cycle, whereas C-SERENADE does not.}


%roughly\footnote{We do not use the ``big $O$" notation here to emphasize the constant factor $1$.} 

\modifiedHL{Recall (from \autoref{subsec: complexity-common}) that SERENADE-common has a time complexity of $1\! +\! \log_2 N$ iterations, each of which involves 
several CPU instructions, 
and a message complexity of $O(\log N)$ messages per vertex.
%$O(N \log N)$ messages, or 
In this section, we analyze the time and the message complexities, including those of SERENADE-common,  
of the three SERENADE variants.  They are summarized in \autoref{tab: complexities} where the time complexity is shown in number of iterations;  the rough CPU instruction counts in each iteration
will also be provided below.  Note the asymptotical message complexities of all three SERENADE variants are $O(\log^2 N)$ when measured in number of bytes, as 
each message is $O(\log N)$ bits in length.   
Their numerical values under various switch sizes $N$ are shown 
later in this section.}
%\addedHL{We will show more detailed numerical message complexity later in this section.}

%\medskip
%\noindent
\subsubsection{C-SERENADE and O-SERENADE}  \modifiedHL{C-SERENADE incurs no additional time and message complexities, as it makes a conservative 
decision right after the execution of SERENADE-common, so its total time complexity is the same as SERENADE-common's.  Almost the same can be said about O-SERENADE:  The additional message complexity 
is that for the leaders of non-ouroboros cycles (typically a tiny number as explained earlier) to report their respective decisions to the switch controller
% \deletedHL{is nearly a constant (see the third paragraph of \autoref{subsubsec: o-decision-rule}),}
plus a broadcast of these decisions, and the additional time 
complexity is just $1$ iteration.   However, since O-SERENADE requires a leader election process to be embedded in SERENADE-common iterations, it increases the time complexity of each SERENADE-common iteration
by at most $2$ CPU instructions (for comparing the identities of two precinct leaders and recording the winner), and the message complexity by $\log_2 N$ bits (for encoding the precinct leader).  
%involves $1$ additional comparison in every iteration except the $0^{th}$, its total time complexity is $1 + 3\log_2 N$ ALU instructions.  
%This leader election process also introduces $\log_2 N$ bits of additional message complexity per input port to each 
%iteration of SERENADE-common. 
%However, since O-SERENADE requires leader election, every message
%exchange in SERENADE-common has to include the identity of a precinct leader, which increases a length of each message 
%by $\log_2 N$ bits.  
We will show in \autoref{subsec:performance-results} that such tiny time and message overheads are a modest cost to pay for the significantly better delay performance than
that of C-SERENADE.}

%The actual increase in systems overhead due to this larger message size is much smaller in practice though, since the
%fixed cost of sending and receiving a message 

%and an extra bit as the overweight indicator in the case of COW (Conservative if OverWeight) extension,

%In E-SERENADE, the time complexity of the binary search process (for a repetition of its leader) on a non-ouroboros cycle is measured by the number of times the  
%search administrator moves from one vertex to another.
%since, as explained in Appendix ..., it takes ``no time" for a  search administrator $i$ to narrow the search interval to the smallest precinct right-ended at $i$.   

%\medskip
%\noindent
\subsubsection{E-SERENADE}  In E-SERENADE, due to the binary nature of the search (for a repetition of its leader on every non-ouroboros cycle), the additional time complexity 
is upper-bounded by $\lceil\log_2 \eta\rceil$ ($\le\! \log_2 N$) iterations, where $\eta$ is the length of the longest non-ouroboros cycle. 
\addedHL{Hence, it can be as large as $\log_2 N$ iterations, each of which contains roughly $3$ CPU instructions ($2$ additions and $1$ comparison), in the worst case.} 
%Therefore, the worst-case total time complexity of E-SERENADE is $1 + 6\log_2 N$ ALU instructions.

%The worst-case additional time complexity of E-SERENADE is the largest among those of all non-ouroboros cycles, and hence upper-bounded by $\log_2 N$.  
In E-SERENADE, the average number of additional iterations is, however, much smaller than $\log_2 N$ for the following reason.   It takes practically no time 
for a search administrator $i$ to narrow the search interval to the smallest precinct right-ended at $i$, since $i$ can remember this information 
(when the vertex with the smallest identity among those ``seen" so far first becomes a precinct leader) during the SERENADE-common iterations.
Hence, a unit of time complexity is incurred only when the search administrator has to move from one vertex to another, which happens often much less than 
$\lceil\log_2 \eta'\rceil$ on a non-ouroboros cycle of length $\eta'$.  
%when there is a repetition of the leader in the right half of the search interval, the search interval is halved (to become the right half) but the same search administrator 
%stays on, which incurs almost zero time complexity.  
\addedHL{For example, the average time complexity as a function of $N$,
% (obtained through Monte-Carlo simulation 
%due to its lack of close-form probability distribution), 
when $\sigma$ is a uniform random permutation, 
% is shown in the last row of \autoref{tab: ouroboros_statistic}.  It 
varies narrowly between $0.46 \log_2 N$ and $0.48 \log_2 N$, 
% for these values of $N$. 
for $N \!\in\! \{ 64, 128, 256, 512, 1024\}$. 
Therefore, we consider E-SERENADE to be $1.5$ times more expensive empirically, in terms of time complexity, than C-SERENADE and O-SERENADE.}

%(\autoref{code: intermediate-passing} in \autoref{alg: serenade-bsearch}) 

\addedHL{As explained in~\autoref{subsec: E-serenade}, 
during the binary search process, on each non-ouroboros cycle a message 
(to ``bookkeeping'' the weight information) 
is transmitted only when the search administrator moves from one vertex to another, so the additional message complexity of E-SERENADE, in the worst-case, 
is $1$ message per vertex.
%Since each vertex receives and transmits at most one message each 
%during the binary search process, the total additional message complexity of E-SERENADE, in the worst-case, is bounded by $O(N)$.  This message complexity is 
%small compared to that of SERENADE-common, which is $O(N\log N)$.  
It can be
shown that the average additional message complexity per vertex is bounded by $O(\frac{\log^2 N}{N})$, which is even smaller asymptotically. } 

%\medskip
%\noindent
\subsubsection{Numerical Values of Message Complexities} \label{subsubsec:detailed-msg-complexity}
\addedHL{
%Now, we investigate the detailed message complexity of SERENADE. 
The numerical values of  
the worse-case message complexities (in bytes) of the three SERENADE variants, under various switch sizes $N$, are shown in~\autoref{tab: msg-complexities}. 
%For comparison, also shown~\autoref{tab: msg-complexities} are those of iSLIP, whose message complexity is precisely $N$ bits per port (for indicating whether any of the $N$ VOQs is empty or not).  
%Clearly, the message complexities of all three variants become smaller than iSLIP when $N$ is 256 or larger.  
%As explained earlier, the message complexity of C-SERENADE is identical to that of SERENADE-common.
Note that in every SERENADE-common message, it suffices to include only $w_r(\bigdot) - w_g(\bigdot)$, the difference between the red and 
the green weights of the corresponding walk. This difference can be encoded in $15$ bits (with a single ``sign'' bit), as we assume that each weight can fit in
$14$ bits ({\it i.e.,} no more than 16,384 packets).  
% in each VOQ). 
Hence for C-SERENADE, each message is $15 + \log_2 N$ bits in length, where
these $\log_2 N$ bits are used to encode the identity of the vertex in the corresponding knowledge set.  In O-SERENADE, each message on average is 
$0.5 \log_2 N$ bits longer (for encoding the ``precinct leader'' information in every other message) than that. 
The worst-case message complexity of E-SERENADE per vertex is a couple of bytes higher than that of O-SERENADE, due to the message exchanges during the 
distributed binary search process.  
Note that the numbers 
in~\autoref{tab: msg-complexities} do not include the 
broadcast cost (paid by the switch controller) in O-SERENADE and E-SERENADE (there is no broadcast in C-SERENADE).  
As mentioned in~\autoref{subsec: o-serenade}, although the worst-case broadcast cost is $N$ bits, 
the average cost is much smaller ({\it e.g.}, no more than $2.667 (\log_2 N + 1)$ bits for $N \le 1,024$) and negligible compared to the corresponding value in~\autoref{tab: msg-complexities}. 

We acknowledge that the message complexity of SERENADE is nontrivial.  Indeed, this message overhead can be viewed as ``bandwidth lost'':
given a fixed packet length of $\alpha$ bytes and a message overhead of $\beta$ bytes, each input port could transmit $\frac{\beta}{\alpha}+1$ times more actual network traffic per switching cycle, 
if the message overhead were instead $0$.
However, this nontrivial message overhead does not dent the theoretical and the practical contributions of SERENADE for three reasons.

First, this message overhead, viewed as a throughput performance bottleneck, is a different than and independent of the bottleneck caused by the (high) time complexity of the 
switching algorithm:  the former is characterized by $\frac{\beta}{\alpha}$ whereas the latter is characterized by how short a switching cycle can be.     
%Consider the scenario that an ultra-high-speed switch in which each input port transmits 100 million packets
%per second (i.e., each switching cycle is $10$ nanoseconds long) operates in a network environment in which the packet length is large (say 1,000 bytes per packet).
%With its low time complexity, SERENADE makes it possible to 
The primary contribution of SERENADE is to remove the latter bottleneck.  
Second, studies on packet length statistics of both Internet and data center traffic~\cite{Sinha2007InternetPacketSize,Benson2010DCTraffic,Roy2015FBDC} 
show that large packets generally have a much larger total byte count than small packets.  
For example, as measured in~\cite{Roy2015FBDC}, around $60\%$ packets of the Hadoop traffic are of MTU length 
({\it i.e.,} 1,500 bytes for the network environment studied in~\cite{Roy2015FBDC}).  Hence we can make $\alpha$ quite large (say $\alpha \!=\! 512$) without wasting much link bandwidth due to ``shipping'' a short (variable-length) packet in an $\alpha$-byte-long
(fixed-length) packet (``container''),
and the message overhead ratio becomes quite small when such a large $\alpha$ is used.  Furthermore, even in the worst case that the average (variable-length) packet length is small, multiple such packets can be packed into
a long fixed-length packet so that the bandwidth waste is minimized.  Third, SERENADE does not stand out, among parallel iterative switching algorithms, as having the highest message overhead.
For example, the message complexity of iSLIP is precisely $N$ bits per port (for indicating whether each of its $N$ VOQs is empty or not)~\cite{McKeown99iSLIP}, which is comparable to or higher than those of 
SERENADE variants when $N \ge 512$.
}

\begin{table}
\centering\caption{Per-port message complexity of SERENADE (bytes).}\label{tab: msg-complexities}
\input{tables/message_complexity_detail}
\end{table}

==> sections/serenade-algorithms/e_serenade.tex <==
%\subsection{Exact Merge Decisions: E-SERENADE}
\subsection{E-SERENADE}
\label{subsec: E-serenade}

Whereas in C-SERENADE and O-SERENADE, each non-ouroboros cycle picks a sub-matching, which may or may not be the heavier one, 
right after the SERENADE-common's  
$1 + \log_2  N$ iterations, in E-SERENADE, vertices on each non-ouroboros cycle execute an additional distributed algorithm to find out
{\it exactly} which sub-matching is heavier.  
Like O-SERENADE, E-SERENADE requires that all $1 + \log_2  N$ SERENADE-common iterations be augmented with leader election.
%(described in \autoref{subsec: leader-election}).  
Recall that, for a vertex $i$ on a non-ouroboros cycle, the ``final product" of the leader election process is 
$\calL(\sigma^{-N}(i)\leadsto i)$,
the leader of the level-$(\log_2 N)$ precinct right-ended at $i$, which is also $\calL_0$, the leader of the entire cycle.   However, during this process, 
$i$ also obtains, as ``intermediate products", the identities of the leaders of level-$k$ precincts right-ended at $i$, {\it i.e.,} $\calL(\sigma^{-2^k}(i)\leadsto i)$ for $k = 0,1,\cdots,\log_2(N)-1$.  We will 
show next that whereas in O-SERENADE only the ``final product" is used, in E-SERENADE, all ``intermediate products" will also be put to full use.  

\subsubsection{Distributed Binary Search}\label{subsubsec: b-search}  It suffices to describe this distributed algorithm on an arbitrary non-ouroboros cycle,
since every non-ouroboros cycle runs an (distinct) instance of the same
algorithm.  Hence, without loss of generality, we assume that $\calL_0$ is the leader of, and $i$ a
vertex on, this non-ouroboros cycle.  The objective of this distributed algorithm is to search for a
{\it repetition} (\ie other than its first occurrence as the starting point of the walk) of its leader $\calL_0$ along the walk %from $\mathcal{L}_c$ to $\sigma^N(\mathcal{L}_c)$.
$\mathcal{L}_0\!\leadsto\!\sigma^N(\mathcal{L}_0)$, the level-($\log_2 N$) precinct right-ended at $\sigma^N(\mathcal{L}_0)$;  this repetition must exist
because $N$, the length of the walk $\mathcal{L}_0 \leadsto \sigma^N(\mathcal{L}_0)$, is no smaller than
the length of this cycle.   
\modifiedHL{To this end, vertices on this non-ouroboros cycle perform a distributed binary search, guided by the
aforementioned ``intermediate" and ``final products" %(\ie the identities of the level-$0$ to level-$N$ precinct leaders right-ended at $i$) 
each vertex obtains through the leader
election process.} \addedHL{In the following, we describe the high-level ideas of this binary search algorithm while referring readers to~\cite{Gong2017arXivSERENADE} for its pseudocode and detailed
descriptions.}

This binary search is initiated by the vertex
$\sigma^{N}(\calL_0)$, who learns ``who herself is" (\ie that herself is $\sigma^{N}(\calL_0)$) during the last iteration
of SERENADE-common;  in other words, the initial {\it search administrator} is $\sigma^{N}(\calL_0)$.
The initial {\it search interval} is the entire walk $\calL_0\leadsto\sigma^{N}(\calL_0)$, also the level-$(\log_2 N)$ precinct right-ended at $\sigma^{N}(\calL_0)$.
%, which consists of $N$ edges (\ie is of length $N$).  
The search administrator $\sigma^{N}(\calL_0)$ first checks whether there is a repetition of $\calL_0$ in the right half of the search interval (\ie the walk
$\sigma^{-N/2}(i)\leadsto i$) by checking whether
$\calL(\sigma^{N/2}(\calL_0)\leadsto\sigma^{N}(\calL_0))$ is equal to $\calL_0$;  note the identity of $\calL(\sigma^{N/2}(\calL_0)\leadsto\sigma^{N}(\calL_0))$, 
the leader of the level-$(\log_2 (N) - 1)$ precinct right-ended at $\sigma^{N}(\calL_0)$,
is known to $\sigma^{N}(\calL_0)$, since it is one of the aforementioned ``intermediate products" $\sigma^{N}(\calL_0)$ learns through the leader election
process.
If so, the same search administrator $\sigma^{N}(\calL_0)$ carries on this binary search in the right half of the search interval.  
Otherwise, the ``middle point" of the search interval $\sigma^{N/2}(\calL_0)$ becomes the new search administrator and carries on this binary search in the left half.  
%Clearly, it takes at most $\log_2 N$ steps for this binary search to end (with finding a repetition of $\calL_0$).
%This way, with each step of this binary search, the search interval is halved (and becomes a precinct that is one level lower), 
%and if needed, a different vertex that is at least twice as close to the target becomes the new search administrator.


\subsubsection{``Bookkeeping" the Weight Information}\label{subsubsec: bookkeep}  
% In the interest of space, we defer the details of this binary search algorithm to \autoref{subsubsec: repetition-search}. 
%[{\bf The following line maybe to be removed}] 
%We will provide the details of this binary search algorithm later in \autoref{subsubsec: repetition-search}.
\modifiedHL{We highlight the following important invariant this binary search algorithm maintains.
Whenever a vertex (say $\sigma^u(\mathcal{L}_0)$) becomes the new search administrator,
the search algorithm maintains the red and the green weights of the walk
$\mathcal{L}_0\leadsto\sigma^u(\mathcal{L}_0)$.  This way, when the search administrator finally reaches a repetition of $\calL_0$ (say $\sigma^v(\calL_0)$ ), 
we have also obtained the red and the green weights of the walk $\mathcal{L}_0\leadsto\sigma^v(\mathcal{L}_0)$.   
Comparing these two weights allows us to tell precisely whether the green weight or 
the red weight of the cycle is heavier because, the walk $\mathcal{L}_0\leadsto\sigma^v(\mathcal{L}_0)$  
coils around the cycle for an integer number of times (since the endpoint $\sigma^v(\mathcal{L}_0)$ is a repetition of 
the starting point $\calL_0$).}

%% remarks

\subsubsection{Registration Requirement} 
\modifiedHL{Like in O-SERENADE, the leader of each non-ouroboros cycle needs to ``register" its identity with the switch controller, at the end of the leader-election-augmented 
SERENADE-common.  However, unlike in O-SERENADE, the leader informs the switch controller, of its determination (as to which sub-matching is heavier)
only after the %collaborative 
distributed binary search completes on the non-ouroboros cycle.  
The switch controller then broadcasts the aforementioned list of leaders and their determinations to all vertices only after hearing from all ``registered" leaders.  
The ``registration" process is important for minimizing the average additional delay of E-SERENADE because, without it, the switch would have to 
conservatively wait the maximum amount of time it would possibly take for 
%``long enough" (the amount of time to make sure that 
the distributed binary search process to complete on every non-ouroboros cycle.}  

%\input{sections/appendix-sections/e_serenade_bisearch}






==> sections/serenade-algorithms/o_serenade.tex <==
%\subsection{Opportunistic Merge Decisions: O-SERENADE}
\subsection{O-SERENADE}
\label{subsec: o-serenade}


% \begin{figure}
% \centering
% \CyclewithWeights
% \caption{The $3^{rd}$ cycle (from left to right) in \autoref{fig: cycles-in-permutation} augmented with weights.}
% \label{fig: cycle-with-weights}
% \end{figure}

% [Long, need to say somewhere that $N$ is assumed to be a 2's power]

In O-SERENADE, input ports on any such non-ouroboros cycle also have to make a
decision based on the same (insufficient) information at hand as in C-SERENADE. \modifiedHL{Recall every vertex $i$ on
this cycle knows the green and the red weights of the walk $i\leadsto \sigma^\eta(i)$, for every
$\eta \le N$ that is a power of $2$.}
% an ouroboros number.  

\subsubsection{Decision Rule}
\label{subsec: o-decision-rule}


\modifiedHL{The decision rule of O-SERENADE is for a designated vertex $\calL_0$ on this cycle to compare the green
and the red weights of the longest such walk
% \footnote{Recall also that $N$ is an ouroboros number since it is assumed to be a power of $2$.}
$\calL_0\!\leadsto\!\sigma^N(\calL_0)$,
and pick, on behalf of the whole cycle, the green or the red matching according to the outcome of this comparison;  note we cannot simply let every vertex $i$ on this cycle to pick the green or the red 
edge individually based on its local view (of $w_r\big{(}i\leadsto\sigma^N(i)\big{)}$ vs. $w_g\big{(}i\leadsto\sigma^N(i)\big{)}$) since these local views can be inconsistent as we have shown in~\cite{Gong2017arXivSERENADE}. 
This strategy is opportunistic as it does not hesitate to pick 
a sub-matching that appears to be larger, even though there is a small chance this appearance is incorrect.  Empirically this strategy performs better than the 
conservative strategy of C-SERENADE (as we will show in~\autoref{sec:evaluation}), for the following reason.}
\addedHL{
When the weight difference between the red and the
green sub-matchings is small, 
it matters little which sub-matching
is picked.  When the difference is large, however, this ``longest ouroboros walk'' likely will further inflate the already large difference and hence result in the correct sub-matching being picked.}

% [move to SERENADE-common where we talked about power of 2]
% For example, if $N$ is not a power of 2, we simply run $\lceil\log N\rceil + 1$ iterations in SERENADE-common.

\deletedHL{
\subsubsection{A Flawed Decision Rule and Its Fix}\label{subsubsec: o-decision-rule}

%We will show shortly that, like in C-SERENADE,
%the node $i$ may not always pick the correct ``color."

This tentative decision rule is however flawed because, for two distinct vertices $i_1$ and $i_2$ on a non-ouroboros cycle, it is possible that 
$w_g(i_1\leadsto\sigma^N(i_1)) \ge w_r(i_1\leadsto\sigma^N(i_1))$ (so $i_1$ picks the green edge) %and 
yet $w_g(i_2\leadsto\sigma^N(i_2)) < w_r(i_2\leadsto\sigma^N(i_2))$ (so $i_2$ picks the red edge).  In other words, $i_1$ and $i_2$
have {\it inconsistent local views} as to which sub-matching is heavier.
%$i_1$  the green weight of the walk ... can be 
%larger than its red weight, whereas 
%different input ports  could pick edges of different colors based on the same decision rule,
It is not hard to check that, 
in this case, at least two distinct input ports (not necessarily $i_1$ and/or $i_2$) on this non-ouroboros cycle would be paired with the same output port,
resulting in a configuration collision.
% (\ie two input ports being paired with the same output port).  
%Note that, unlike the case of C-SERENADE, O-SERENADE cannot let each vertex $i$ on a non-ouroboros cycle independently makes a decision based on its ``local knowledge sets". %This is because two different vertices on the same non-ouroboros cycle, whose $N$-edge-long walks have different ``remainder sections", could pick two sub-matchings (edges) of %opposite colors.
%For example, as shown in 

\autoref{fig: cycle-with-weights} shows an example of such inconsistent local views:  
%vertices $3$ and $4$ have ``inconsistent local views":
%input port 3 will pick the green edge because 
$w_g\big{(}3\leadsto\sigma^8(3)\big{)} \!=\! 18 \!<\! 20 \!=\! w_r\big{(}3\leadsto\sigma^8(3)\big{)}$ (vertex $3$'s local view) and
%input port 4 will pick the red edge because 
$w_g\big{(}7\leadsto\sigma^8(7)\big{)} \!=\! 23 \!>\! 18 \!=\! w_r\big{(}7\leadsto\sigma^8(7)\big{)}$ (vertex $7$'s local view).  Although the inconsistent local views
here do not result in a 
configuration collision because the cycle $(3, 4, 7)$ is ouroboros ($3$ is an ouroboros number), they would in a non-ouroboros cycle.  Note that, as mentioned earlier, 
since the smallest non-ouroboros number is $19$ %(see remarks after ...), 
(when $N\geq 64$ and is a power of $2$), 
a more qualified example involving a non-ouroboros cycle would be unnecessarily large and complex to plot here.
}

%Note this example is aimed at illustrating the possible inconsistency issue of the decision rule used by O-SERENADE. However, in the specific example, we would not have
%this issue since $3=2^2-2^1$ is ouroboros. We choose this example because the smallest non-ouroboros number is $19$, which will make the example too complex. }.
%Using the same example as above, if making decision based on the longest
%walk, the input port $4$ would choose red, while input port $3$ would choose green.
%In this case, two input ports attempt to transmit to the same output port, resulting in a collision.


% We will show in \autoref {subsec: leader-election} t
\modifiedHL{In O-SERENADE, this designated vertex $\calL_0$ is decided through a distributed leader
election~\cite{Lynch1996Distributed} by the vertices on this cycle.  
% which we will describe shortly in~\autoref{subsec: leader-election}.
Although distributed leader election is in general a relatively expensive operation~\cite{attiya2004distributed,Lynch1996Distributed}, 
%for example, the algorithm proposed in~\cite{attiya2004distributed} takes $O(N)$ rounds in a synchronous ring with knowing the ring size $N$, 
it is much less so in O-SERENADE, since leader 
election on each non-ouroboros cycle can be seamlessly embedded into the $1 + \log_2 N$ iterations of SERENADE-common, and leader elections on distinct non-ouroboros cycles 
can be computed in parallel, as we will show shortly in~\autoref{subsec: leader-election}.
%% cite Radia Perlmann's bridge book
Once the leader of a non-ouroboros cycle is decided, the leader $\calL_0$ informs the switch controller of its decision on whether to choose the green or the red sub-matching.} 
% The switching controller then broadcasts a list of leaders, one for each non-ouroboros cycle, and their decisions to all $N$ vertices.

\modifiedHL{The size of this broadcast, equal to the number of {\it non-ouroboros} cycles in a permutation, is small (with overwhelming probability).
For example, even when $N = 1,024$, the average 
number of non-ouroboros cycles is only $2.667$ for a uniform random permutation.
Since each vertex on a non-ouroboros cycle knows the identity of its leader, as we will ``prove" in~\autoref{subsec: leader-election},
it will follow the decision made by its leader in choosing between the red and the green edges.} \addedHL{Note that when there are many non-ouroboros cycles, albeit is rare 
empirically, the above broadcast approach would not scale. Under such a case, 
the switch controller, after getting the decisions from all the leaders, can simply 
broadcast a bitmap with length $N$. The $i^{th}$ bit equals $1$ indicates that 
the vertex $i$ picks the red sub-matching, otherwise, the green sub-matching is 
picked by $i$. Clearly, this broadcast scheme, costing more bits when there are 
few non-ouroboros cycles, has a fixed size of $N$ bits and every vertex on 
a non-ouroboros cycle can read its leader's decision in one operation.}


%Intuitively, this is because, for this number to be large, there has to be many short cycles, but all short cycles (up to length $22$ when $N = 1,024$) are ouroboros.

\deletedHL{The switching controller then simply broadcasts a bitmap with a length of $N$, in which 
the $i^{th}$ bit is the decision of the leader with identity $i$, {\it i.e.,} ``0'' means 
it selects the green submatching, otherwise it selects the red submatching\footnote{\addedHL{Instead of 
using a bitmap with a length of $N$, the switching controller can also broadcast a list of 
leaders, one for each non-ouroboros cycle, 
and their decisions. By doing so, we can reduce the broadcast size significantly, since the 
number of non-ouroboros cycles is very small. For example, even when $N = 1,024$, the average 
number of non-ouroboros cycles is only $2.667$ for a uniform random permutation.}}.} 

\deletedHL{
The size of this broadcast, equal to the number of {\it non-ouroboros} cycles in a permutation, is small (with overwhelming probability), 
as shown in the fourth row of 
\autoref{tab: ouroboros_statistic} for a uniform random permutation (same for other random permutations as observed in our simulation results).
For example, even when $N = 1,024$, the average broadcast size is only $2.667$.  
%\glong{Empirically, this average broadcast size is bounded by $O(\log N)$.}  
%An  intuitive explanation of why this (average) number is so small 
%is that, 
Intuitively, this is because, for this number to be large, there has to be many short cycles, but all short cycles (up to length $22$ when $N = 1,024$) are ouroboros.

%% move from Section An Idempotent Trick
% [{\bf Maybe, we should swap the order of the following two paragraphs.}]
This solution solves the {\it decision consistency problem} of O-SERENADE:  It guarantees that all vertices on a non-ouroboros cycle make a consistent decision 
(by picking the same sub-matching).
However, like in C-SERENADE, there is no guarantee that the final decision results in the heavier sub-matching of the cycle being chosen, so O-SERENADE also 
emulates SERENA only approximately.
%correct (with probability $1$) in the sense the heavier sub-matching is always
%picked. 
%\textbf{Note that, the results from C-SERENADE and O-SERENADE are feasible matchings but might have lower weight than that from SERENA.}  
%\footnote{This is not a shortcoming of O-SERENADE:  No decision rule can
%guarantee, with the limited amount of knowledge obtained at this point (to be elaborated on in~\autoref{sec: making_do}), the correctness of the decision.}.
% which as explained in \autoref{sec: serenade-algorithms} should be expected. 
%For example, in \autoref{fig: cycle-with-weights}, 
%vertex $3$ is the leader of the cycle (to be consistent with the 
%leader election rule described next in~\autoref{subsec: leader-election}), and its determination that the red sub-matching is heavier (due to  $w_g(3\leadsto\sigma^8(3))<w_r(3\leadsto\sigma^8(3))$) is not correct.  
However, empirically the heavier sub-matching is chosen most of the time, 
as we will show and explain why in~\autoref{subsec:performance-results}. 
%, and usually is incorrect only when the green and the red weights of the cycle are very close to each other, in which case the ``damage" (to the total weight of the final matching) caused by this incorrect decision is tiny anyway. 
An alternative solution used in~\cite{ModianoShahZussman2006DistSched} to this {\it decision consistency problem} is described
and compared with 
% in~\autoref{subsubsec: idempotent}.
in~\cite{Gong2017arXivSERENADE}. 
}
%\glong{We emphasize this is not a shortcoming of O-SERENADE:  With the limited amount of information each vertex has after the $1 + \log_2 N$ iterations of SERENADE-common, apparently no decision rule can
%guarantee the correctness (with probability $1$) of the decision.}  

\subsubsection{Leader Election}
\label{subsec: leader-election}

\addedHL{Now we describe 
%the leader election process in O-SERENADE.
% As explained earlier, O-SERENADE does not have to pay much extra for running this leader election:
% The election process can be seamlessly embedded into the $1+ \log_2 N$ knowledge-discovery iterations of SERENADE-common.
% More specifically, 
how to embed the leader election process into the $1\!+\! \log_2 N$ 
knowledge-discovery iterations of SERENADE-common.   
%each of the $2(1+ \log_2 N)$ messages transmitted in SERENADE,
We explain this process on an arbitrary non-ouroboros cycle, 
focusing on the actions of a 
vertex $i$ that belongs to this cycle.  
We follow the standard 
%leader-designation 
practice~\cite{Perlman2000:leaderelection}
of making the vertex with the
smallest identity (an integer between $1$ and $N$) on this cycle the leader.  Recall that in SERENADE-common, after each (say $k^{th}$) iteration,
vertex $i$ learns $\phi^{(i)}_{k-}$, which contains the identities of the vertex $\sigma^{-2^k}(i)$ that is ``$2^k$ $\sigma$-hops away" from it on the cycle, and the red and the green weights of the walk 
$\sigma^{-2^k}(i)\leadsto i$. %(to that vertex).  
Our goal is to augment this $k^{th}$ iteration to learn the vertex with the smallest identity on this walk $\sigma^{-2^k}(i)\leadsto i$, which we denote as $\calL(\sigma^{-2^k}(i)\leadsto i)$
and call a level-$k$ ``precinct leader."   This way, after the $(\log_2 N)^{th}$ iteration, input port $i$ learns the identity of the level-($\log_2 N$) precinct leader 
$\mathcal{L}(\sigma^{-N}(i)\leadsto i)$, which must be $\calL_0$, the leader of the entire cycle, because the length of this cycle is no larger than $N$, the
length of the precinct (walk) $\sigma^{-N}(i)\leadsto i$.}

%the entire cycle, containing no more than $N$ distinct vertices,
%is a subset of the the ``$N$-step-long" precinct/walk $\sigma^{-N}(i)\leadsto i$.


%Note this leader designation can be randomized.  For example, we can give every node an equal chance
%to become the leader of a non-ouroboros cycle during each time slot, by making the node with the smallest $\gamma$-shifted-identity the leader  $(i + \gamma) modulo N$.

%precinct is large enough (i.e., the walk is long enough) 
%to include every vertex on the cycle.

Like in SERENADE-common, we explain this augmentation ``inductively."
The case of $k\!=\!0$ is trivial:  Each vertex $i$ considers %itself 
the one with smaller identity between itself and $\sigma^{-1}(i)$ 
to be the leader of its respective level-0 precinct.
%Then, the leader election can be seamlessly embedded in \autoref{alg: serenade-general} to ``inductively" (recursively) search $\mathcal{L}(\sigma^{(-N)}(i) \leadsto i)$. 
We claim that after iteration $k\!-\!1$, every input port $i$ gets two things done (This claim is ``the induction hypothesis").  
First, $i$ learns the identity of $\mathcal{L}(\sigma^{(-2^{k\!-\!1})}(i) 
\!\leadsto\!i)$, the leader of the level-($k\!-\!1$) precinct right-ended at
$i$ (Part I of the claim). Second, $i$
receives, from $i_U\!=\!\sigma^{(-2^{k-1})}(i)$, the vertex $2^{k\!-\!1}$ $\sigma$-hops upstream, its level-$(k-1)$ precinct leader information (Part II of the claim).
However, the union of these two level-$(k\!-\!1)$ precincts $\mathcal{L}(\sigma^{(-2^{k\!-\!1})}(i) \!\leadsto\! i)$ and $\mathcal{L}(\sigma^{(-2^{k\!-\!1})}(i_U) \!\leadsto\! i_U)$ is precisely the level-$k$ precinct $\mathcal{L}(\sigma^{-2^{k}}(i) \!\leadsto\! i)$. 
Hence, in iteration $k$,  input port $i$ simply computes 
%
%$... \leftarrow \min\big{\{}\mathcal{L}(\sigma^{(-2^{k-1})}(i_U)\!\leadsto\!i_U), \mathcal{L}(\sigma^{(-2^{k-1})}(i)\!\leadsto\!i)\big{\}}.$
$ \mathcal{L}(\sigma^{-2^{k}}(i) \leadsto i) \!\leftarrow\! \min\big{\{}\mathcal{L}(\sigma^{(-2^{k-1})}(i_U)\!\leadsto\!i_U), \mathcal{L}(\sigma^{(-2^{k-1})}(i)\!\leadsto\!i)\big{\}}$, so part I of the above claim is fulfilled;  this local computation is added to \autoref{alg: serenade-general} as ``Line 5.5".
In addition, (each) vertex $i$ sends the information $\mathcal{L}(\sigma^{(-2^{k-1})}(i)\!\leadsto\!i)$ downstream to $i_D=\sigma^{2^{k-1}}(i)$, so part II of the above claim is fulfilled;  this information is appended to the message
that $i$ sends to $i_D$ in \autoref{serenade: send-down} of \autoref{alg: serenade-general} and hence does not require a separate message exchange.  Therefore, the ``inductive step is proved''.

\addedHL{To summarize, the leader election process incurs only a small additional message complexity: 
%To do so,
% only 
a $\log_2 N$-bit-long ``precinct leader'' field needs to be added,
in each iteration of SERENADE-common, to one of the two messages sent by each vertex. 
Note however this 
% leadership information
field 
has to be included in these messages from 
% round $0$
the $0^{th}$ iteration 
onwards, if the switch intends to execute O-SERENADE in this time slot.
This is the reason why the switch controller is required to declare this intention at the beginning of the time slot 
(mentioned in $\autoref{sec: serenade-algorithms}$). }



==> sections/serenade-algorithms/serenade_comment_out.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%BELOW ARE ALL COMMENT-OUT CONTENTS%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}


In E-SERENADE, with the ``byproduct'' (\ie leadership information) of
leader election in O-SERENADE,
all vertices (input ports) on a non-ouroboros cycle can
make the same decision as SERENA does -- through up to $\log_2 N$ additional
binary search iterations. The essential idea behind E-SERENADE is to find a
repetition of the leader $\calL$ (\ie vertex with the smallest identity) of the cycle
on the walk from $\mathcal{L}$ to $\sigma^N(\mathcal{L})$. With the ``byproduct''
of the leader election (see \autoref{subsec: leader-election}), \ie the
leadership information in walks with length of power of $2$, the repetition
can be searched by a distributed version of classic binary search on the walk
$\calL \leadsto \sigma^{N}(\calL)$ -- check the identity of the middle vertex;
if it is not, the search continues on the half that contains the leader. The detail
of the binary is deferred to \autoref{subsec: binary search}.



% \begin{figure}
% \center
% \BinarySearchDemo
% \caption{An illustration of collaborative binary search.}
% \label{fig: bs}
% \end{figure}


In this section, we describe, the distributed binary search algorithm each non-ouroboros
cycle used in E-SERENADE to learn simultaneously, among the green and red weights of the
cycle, which is heavier, thus making the same decision as SERENA. This algorithm utilizes
the following information: the neighborhood knowledge sets $\{\phi^{(i)}_{k+}\}_{k = 0}^{\log N}$,
and $\{\phi^{(i)}_{k-}\}_{k = 0}^{\log N}$ obtained during the ``distance doubling'' algorithm
(see \autoref{subsec: compute-phi-k}); and leadership information produced during
the leader election algorithm in O-SERENADE
(see \autoref{subsec: leader-election}).

It suffices to describe the algorithm on an arbitrary non-ouroboros cycle,
since every non-ouroboros cycle runs an (distinct) instance of the same
algorithm. In order to obtain which is heavier among the green and red
weights of a cycle, it suffices to learn the green and red weights of
a walk which circles the cycle for integer times. Therefore, this algorithm
aims at searching a repetition of $\calL$ (\ie the leader of the cycle) on
the walk $\calL\leadsto\sigma^N(\calL)$. Note that, the repetition must exist
because $N$ -- the length of
walk $\mathcal{L} \leadsto \sigma^N(\mathcal{L})$ -- is greater than
the length of the cycle.

\autoref{alg: serenade-bsearch} captures the binary
search at search depth $d$. The search depth determines the length of the search interval: a depth of value $d$
corresponds to a search over a walk of length $N/2^d$, \ie the walk $\sigma^{-N/2^d}(i)\leadsto i$.
In \autoref{alg: serenade-bsearch}, $w_g$ and $w_r$ are the green weight and red weight of the walk
from the leader $\calL$ to $i$ respectively. {\color{blue}Note that, the term ``walk from $\calL$ to $i$''
is somehow ambiguous. However, the walk (``walk from $\calL$ to $i$'') can be easily uniquely determined
during the whole process of~\autoref{alg: serenade-bsearch} based on the initial value of $i$ -- \ie
$\sigma^N(\calL)$ -- of which the corresponding walk is $\calL\leadsto\sigma^N(\calL)$, \ie $\walk{\calL,
\sigma(\calL),\sigma^2(\calL),\cdots,\sigma^N(\calL)}$.
} {\bf I suggest to remove the comments, since we do not have space to explain the abused notations in the
pseudocodes. And I think it is not very natural to explain something here for the comments of the pseudocode.}
This binary search is initiated by $\sigma^N(\calL)$ upon the finish of the $1 + \log N$ iterations
of ``distance doubling'' (including the leader election) algorithm. Unlike the centralized binary search,
this binary search is always administrated by the ``rightmost vertex'', \ie the endpoint of the
corresponding walk to be searched.
At the initial step, $d = 0$, $w_g=w_g(\calL\leadsto \sigma^N(\calL))$, and $w_r=w_r(\calL\leadsto \sigma^N(\calL))$,
the vertex $i$ (\ie $\sigma^N(\calL)$) searches
over the walk $\sigma^{-N/2^d}(i)\leadsto i$: first, it queries whether the middle vertex of
the walk -- \ie $\sigma^{-N/2^{(d + 1)}}(i)$ -- is $\calL$ (see \autoref{code: middle-check}); if it is not,
it then queries whether the leader $\calL$ exists in the ``right half'', \ie the walk
$\sigma^{-N/2^{(d + 1)}}(i)\leadsto i$ (see \autoref{code: walk-leader-check}). If the answer is {\it yes}, the vertex $i$ keeps administrating
the binary search and goes to the next search depth (see \autoref{code: dummy-passing}). Otherwise, the vertex $i$ passes the ``baton''
to the ``rightmost vertex'' of the left half of the walk $\sigma^{-N/2^d}(i)\leadsto i$ (see
\autoref{code: intermediate-passing}). Before passing the ``baton'', in order to keep
the invariant of the weights, the vertex $i$ should update them to the weights of the walk from
$\calL$ to the new ``administrator'' (see \autoref{code: green-weight-update} and \autoref{code: red-weight-update}).
Clearly, all the queries and updates above can be finished in $O(1)$ and this binary search halts after at most $\log N$
iterations.



\noindent
{\bf Message Complexity per Iteration.}
As explained clearly, E-SERENADE has two stages, the first one is for
computing $\phi_{k+}^{(i)}$ and $\phi_{k+}^{(i)}$ with leadership information
(the same as O-SERENADE). During this stage the message complexity is
the same as O-SERENADE. The second stage is the collaborative binary
search, during each such iteration, the message complexity is $O(\log\log N + 2\cdot \log W + 1)$.

\noindent
{\bf Computational Complexity per Iteration.}
The computational complexity of E-SERENADE, during each iteration is also $O(1)$ per port, because during each iteration of the collaborative binary search, the participating ports need only $O(1)$ to do the local computation and send/receive binary search message (when necessary).


In E-SERENADE (Section ???), up to $0.5 \log_2 N$ additional rounds of iterations are carried out to gather additional
information, with which all input ports can make the same (correct) decision as they would under SERENA.  The tradeoff
is that its computational complexity is about 50\% higher than that of C-SERENADE and O-SERENADE.

\end{comment}


\begin{comment}
In this subsection, we describe, the distributed (collaborative) binary search algorithm each non-ouroboros cycle uses in E-SERENADE to learn simultaneously
the length of the cycle and the result of the green-red weight comparison.
 This algorithm makes use of the information contained in the knowledge sets
 $\{\phi^{(i)}_k\}_{k = 0}^{\log N}$, and $\{\phi^{(i)}_k\}_{k = 0}^{\log N}$,
 obtained respectively through the ``distance doubling" algorithm
 (\ie \autoref{alg: serenade-general}) and the leader election algorithm as
 a part of O-SERENADE.

 The essential idea of this binary search is to make
 use of the ``propagation speed'' of the identity of the ``leader''. Now
 we focus on a single non-ouroboros cycle (other non-ouroboros cycles
 are the same). Suppose $\mathcal{L}$ is the identity of the leader in the
 cycle. As explained in \autoref{subsec: leader-election}, after the
 $1 + \log N$ iterations for computing knowledge sets (with ``leadership
 information''), each vertex in the cycle learns the identity of the
 leader. However, different vertices learns $\mathcal{L}$ in different
 iterations. Roughly speaking, vertices with shorter distance from
 the leader learns $\mathcal{L}$ earlier. For example,
 $\sigma^{2}(\mathcal{L})$ learns $\mathcal{L}$ in the $1^{st}$ iteration
 (\ie the second iteration among the $1 + \log N$ iterations).
 By making full use of such properties, focusing on a special iteration
 (we will specify it later), based on whether the vertices learn $\mathcal{L}$
 or not, the vertices on the path from $\mathcal{L}$ (including) to
 $\mathcal{L}$ (excluding) can be converted in to an ordered array.
 Therefore, we perform a binary search on the array.

The special iteration is the first iteration when the ``leadership
information'' received by $\mathcal{L}$ is $\mathcal{L}$. Let $k_0$
be the iteration. Then, recall from \autoref{subsec: leader-election},
it is clear that the leader $\mathcal{L}$ is on the walk
$\sigma^{(-2^{k_0 - 1})}\bigParenthes{\sigma^{(-2^{k_0 - 1})}(\mathcal{L})} \leadsto \sigma^{(-2^{k_0 - 2})}(\mathcal{L})$ and
not on the walk $\sigma^{(- 2^{k_0-2})}\bigParenthes{\sigma^{(-2^{k_0 - 1})}(\mathcal{L})}\leadsto \sigma^{(-2^{k_0 - 1})}(\mathcal{L})$. Hence, $l<2^{k_0}<2l$, where $l$ is the length of the cycle. Therefore, at the $(k_0-1)^{th}$
iteration, vertex $\sigma^{(2^{k_0-1})}(\mathcal{L})$ is the farthest vertex
from $\mathcal{L}$ learns $\mathcal{L}$. Both the two walks
$\mathcal{L}\leadsto \sigma^{(2^{k_0-1})}(\mathcal{L})$ and $\sigma^{(2^{k_0-1})}(\mathcal{L}) \leadsto \sigma^{(2^{k_0})}(\mathcal{L})$ reduce to paths,
as shown in \autoref{subfig: cycle-demo}.
And any vertices on the path $\mathcal{L}\leadsto \sigma^{(2^{k_0-1})}(\mathcal{L})$ learns $\mathcal{L}$, while all vertices on the path from $\sigma^{(2^{k_0-1})}(\mathcal{L})$ to $\mathcal{L}$ (excluding the source and destination) do not learn $\mathcal{L}$. As $\mathcal{L}$ already learns the
weight information from the knowledge set $\phi^{(\mathcal{L})}_{k_0-1}$, to
get the weight information of the cycle reduces to compute the weight
information of the path from $\sigma^{(2^{k_0-1})}(\mathcal{L})$ to $\mathcal{L}$. As shown in \autoref{subfig: bs-analogy}, based on whether or not
learning $\mathcal{L}$, all vertices on the path from $\sigma^{(2^{k_0-1})}(\mathcal{L})$ to $\sigma^{2^{k_0}}(\mathcal{L})$ can be converted as an
ordered array. After such conversions, the problem to obtain the exact
weight information of the path $\sigma^{(2^{k_0-1})}(\mathcal{L})$ to $\mathcal{L}$ is reduced to find a specific value in an ordered array.

The leader $\mathcal{L}$ first sends
$\sigma^{(2^{k_0-1})}(\mathcal{L})$ the value of $k_0$ to initiates
the binary search. Then, $\sigma^{(2^{k_0-1})}(\mathcal{L})$ sends a message to the vertex in the middle
of $\sigma^{(2^{k_0-1})}(\mathcal{L})$ and $\sigma^{(2^{k_0})}(\mathcal{L})$ (\ie checking the middle element). If it already
learns $\mathcal{L}$, continue searching the path from $\sigma^{(2^{k_0-1})}(\mathcal{L})$ to the middle vertex (\ie searching the lower half of the
array), otherwise searching the path from the middle to $\sigma^{(2^{k_0})}(\mathcal{L})$ (\ie searching the upper half of the array). So on and so force
until reaches the leader $\mathcal{L}$ (\ie finding the target).

% As explained in \autoref{sec: serenade}, to exactly emulate SERENA parallelly (\ie E-SERENADE),
% we need at most $\log N$ more iterations to conduct a ``chord-like'' binary
% search~\cite{Stoica2003chord}. The binary search procedure is of course initialized by the
% leader itself, and searches itself. First of all, the leader $v$ searches the very first
% iteration (say $k_0$) in which the leader information it receives is itself. It is clear that,
% the length of the walk from $v$ to $\sigma^{2^{k_0}}(v)$, \ie $v\leadsto \sigma^{2^{k_0}}(v)$,
% satisfies $l < 2^{k_0} < 2l$, where $l$ is the exact length of the
% non-ouroboros cycle. Hence to get the exact weight of the cycle, the leader needs to learn
% the weight information on the {\bf path} from $\sigma^{2^{k_0-1}}(v)$ to $v$, since the leader
% already learns the weight information on the {\bf path} from $v$ to $\sigma^{2^{k_0-1}}(v)$. Now it is
% the time to make the full use of the leadership information. As explained before, the
% leadership information in the $k^{th}$ iteration at input port $i$ is the minimum identity
% among all the inputs in the walk $\sigma^{-2^k}(i)\leadsto i$. Therefore, at the $(k_0-1)^{th}$
% iteration, no input ports on the path from $\sigma^{(2^{k_0 - 1})}(v)$ to $v$ have learned the
% identity of the leader, \ie the identities of their candidate leaders are not equal to
% the identity of the leader in the cycle. And all the input ports on the path from $v$ to
% $\sigma^{(2^{k_0 - 1})}(v)$ already learns the identity of the leader at the $(k_0 - 1)^{th}$
% iteration. By
% using
% such
% information, an input port can
% easily figure out the leader's relative position on
% the path from $\sigma^{(2^{k_0 - 1})}(v)$ to $\sigma^{(2^{k_0})}(v)$.


\begin{algorithm}[t]
\caption{Binary search at input port $i$.}
\label{alg: serenade-bsearch}
\SetKwProg{Proc}{Procedure}{}{}

% \tcc{Require $k_0$}
% \tcc{Require current walk length, $\ell$}
% \tcc{Require current weights, $w_r$ and $w_g$}
% \tcc{Require current message direction, $d$}

Receive message $\mathcal{M}=\{\ell, w_r\}$


\tcc{Update weights}
\uIf{$\mathcal{M}$ is from ``downstream'' relative to $i$}{
  $w_r \leftarrow w_r - w_r\bigParenthes{i \leadsto \sigma^\ell(i)}$
}\uElse{
  $w_r \leftarrow w_r + w_r\bigParenthes{\sigma^{-\ell}(i) \leadsto i}$
}

\tcc{Stop check}
\uIf{I am the leader}{
    {\bf stop}
}

\tcc{Continue searching}
\uIf{$(k_0-1)^{th}$ candidate leader is leader}{

Send to $\sigma^{(-\ell/2)}(i)$ message $\mathcal{M}=\{\ell / 2, w_r\}$

}
\uElse {
        Send to $\sigma^{(\ell/2)}(i)$ message $\mathcal{M}=\{\ell/2, w_r\}$
}

\end{algorithm}

% \begin{algorithm}
% \caption{Binary search at input port $i$.}
% \label{alg: serenade-bsearch}
% \SetKwProg{Proc}{Procedure}{}{}

% % \tcc{Require $k_0$}
% % \tcc{Require current walk length, $\ell$}
% % \tcc{Require current weights, $w_r$ and $w_g$}
% % \tcc{Require current message direction, $d$}

% Receive message $\mathcal{M}=\{k_0, w_r, w_g, \mathcal{L}, \ell, \mathcal{R},\mathcal{D}\}$


% Backup walk length $\hat{\ell} \leftarrow \ell$

% Update walk length $\ell \leftarrow \ell / 2$

% \tcc{The message is from $\mathcal{R}$}
% \uIf{$\mathcal{D}=1$}{

%     Update the weights:
%     \begin{equation*}
%         \begin{aligned}
%             w_r &\leftarrow w_r - w_r\bigParenthes{\mathcal{W}_i(\hat{\ell})}\\
%             w_g &\leftarrow w_g - w_g\bigParenthes{\mathcal{W}_i(\hat{\ell})}
%         \end{aligned}
%     \end{equation*}

%     \uIf{I am the leader}{

%         {\bf stop}

%     }

%     \uIf{$(k_0-1)^{th}$ candidate leader is leader}{

%         \tcc{Leader is on the path from $\mathcal{L}$ to me}

%         $\mathcal{R} \leftarrow \mathcal{R} - \hat{\ell}$
%         \label{code: redundant-1}


%         Send to $\sigma^{-\ell}(i)$ message $\mathcal{M}=\{k_0, w_r, w_g, \mathcal{L}, \ell,
%         \mathcal{R},1\}$
%     }
%     \uElse{

%        \tcc{Leader is on the path from me to $\mathcal{R}$}

%        $\mathcal{L} \leftarrow \mathcal{R} - \hat{\ell}$
%        \label{code: redundant-2}

%        Send to $\sigma^{\ell}(i)$ message $\mathcal{M}=\{k_0, w_r, w_g, \mathcal{L}, \ell,
%        \mathcal{R},0\}$
%     }
% }
% \uElse{

%     Update the weights:
%     \begin{equation*}
%     \begin{aligned}
%         w_r &\leftarrow w_r + w_r\bigParenthes{\mathcal{W}_i(\hat{\ell})}\\
%         w_g &\leftarrow w_g + w_g\bigParenthes{\mathcal{W}_i(\hat{\ell})}
%     \end{aligned}
%     \end{equation*}

%     \uIf{I am the leader}{

%         {\bf stop}

%     }

%     \uIf{$(k_0-1)^{th}$ candidate leader is leader}{
%         \tcc{Leader is on the path from $\mathcal{L}$ to me}

%         $\mathcal{R} \leftarrow \mathcal{L} + \hat{\ell}$
%         \label{code: redundant-3}

%         Send to $\sigma^{-\ell}(i)$ message $\mathcal{M}=\{k_0, w_r, w_g, \mathcal{L}, \ell,
%        \mathcal{R},1\}$
%     }
%     \uElse{

%        \tcc{Leader is on the path from me to $\mathcal{R}$}

%        $\mathcal{L} \leftarrow \mathcal{L} + \hat{\ell}$
%        \label{code: redundant-4}

%        Send to $\sigma^{\ell}(i)$ message $\mathcal{M}=\{k_0, w_r, w_g, \mathcal{L}, \ell,
%        \mathcal{R},0\}$
%     }

% }


% \end{algorithm}


% At the very beginning of the binary search,
% the leader sends the value of $k_0$ to $u=\sigma^{(2^{k_0-1})}(v)$ and lets it start the
% binary search. Let $\mathcal{M}=\{\ell,w_r, w_g\}$ be the binary search message, where $\ell$ is the walk length from the
% sender to the receiver, $w_r$ and $w_g$ represents the red weight and green
% weight of the walk from $u$ to the sender. Note that, in fact, the binary
% search message should also contain $k_0$, and a ``downstream''-``upstream''
% indicator to tell the receiver where the message is from. For simplicity,
% we omit these two parts and assume all input ports know $k_0$ and can figure
% out where the binary search message is from.
\autoref{alg: serenade-bsearch} details the collaborative binary search at
input port $i$. Note that, $\mathcal{M}=\{\ell,w_r\}$ represents the binary
search message, where for $\ell$ is the walk length from the
sender to the receiver, $w_r$ represents the red weight of the path from $\sigma^{(2^{k_0-1})}(\mathcal{L})$ to the sender. For
simplicity we omit three necessary messages: 1) the value of $k_0$; 2)
the green weight $w_g$ in $\mathcal{M}$ and
only show the updating for $w_r$, because the updating for $w_g$ is the same;
3) a $1$-bit information to tell the receiver where the message is from (\ie
``upstream'' or ``downstream'').
Initially, $u$ set $\mathcal{M}$ as $\ell=2^{k_0 -2}$, $w_r=w_g=0$.

% Initially, $u$ sets the walk length $\ell$ to be $2^{k_0 - 2}$, position of the
% ``leftmost'' vertex $\mathcal{L}=0$, position of the ``rightmost'' vertex $\mathcal{R}=2^{k_0-1}$, and
% sends message $\mathcal{M}$ to $\sigma(u)$ (\ie the middle
% point in the
% path from $u$ to $\sigma^{(2^{k_0})}(v)$), where the message $\mathcal{M}$ is defined as
% \begin{equation*}
% \mathcal{M}\triangleq\{k_0, w_r\bigParenthes{\mathcal{W}_{u}(\ell)}, w_g\bigParenthes
% {\mathcal{W}_{u}(\ell)},\mathcal{L}, \ell, \mathcal{R},\mathcal{D}\},
% \end{equation*}
% where $\mathcal{D}$ is a binary information to indicate where the message $\mathcal{M}$
% is from. Specifically, $\mathcal{D}=1$ if $\mathcal{M}$ is from $\mathcal{R}$, otherwise,
% $\mathcal{D}=0$. \autoref{alg: serenade-bsearch}
% gives the details of the binary search procedure. Clearly, \autoref{alg: serenade-bsearch}
% can be finished in at most $(k_0 - 1)$ iterations, which is less than $\log N$. Note that,
% in \autoref{alg: serenade-bsearch}, $\mathcal{L}$ and $\mathcal{R}$ are not necessary,
% we choose to include them just from the sake of understanding. In other words, the message
% $\mathcal{M}$ can be simplified to $\mathcal{M}\triangleq\{k_0, w_r\bigParenthes{\mathcal{W}_{u}(\ell)}, w_g\bigParenthes
% {\mathcal{W}_{u}(\ell)},\ell,\mathcal{D}\}$, and all lines related to $\mathcal{L}$ and
% $\mathcal
% {R}$ (\ie \autoref{code: redundant-1}, \autoref{code: redundant-2}, \autoref{code: redundant-3},
% and
% \autoref{code: redundant-4}) can be removed.

%E-SERENADE builds upon O-SERENADE.
\end{comment}
\begin{comment} %% 02-23-2017
\subsection{Leader Election}
\label{subsec: leader-election}

\hlc{red}{}{\bf Revised by Grace.}

{\color{blue}
In O-SERENADE and E-SERENADE, one vertex with the smallest identity in a cycle is designated as the leader to make the merge decision. The leader election can be seamlessly embedded in \autoref{alg: serenade-general} because it can also be described ``inductively" (recursively). Suppose in iteration $k-1$, input port $i$ learns a "precinct-level" leader $\mathcal{L}(\sigma^{(-2^{k-1})}(i) \leadsto i)$ in the walk $\sigma^{(-2^{k-1})}(i) \leadsto i$. Then in iteration $k$, input port $i$ simply computes $\mathcal{L}(\sigma^{(-2^{k})}(i) \leadsto i)$ after receiving the walk leader of its upstream node $i_U$, $\sigma^{(-2^{k-1})}(i)$. After the $1 + \log N$ iterations, input port $i$ learns $\mathcal{L}(\sigma^{(-N)}(i)\leadsto i)$ in a long enough walk, since the cycle length is at most $N$. This walk leader points to the leader of cycle, whose identify is smallest ($\mathcal{L}$ for short).

We simply augment \autoref{alg: serenade-general} with leader election as follows. Initially, input port $i$ computes $\mathcal{L}(\sigma^{(-1)}(i) \leadsto i)$, the minimal identity between $i$ and its 1-step upstream $\sigma^{(-1)}(i)$. At the beginning of iteration $k$, every input port $i$ sends $\mathcal{L}(\sigma^{(-2^{(k-1)})}(i)\leadsto i)$ to its downstream $i_D$ (added in line 3), and similarly receives $\mathcal{L}(\sigma^{(-2^{(k-1)})}(i_U) \leadsto i_U)$ from its upstream $i_U$ (added in line 4). In line 5, input port $i$ also computes its current walk leader,\\
\textit{$\mathcal{L}(\sigma^{(-2^{k})}(i)\leadsto i)=\min\{\mathcal{L}(\sigma^{(-2^{k-1})}(i_U)\leadsto i_U), \mathcal{L}(\sigma^{(-2^{k-1})}(i)\leadsto i)\}$}.\\
Note that the leader election lets every input port $i$ update the walk leadership information to its downstream, while the computation of knowledge sets requires the information updates in both: upstream and downstream. Finally, each input port $i$ learns the leader identity $\mathcal{L}$, and records the walk leadership information in all iterations $\mathcal{L}(\sigma^{(-2^{k})}(i)\leadsto i)$ ($\forall k$), which will be used in collaborative binary search (\autoref{subsec: binary search}).
}

%In each iteration $k$, input port $i$ computes\\
%\textit{$\mathcal{L}(\sigma^{(-2^{k})}(i)\leadsto i)=\min\{\mathcal{L}(\sigma^{(-2^{k-1})}(i_U)\leadsto i_U), \mathcal{L}(\sigma^{(-2^{k-1})}(i)\leadsto i)\}$},\\
%and sends it to the downstream (in line 3). At the same time, input port $i$ will receive $\mathcal{L}(\sigma^{(-2^{k})}(i_U) \leadsto i_U)$ from its upstream $i_U$ (in line 4).

\hlc{red}{}{\bf It seems that this section was not revised.}

% With \autoref{alg: serenade-general}, we only finish the algorithmic part for C-SERENADE.
% For O-SERENADE and E-SERENADE, as mentioned in \autoref{sec: serenade}, we need one designated
% vertex (\ie a leader) per cycle to make decision. To augment \autoref{alg: serenade-general}
% with leadership election feature, we only need to send a little more information in
% each iteration. More specifically, since every input port has its own unique identity, we
% make the one in a cycle with the minimum identity as a leader. To achieve
% this, during the iteration for computing $\phi^{(i)}_{k-}$,
% besides the knowledge set $\phi^{(i)}_{(k-1)-}$, input
% port $i$ also needs
% to send to $\sigma^{(2^{k-1})}(i)$ the leadership information, \ie the minimum identity in
% the walk $\sigma^{(-2^{k-1})}(i)\leadsto i$, which will be referred to as the candidate leader.
% Note that, it should also receive the leadership information \ie candidate leader in
% $\sigma^{(-2^{k})}(i)\leadsto \sigma^{(-2^{k-1})}(i)$ in the same iteration.
% Hence, input port $i$ can compute the
% candidate leader in the walk $\sigma^{(-2^{k})}(i)\leadsto i$. Therefore,
% after the $k^{th}$ ($k=0,1,2,\cdots,\log N$) iteration, each input port $i$ knows the candidate
% leader in the walk $\sigma^{(-2^{k})}(i)\leadsto i$. Therefore, after the $1 + \log N$ iterations, each
% input port will know the minimum identity among the vertices in the cycle, since the cycle
% length is at most $N$. In other words, each input port learns the identity of the leader in
% the cycle.

With \autoref{alg: serenade-general}, we only finish the algorithmic part for C-SERENADE.
For O-SERENADE and E-SERENADE, as mentioned in \autoref{sec: serenade}, we need one designated
vertex (\ie a leader) per cycle to make decision. To augment \autoref{alg: serenade-general}
with leadership election feature, we only need to
% send a little more information in
% each iteration.
compute the leadership knowledge set $\psi^{(i)}_{k}$ during iteration
$k$ at input port $i$.
As explained in \autoref{subsec: o-serenade}, the leadership knowledge
set $\psi^{(i)}_{k}$ is just the neighborhood knowledge set $\phi^{(i)}_{k-}$
augmented with the leader in the walk $\sigma^{(-2^{k})}(i) \leadsto i$,
\ie the input port in $\sigma^{(-2^{k})}(i) \leadsto i$ with the minimum identity.
% More specifically, since every input port has its own unique identity, we
% make the one in a cycle with the minimum identity as a leader.
To achieve
this, during the iteration for computing $\phi^{(i)}_{k-}$,
besides the knowledge set $\phi^{(i)}_{(k-1)-}$, input
port $i$ also needs
to send to $\sigma^{(2^{k-1})}(i)$ the leadership information, \ie the leader in
the walk $\sigma^{(-2^{k-1})}(i)\leadsto i$.
Note that, it should also receive the leadership information \ie candidate leader in
$\sigma^{(-2^{k})}(i)\leadsto \sigma^{(-2^{k-1})}(i)$ in the same iteration.
Hence, input port $i$ can compute the
leader in the walk $\sigma^{(-2^{k})}(i)\leadsto i$, thus obtaining the
leadership knowledge set $\psi^{(i)}_{k}$.
Therefore,
after the $k^{th}$ ($k=0,1,2,\cdots,\log N$) iteration, each input port $i$ learns $\psi^{(i)}_{k}$. After the $1 + \log N$ iterations,
with $\psi^{(i)}_{\log N}$, input port $i$ learns the leader in the walk $\sigma^{(-N)}(i)\leadsto i$, \ie the minimum
identity in $\sigma^{(-N)}(i)\leadsto i$. Therefore, after the $1 + \log N$ iterations, each
input port will know the minimum identity among the vertices in the cycle, since the cycle
length is at most $N$. In other words, each input port learns the identity of the leader in
the cycle.

%\begin{table*}
%\caption{Cycle statistics.}
%\centering
%\OuroborosStats
%\label{tab: ouroboros_statistic}
%\end{table*}

After the \autoref{alg: serenade-general} augmented with leadership information, the leaders need
one more iteration to finish O-SERENADE. That is, the leader in each cycle sends its decision (\ie
one-bit
information with $0$ stands for red, and $1$ represents green) together with its identity
to a centralized controller, who broadcasts this information to all input ports. Note that, in theory the centralized controller might need to broadcast for up to $O(N)$ times,
since there could be up to $O(N)$ non-ouroboros cycles in the worst case. However, in practice
this event is rare.
% \autoref{tab: ouroboros_statistic} shows the cycle statistics of the
% graph for the merged matching of two uniformly random matchings.
For example, as shown by \autoref{tab:
ouroboros_statistic}, there are less than $3$ non-ouroboros cycles in a
uniformly random permutation on average even when $N=1024$.
% In other words, we can consider that there are only constant number (\ie $O(1)$) of broadcasts.
% [The following claim is not $100\%$ sure.] However, strict $O(1)$ operations (per port) to passing
% the leaders' information to all the input ports inside the corresponding cycles can also be
% achieved. For example, we can use two $N$-bit bitmaps $B_1$ and $B_2$ (we assume that each bit can be
% read and
% written independently), which can be accessed by all input ports. $B_1$ is for informing whether
% the corresponding leader has made its decision, and $B_2$ records the leaders' decisions. More
% precisely, $B_1[k] = 1$ for $k=1,2,\cdots,N$ means the leader with identity $k$ has recorded its
% decision, $B_1[k] = 0$ means it has not. $B_2[k]$ records the decision of
% the leader $k$ ($1$ for green, $0$ for red). At
% the
% beginning of each
%  time slot, the two $N$-bit bitmaps are reset to all-zero (by hardware with $O(1)$). After the
%  $1 + \log N$ iterations, the
%  leader $k$
%  just
%  needs first set $B_2[k] = 1$ if it chooses green, otherwise $B_2[k] = 0$. Then,
%  it sets $B_1[k]=1$. As every vertex (input port) learns the identity of the leader inside
%  the corresponding cycle, it just needs to check the $k^{th}$ bit of the two bitmaps, if
%  it learns the leader is $k$.
\end{comment}
%

%
%% comment out for revision 02-17-2016
\begin{comment}
A natural question to ask is whether SERENA (with its MERGE procedure) can be
emulated {\bf EXACTLY} in a parallel manner with only $O(\log N)$ work per
port. The last scheme of SERENADE answers this question definitively.
With the leadership information, all vertices on a non-ouroboros cycle can
collaboratively perform, through up to $\log_2 N$ additional iterations,
%``Chord-like"~\cite{Stoica2003chord}
a binary search over the sets of
``leadership information" these vertices collectively have, can compute the
red and the green weights of the cycle exactly. Here, we will only give
some intuitions, details are deferred to \autoref{subsec: binary search}.
The essential idea is to make full use of the leadership information
in the leadership knowledge sets. As explained earlier, after the
$1+\log N$ iterations with leadership information, each input port
$i$ will learn the leader of the cycle. Besides, there are some
useful by-products, \ie the leader in the walks in all the leadership
knowledge sets. The binary search is targeting at the last repetition of
the leader $\mathcal{L}$ on the walk $\mathcal{L}\leadsto \sigma^{N}(\mathcal{L})$. Clearly, this can be done by check whether $\mathcal{L}$
appears in the walk $\sigma^{N/2}(\mathcal{L})\leadsto \sigma^{N}(\mathcal{L})$. If yes, then checking the walk with half length, $\sigma^{3N/4}(\mathcal{L})\leadsto \sigma^{N}(\mathcal{L})$ otherwise, checking $\sigma^{N/4}(\mathcal{L})\leadsto \sigma^{N/2}(\mathcal{L})$. Repeating such process, we
can eventually find the last repetition of $\mathcal{L}$.

\end{comment}

\begin{comment}
\begin{algorithm}[t]
\caption{O-SERENADE at any input port $i$ on any non-ouroboros cycle.}
\label{alg: o-serenade}
\SetKwProg{Proc}{Procedure}{}{}


% \uIf{I am in an ouroboros cycle}{

%     \uIf{Red weight (of the cycle) is heavier}{

%         pick red edges

%     }
%     \uElse
%     {
%         pick green edges
%     }


% }
% \uElse {

\If{$i$ (self) is the leader of the cycle}{
    \eIf{$w_r\bigParenthes{i\leadsto \sigma^N(i)} > w_g\bigParenthes{i\leadsto \sigma^N(i)}$}{

        pick the red sub-matching\;

    }
    {
        pick the green sub-matching\;
    }

}
% }

\end{algorithm}
\end{comment}

\begin{comment}

\begin{algorithm}[t]
\caption{C-SERENADE at any input port $i$.}
\label{alg: c-serenade}
\SetKwProg{Proc}{Procedure}{}{}

% \uIf{I am in an ouroboros cycle {\bf AND} red weight (of the cycle) is heavier}{

%         pick red edges

% }
% \uElse {

%         pick green edges

% }
\eIf{$i$ (self) is on an ouroboros cycle}{

    \If{Red weight (of the cycle) is heavier}{

        pick the red edge\;

    }
    % {
    %     pick green edges
    % }


}
{

        pick the green edge\;

}
\end{algorithm}

\noindent
{\bf Message Complexity per Iteration.} The message complexity of each iteration is $(2 \cdot \log N + 4 \cdot \log W)$ \hlc{red}{}{Here, $W$ might not be appropriate.} bits per port, where $W$ denotes the maximum weight. Because, during the $k^{th}$ iteration, each input port only needs to send the message about its own $\phi_{(k-1)+}$ and $\phi_{(k-1)-}$,
in which each identity needs $\log N$ bits and each weight information
need at most $\log W$ bits. In fact, message complexity (per iteration) can be
reduced to $2\cdot \bigParenthes{\log N +(\log W + 1)}$ bits per port, because C-SERENADE
only needs the difference between the red weight and green weight of
walks with certain lengths. Similar arguments also apply to O-SERENADE
and E-SERENADE.

\noindent
{\bf Computational Complexity per Iteration.} The computational complexity per iteration (per port) in C-SERENADE is $O(1)$, since
% it has at most $1 + \log N$ iterations, and
each iteration takes
$O(1)$ time to send/receive message and do local computation.

\end{comment}

\begin{comment}%% 02-22-2017
One can imagine there is much room to improve C-SERENADE, since it ignores a considerable amount of information that can help vertices in a non-ouroboros cycle make an educated guess about which sub-matching is heavier. More specifically, each vertex $i$ knows the red and green weights of any walk from $i$ to $\sigma^n(i)$ where $n$ is an ouroboros number. [{\color{red}$n$ is not suitable to denote an ouroboros number}] From this set of weights, vertex $i$ can make a merge decision by guessing whether the red or the green sub-matching is heavier. It is clear that the larger $n$ is, the more times the walk $i\leadsto \sigma^n(i)$ circles the cycle. That is, the larger $n$ is, the higher probability there is that the relative order of \ie $w_r(i\leadsto \sigma^n(i))$ and $w_g(i\leadsto \sigma^n(i))$, is the same as that of the red and green weights of the cycle.

%Therefore, our O-SERENADE scheme is to make a call based on the two largest numbers in this set: $w_g(i\leadsto \sigma^N(i))$ and $w_r(i\leadsto\sigma^N(i))$. We refer to this scheme as O-SERENADE, because it opportunistically use the weights of the walk $i\leadsto\sigma^N(i)$ to represent those of the cycle. The decision rule of O-SERENADE is that if $w_r(i\leadsto \sigma^N(i)) \ge w_g(i\leadsto\sigma^N(i))$, then the red sub-matching is chosen. Otherwise, the green sub-matching is chosen. Note this decision rule does not guarantee with certainty the heavier sub-matching is chosen, because there is a non-zero remainder (otherwise this cycle is ouroboros) when $N$, the length of the walk is divided by the length of the cycle $l$. The red and green weights of this remainder section are counted once more than those of the rest, which can ``tip the scales in the wrong direction".

Therefore, O-SERENADE scheme is designed to make a decision based on the knowledge sets of a long talk whose length is $N$, \ie $w_g(i\leadsto \sigma^N(i))$ and $w_r(i\leadsto\sigma^N(i))$. This scheme is called as O-SERENADE because it opportunistically use the weights of $i\leadsto\sigma^N(i)$ to represent those of the cycle. The decision rule of O-SERENADE is that if $w_r(i\leadsto \sigma^N(i)) \ge w_g(i\leadsto\sigma^N(i))$, then the red sub-matching is chosen. Otherwise, the green sub-matching is chosen. Note that it does not guarantee that a heavier sub-matching is chosen, because there is a non-zero remainder when $N$ is divided by the cycle length $l$ (otherwise the cycle is ouroboros). The red and green weights of this remainder section are counted once more than those of the rest, which can ``tip the scales in the wrong direction". Here, ``remainder section'' is
the last ($N \bmod l$) edges on the walk $i\leadsto \sigma^N(i)$, where
$l$ is the length of the cycle.

% Use the example in \autoref{subsec: merge-perm} but assuming different weights of edges,
% Use the third cycle (from left to right) in \autoref{fig: cycles-in-permutation} as an example, and assume the weights of edges on the cycle are as follows:
% $w_r(I_4,O_6)\sm{=}3$, $w_r(I_7,O_1)\sm{=}3$, $w_g (O_8,I_1)\sm{=}6$, and all
% other edges have a weight of $1$.
Use the cycle shown in \autoref{fig: cycle-with-weights} as an example.
For the walk $4\leadsto \sigma^8(4)$, its
red weight is larger than its green weight because $w_r(4\leadsto \sigma^8(4)) = 2\cdot (3 + 3 +1) + (3 + 3)=20$,
and $w_g(4\leadsto \sigma^8 (4))=2\cdot(6 + 1 + 1) + (1 + 1)=18 < 20$. However, for the cycle, its red weight is $7$ which is less than its green
weight, $8$. Note that, in the above example, we will not have any issue, as
the cycle is ouroboros.
% [{\color{red}?However, empirically the vast majority such decisions made by this decision rule is correct (in terms of choosing the heavier sub-matching), as shown in our simulations}].

%Note that, unlike the case of C-SERENADE, O-SERENADE cannot let each vertex $i$ on a non-ouroboros cycle independently makes a decision based on its ``local knowledge sets". %This is because two different vertices on the same non-ouroboros cycle, whose $N$-edge-long walks have different ``remainder sections", could pick two sub-matchings (edges) of %opposite colors.
%Using the same example as above, if making decision based on the longest
%walk, the input port $4$ would choose red, while input port $3$ would choose green.
%In this case, two input ports attempt to transmit to the same output port, resulting in a collision. To avoid this situation, we let one designated vertex to make such a decision based on %its local knowledge sets for all vertices on a non-ouroboros cycle.

% We will show in \autoref {subsec: leader-election} t




 % that can be seamlessly embedded into the $1+ \log_2 N$ knowledge-discovering iterations. \autoref{alg: o-serenade} summaries the final decision rule of O-SERENADE.
\end{comment}%% 02-22-2017

\begin{comment}
For a cycle that is not ouroboros, however, vertices cannot tell with certainty which sub-matching is heavier, since they cannot find a walk which circles this cycle with its own knowledge sets. In such a case, each vertex will choose the old (green) sub-matching (\ie the edges belong to the matching for the previous time slot), even when the new (red) sub-matching is actually heavier. The rationale is that this Conservative approach is safe as it guarantees (with certainty) that the newly merged matching is at least as heavier as the old one, with respect to the current queue lengths. That is why we call the scheme C-SERENADE. \autoref{alg: c-serenade} summarizes
the decision rule of C-SERENADE.
\end{comment}



%% comment out: 02-18-2017
\begin{comment}
In this section, we describe, the distributed binary search algorithm each non-ouroboros cycle uses in E-SERENADE to learn simultaneously
% the length of the cycle and
the result of the green-red weight comparison.  This algorithm makes use of the information contained in the
% knowledge sets $\{\phi^{(i)}_k\}_{k = 0}^{\log N}$, and $\{\phi^{(i)}_{-k}\}_{k = 0}^{\log N}$
knowledge sets $\{\phi^{(i)}_{k+}\}_{k = 0}^{\log N}$, and $\{\psi^{(i)}_{k}\}_{k = 0}^{\log N}$
, obtained respectively through the ``distance doubling" algorithm and the leader
election algorithm as a part of O-SERENADE.

It suffices to describe the algorithm on an arbitrary non-ouroboros cycle,
since every non-ouroboros cycle runs an (distinct) instance of the same
algorithm. Suppose the leader of this cycle is $\mathcal{L}$.
The essential idea of the algorithm to search for the last repetition of
$\mathcal{L}$ along the walk $\mathcal{L} \leadsto \sigma^N(\mathcal{L})$,
obtaining? the result of the green-red weight comparison along the walk
from $\mathcal{L}$ to its last repetition. With this
result, $\mathcal{L}$ can know precisely whether the green
weight of the cycle, or the red weight of the cycle, is heavier, thus
making the same (correct) decision as SERENA. The reasoning is the same as that
of the three ideal situations in~\autoref{subsubsec: ideal-situations}.
% The essential idea of the algorithm is to let
% $\sigma^N(\mathcal{L})$ initiate a distributed binary
% search, for the last repetition of of $\mathcal{L}$, along the walk $\mathcal{L} \leadsto \sigma^N(\mathcal{L})$.
Note that, this repetition must exist because $N$ -- the length of
walk $\mathcal{L} \leadsto \sigma^N(\mathcal{L})$ -- is greater than
% or equal to
the length of the cycle.

This search is initiated at $\sigma^N(\mathcal{L})$, and proceeds
``recursively" as follows. The vertex (\ie input port)
$\sigma^N(\mathcal{L})$ first checks whether the middle vertex
(\ie $\sigma^{N/2}(\sleader)$)
along the walk $\SWalk{\mathcal{L}}{N}$ is the target
(\ie $\sleader$) by querying its knowledge set $\phi^{\sigma^N(\sleader)}_{(\log_2 N - 1)-}$ (note $\sigma^{N/2}(\sleader) = \sigma^{(-N/2)}\bigParenthes{\sigma^{N}(\sleader)}\in \phi^{\sigma^N(\sleader)}_{(\log_2 N - 1)-}$).
If the answer is luckily yes (referred to as {\it Case 0}), the baton is passed to $\sigma^{N/2}(\sleader)$ and
the search stops. Otherwise, $\sigma^N(\sleader)$ then
checks whether there is a repetition of $\mathcal{L}$ along the walk
$\sigma^{N/2}(\mathcal{L}) \leadsto \sigma^{N}(\mathcal{L})$ -- the
``right half'' of the walk $\mathcal{L}\leadsto \sigma^N(\mathcal{L})$ --
by querying ``$\mathcal{L} \in \psi^{\sigma^N(L)}_{(\log_2 N - 1)}$?''
against its leadership knowledge sets.
%
% The node (\ie input port)
% $\sigma^N(\mathcal{L})$
% queries its leadership knowledge set $\psi^{(\sigma^N(\mathcal{L}))}_{(\log N - 1)}$
% checking whether there is a repetition of
% $\mathcal{L}$ along the walk $\sigma^{N/2}(\mathcal{L}) \leadsto \sigma^{N}(\mathcal{L})$, \ie whether the leader in $\sigma^{N/2}(\mathcal{L}) \leadsto \sigma^{N}(\mathcal{L})$ is $\mathcal{L}$.
%
% contacts $\sigma^{N/2}(l)$ asking it whether there is a repetition of $l$ along the walk $\sigma^{N/4}(l)\leadsto \sigma^{N/2}(l)$.
% For $\sigma^{N/2}(l)$ to answer this question, it simply checks whether the leader along the walk $\sigma^{N/4}(l)\leadsto \sigma^{N/2}(l)$ (i.e., knowledge
% set $???$), obtained during the leader election algorithm, is $l$.
If the answer
% to
% this question
% this query
is no (referred to as {\it Case 1}), the target (\ie the last? repetition of
$\mathcal{L}$) must exist in the ``left half''. Hence,
the baton is passed on to $\sigma^{N/2}(\mathcal{L})$, which shall continue
the binary search along the walk $\mathcal{L} \leadsto \sigma^{N/2}(\mathcal{L})$,
the ``left half" of the walk $\mathcal{L} \leadsto \sigma^N(\mathcal{L})$.
%  by
% % first contacting $\sigma^{N/4}(l)$.
% repeating the same query along the walk $\sigma^{N/4}(\mathcal{L}) \leadsto \sigma^{N/2}(\mathcal{L})$.
Otherwise (referred to as {\it Case 2}), the node $\sigma^N(\mathcal{L})$ remains in charge of
the binary search along the walk $\sigma^{N/2}(\mathcal{L})\leadsto \sigma^N(\mathcal{L})$, the ``right half" of the walk $\mathcal{L} \leadsto \sigma^N(\mathcal{L})$
% , by first contacting $\sigma^{3N/4}(l)$.
% repeating the same query along the walk $\sigma^{3N/4}(\mathcal{L}) \leadsto \sigma^{N}(\mathcal{L})$.
It is clear that after at most $\log_2 N$ recursive
search steps, the exact location of the target (\ie the last repetition of $\mathcal{L}$)
%  --
% % the length of the cycle
% the length of the walk $\sigma^{-(N \bmod l)}\bigParenthes{\sigma^{N}(\mathcal{L})} \leadsto \sigma^{N}(\mathcal{L})$ (\ie $N \bmod l$)
% --
will be learned. Therefore, we can obtain the result of the green-red weight
comparison, of course with simple augmentation which we will describe later.
\end{comment} %% 02-18-2017

% \begin{algorithm}[t]
% \caption{Binary search at input port $i$ after $i$ receiving the baton.}
% \label{alg: serenade-bsearch}
% \SetKwRepeat{Do}{do}{while}
% \SetKwProg{Proc}{Procedure}{}{}

% % \tcc{After ($i$) receiving the baton }

% If $i$ is $\mathcal{L}$ (\ie the leader of the cycle) then exit
% \label{code: exit-check}

% Update depth of the search: $d \leftarrow d + 1$
% \label{code: depth-update}

% \eIf{The leader in $\sigma^{(-N/2^d)}(i) \leadsto i$ is $\mathcal{L}$} {\label{code: walk-leader-check}

%     \eIf{$\sigma^{(-N/2^d)}(i)$ is $\mathcal{L}$} {\label{code: endpoint-check}

%         Pass the baton to $\sigma^{(-N/2^d)}(i)$
%         \label{code: final-passing}

%     }
%     {

%        Pass the baton to \hlc{red}{SELF}{$\mathcal{s}$ curlycue font of $s$ does not work}
%        \label{code: dummy-passing}

%     }
% }
% {

%         Pass the baton to $\sigma^{(-N/2^d)}(i)$
%         \label{code: intermediate-passing}

% }

% \end{algorithm}

% \begin{algorithm}[t]
% \caption{Binary search at input port $i$ after $i$ receiving the baton.}
% \label{alg: serenade-bsearch}
% \SetKwRepeat{Do}{do}{while}
% \SetKwProg{Proc}{Procedure}{}{}

% % \tcc{After ($i$) receiving the baton }

% \tcc{Stop check}

% \uIf{I am the Leader}{\label{code: ifcond}

%     {\bf stop}\label{code: ifstate}

% }

% \tcc{Query}

% \Do{Leader $\mathcal{L} \in \sigma^{(-N/2^d)}(i) \leadsto i$}{\label{code: whilecond}

%     \tcc{remaining holding the baton}
%     $d \leftarrow d + 1$\label{code: depth-update}

% }

% \tcc{Update weight}
% Update weights $w_{*} \leftarrow w_{*} - w_{*}\bigParenthes{\sigma^{(-N/2^{d})}(i) \leadsto i}$, where $w_{*}$ means $w_r$ and $w_g$\label{code: weight-update}

% \tcc{Passing baton}
% Passing the baton along with the ``current'' depth $d$ and weight $w_{*}$ to $\sigma^{(-N/2^{d})}(i)$\label{code: passing-baton}
% % \tcc{Update weights}
% % \uIf{$\mathcal{M}$ is from ``downstream'' relative to $i$}{
% %   $w_r \leftarrow w_r - w_r\bigParenthes{i \leadsto \sigma^\ell(i)}$
% % }\uElse{
% %   $w_r \leftarrow w_r + w_r\bigParenthes{\sigma^{-\ell}(i) \leadsto i}$
% % }

% % \tcc{Stop check}
% % \uIf{I am the leader}{
% %     {\bf stop}
% % }

% % \tcc{Continue searching}
% % \uIf{$(k_0-1)^{th}$ candidate leader is leader}{

% % Send to $\sigma^{(-\ell/2)}(i)$ message $\mathcal{M}=\{\ell / 2, w_r\}$

% % }
% % \uElse {
% %         Send to $\sigma^{(\ell/2)}(i)$ message $\mathcal{M}=\{\ell/2, w_r\}$
% % }

% \end{algorithm}

%% comment out: 02-18-2017
\begin{comment}
\autoref{alg: serenade-bsearch} captures a ``recursive" step of this binary
search process. It starts with a vertex (input port) $i$ being passed the
baton along with other important information such as the depth $d$ of the
search.
The depth determines the length of the search interval: a depth of value $d$
corresponds to a search interval of length $N/2^d$. Like in the initial
search step (\ie when $d = 0$) described above,
the vertex $i$
% first increases the search depth $d$ to $d + 1$ (see \autoref{code: depth-update}).
% Then, it
% asks $x \ominus N/2^{d+1}$
queries
whether the middle vertex of the
% interval $[x \ominus 3N/2^{d+2}, x \ominus N/2^{d+1}]$ is $l$ (line ?).
walk $\sigma^{(-N/2^{d})}(i)\leadsto i$, \ie $\sigma^{(-N/2^{d + 1})}(i)
\in \phi^{(i)}_{(\log_2 N - d - 1)-}$,
is $\mathcal{L}$ (see \autoref{code: endpoint-check}). Clearly, this query can be done in $O(1)$ by checking
the identity information in the knowledge set $\phi^{(i)}_{(\log N - d - 1)-}$.
If the answer is yes, then the target is found, the baton along with other important messages
(\eg search depth $d + 1$) is passed on to $\sigma^{(-N/2^{d + 1})}(i)$ to
finish the binary search (see \autoref{code: final-passing}).
Otherwise, node $i$ queries whether the leader of the
% interval $[x \ominus 3N/2^{d+2}, x \ominus N/2^{d+1}]$ is $l$ (line ?).
walk $\sigma^{(-N/2^{d + 1})}(i)\leadsto i$ -- the ``right half'' of
the walk $\sigma^{(-N/2^{d})}(i)\leadsto i$ --
is $\mathcal{L}$
(see \autoref{code: walk-leader-check}). This can be done by checking
the leadership information in the knowledge set $\psi^{(i)}_{(\log N - d - 1)}$?.
If the answer is no, the baton along with other important messages
(\eg search depth $d + 1$) is passed on to $\sigma^{(-N/2^{d + 1})}(i)$ (see \autoref{code: intermediate-passing}).
Otherwise, the node $i$
% checks whether $\sigma^{(-N/2^d)}(i)$ is $\mathcal{L}$ (see \autoref{code: endpoint-check}). Again, this can be
% done by checking the identity information in the knowledge set $\psi^{(i)}_{(\log N - d)}$. If yes, it passes the baton to the leader, \ie $\sigma^{(-N/2^d)}(i)$ (see \autoref{code: final-passing}),
% otherwise,
% the node $i$
should continue to administer the binary search
process as explained earlier.
% Note that,
% in the pseudocode, for ease of presentation, we use
% \autoref{code: dummy-passing}, \ie passing the baton to SELF. However,
% in real implementation, this is not required. The node $i$ can
% directly come to the next step of binary search, but without
% executing \autoref{code: exit-check}.
% However, to make the pseudocode succinct, we let $x$ pass on the baton ``recursively" to itself (line ?)
% with depth increased by 1 (to $d+1$).
Note that whenever the node $\mathcal{L}$ is passed on the baton, the search
process terminates (\autoref{code: exit-check}), and $\mathcal{L}$ will learn whether the green weight, or
the red weight of the cycle, is heavier with certain augmentation (detailed below).

Note that
% learning the length of the cycle is not the ultimate goal:
searching for the exact location of the repetition of $\mathcal{L}$ along
the walk $\SWalk{\sleader}{N}$ is not the ultimate goal:
The result of the green-red weight comparison of the cycle is. To achieve this ultimate goal,
we can augment this binary search process by asking each node that was handed the ``baton" at some point of time to perform the following ``housing-keeping" computations:  compute and record the ``current"
green and red weights, \ie those of the walk from $\mathcal{L}$ to this node.
More specifically, besides the identity $i$ and search depth $d$ shown in
\autoref{alg: serenade-bsearch}, node (\ie input port) $i$ will also be
passed the green weight and red weight along the walk from the leader
$\sleader$ to $i$ (self). And before passing the baton to
$\sigma^{(-N/2^{d+1})}(i)$ (\ie \autoref{code: intermediate-passing} and \autoref{code: final-passing}), it first updates the red weight as follows:
$w_r\leftarrow w_r - w_r\bigParenthes{\EWalk{N/2^{d+1}}{i}}$ (note
$w_r\bigParenthes{\EWalk{N/2^{d+1}}{i}} \in \phi^{(i)}_{(\log_2 N - d - 1)-})$.
Green weight is updated similarly. Besides the search depth $d + 1$, the
updated weight information is also passed with the baton. Note that,
at the initial step, node $\sigma^N(\mathcal{L})$
knows the green weight and red weight of the walk from the leader
$\mathcal{L}$ to it (\ie $w_g(\SWalk{\sleader}{N})$ and $w_r(\SWalk{\sleader}{N})$), because $w_g(\SWalk{\sleader}{N})$ and $w_r(\SWalk{\sleader}{N})$ are parts of its knowledge set $\phi^{\sigma^N(\sleader)}_{\log_2 N -}$.
 %
% For example, as shown in \autoref{fig: bs}, if the baton is passed on to $\sigma^{3N/4}(\mathcal{L})$ (say
% in the {\it Case 2} in the above example, the query along the walk $\sigma^{3N/4}(\mathcal{L})\leadsto \mathcal{L}$ answers no),
% the node $\sigma^{N}(\mathcal{L})$ computes the ``current" red weight $w_r(\mathcal{L} \leadsto \sigma^{3N/4}(\mathcal{L}))$, according to the ``previous" red weight $w_r(\mathcal{L} \leadsto \sigma^N(\mathcal{L}))$ -- ``passed'' to it from the node
% $\sigma^N(\mathcal{L}))$ --
% and the ``depth" of the current search step ($=2$ in this case), which determines the red weight to be subtracted (from the ``previous" red weight) in the amount of $w_r(\sigma^{3N/4}(\mathcal{L}) \leadsto \sigma^N(\mathcal{L}))$.
This
``housekeeping" computation of the red and green weight can be easily carried out by augmenting \autoref{alg: serenade-bsearch}.
% ; that of the green weight is carried out in line ?.
Through this simple augmented
% data structure and
algorithm
% ~\cite{Cormen2001IntroAlg}
, the leader $\mathcal{L}$ will find out the red and green weights of (certain multiples of) the cycle when the binary search process terminates.
\end{comment}





% [possibly move to an earlier section]
% Whereas O-SERENADE makes a decision based on these two knowledge sets,
% E-SERENADE goes on to learn the exact length of the cycle and the precise result of the green-red weight comparison.

%As we explain earlier, E-SERENADE needs to run O-SERENADEbuilds upon.


%i.e., the shared initial part
%for all three SERENADE variants).
%Like with other SERENADE steps,

\begin{comment}
% Move to appendix
\subsection{Parallelized Population}
\label{subsec: parallel-population}

In the previous parts of this section (\ie \autoref{sec: serenade-algorithms}),
we have demonstrated the parallelized {\it MERGE} operator. However, as mentioned
that we need to populate the partial matching to the full matching.

SERENADE parallelizes the population procedure, \ie the round-robin pairing operation so that the computational complexity
for each input port becomes only $O(\log N)$ and that for the switch controller is in theory still $O(N)$, but in practice
around $O(\log N)$ for $N$ that is not too large (say $N\le 1024$) as follows. In SERENADE, each unmatched input or
output sends a pairing request ($1$-bit) to the switch controller.  The controller creates two $N$-bit bitmaps,
one indicating which input ports are unmatched and the other indicating which output ports are unmatched,
and broadcasts both bitmaps to all input ports. Note this (broadcast) communication cost of $2N$ bits is very reasonable,
considering that the switch controller in iSLIP needs to receive a total of  $N^2$ bits, one for each VOQ indicating whether or not it is empty,
from the $N$ input ports.
Each unmatched input port $i$ independently needs to figure out, by scanning the IN bitmap, its rank-order (say $j$) among the unmatched input ports.
The input port $i$ then needs to scan the OUT bitmap for the output port that has rank-order $j$.

Although each scanning step still has complexity $O(N)$, it is not hard to show that,
using a $64$-bit CPU equipped with the POPCNT instruction~\cite{popcnt2016}, which counts, in one CPU cycle~\cite{popcntthroughput2016}, the
number of bits that take value $1$ in a $64$-bit word, each step can be carried out in roughly $\frac{N}{64}$ CPU cycles.  For $N$ that is not too large,
this complexity is comparable to $O(\log N)$.  Furthermore, we can make the asymptotic complexity of this step
strictly bounded at $O(\log N)$ by having the switch controller, conceivably equipped with a faster processor,
perform these POPCNT computations for, and broadcast the precomputed POPCNT values to, all input ports.
%%
After receiving the two bitmaps and the POPCNT values of each $64$-bit word in the bitmaps,
each unmatched input port first finds the $64$-bit word where itself locates, getting
its rank $r$ in the word through a binary search, \ie it is the $r^{th}$ ``1'' in the word


\end{comment}
% ====

% -Note that in a switch it is possible for an input port to send a packet to another input port.  This is because, in an actual switch, each line card is attached
% to both an input port and an output port.  So an input port $i$ can send a message to the output port $j$, asking it to pass it on to the input port $j$.
% We did not assume this co-location in defining earlier the load matrices used to simulate the
% performance of QPS, which have large diagonal components
% (amount of traffic from input port $i$ to output port $i$ for $i = 1, 2, \cdots, N$) that would make no sense under this co-location assumption;

% ====

% -leader election \cite{awerbuch1987leaderelection}


% -Note that $k_1$ could be equal to $k_2$, which happens when this edge ( , ) belongs to both matchings.  For example, in Figure ?, there is a self-loop (move up).

% -In this iteration, each input port and each output port sends out a message during this iteration.

% Suppose after the $k^{th}$ iteration, each node knows ?, ?, and ?.  The $(k+1)_{st}$ iteration works as follows.
% Each vertex $i$ sends to $ ??? $ the identity of the vertex.  Hence this vertex $i$ will receive, from ..., ??? and ???.
% It can then compute $ ??? := ??? + ???$.  Then it can send ??? a message informing it of ... and ...
% Note that $i$ will receive such a message from ???, so that it knows ... upstream and ... downstream.  THis completes the
% ``inductive" description of this algorithm

% Finally, we note that we can further reduce the length of each message, by encoding, instead of ? and ?, their difference ?,
% since the decision rules in both C-SERENAde and O-SERENAde involve only their difference.  In a high-speed switch where
% each time slot is tens or hundreds of nanoseconds, every bit of overhead counts.

% This distributed algorithm is a standard ``distance doubling" technique \cite{} in distributed computing.  We are however
% the first to realize that such a technique can be used to approximately or exactly emulate the Merge operation of SERENA.

% Now we can explain how to augment this distributed algorithm to achieve the aforementioned leader election.
% In the two messages sent in the (k+1)th round, we add the information regarding the smallest vertex (input port)
% index within along the walk ...  It is not hard to verify this information can be obtained ``inductively" (recursively) like the
% $2^k$-upstream/downstream information set.
% THe only cost of this leader election, on top of the cost of this distributed algorithm, is the $log_2 N$ additional bits to encode
% this (smallest vertex) index in each message.


% The problem of distributed leader election \cite{awerbuch1987leaderelection} is classical and we adopt a simple solution here. In a cycle, the input vertex with the minimum {\it ID} is regarded as the leader. And all vertexes obtain the unique leader information after $\log N$ iterations. To be specific, every vertex $v$ adds a new field $L_k(v)$ to record the leader {\it ID} it learns in the $k^{th}$ iteration, and initially $L_0(v) = v$ ($\forall v$). In the $k^{th}$ iteration, every vertex completes two jobs described in the conservative algorithm, and updates the leader as follows, $L_k(v) = \min\big{\{}L_k(v), L_k\big{(}P_{k-1}(v)\big{)}\big{\}}$.

% In E-SERENAde, this augmented (with leader election) distributed algorithm is further extended to emulate SERENA exactly as follows.

% %After ... iterations,
% %every node $i$ knows the indices of the ``leaders" within the walks ..., ...., ..., and ... respectively.    can compute the exact
% %green and red weights of the

% Armed with this ``leadership information", all vertices on a non-ouroboros cycle can collaboratively perform,
% through up to $2 + \log_2 N$ additional iterations, ``Chord-like" \cite{} binary searches over
% the sets of ``leadership information" these vertices collectively have, to compute the green and the green weights of the cycle exactly;
% we omit the details of this algorithm in the interest of space.
% Our simulations show that on average, an additional $0.6 \log_2 N$ iterations are needed, bringing the total number of iterations to $1.6 \log_2 N$.
% Hence in a sense, E-SERENAde is 1.6 times slower than C-SERENAde and O-SERENAde.  Since both O-SERENAde and C-SERENAde perform only slightly
% worse than SERENA, they are clearly better solutions than E-SERENAde in practice.  However, E-SERENAde makes an important point that
% the Merge operation of SERENA can be exactly emulated in $O(\log_2 N)$ iterations.


% We propose to study three research problems that arise in my preliminary investigations into the SERENAde algorithms.


% The first problem we would like to investigate is whether O-SERENAde is stable (i.e., can achieve 100\% throughput) under all admissible workloads.
% Although our simulation results show that it empirically achieves 100\% throughput under all four load matrices when $N = 32, 64, 128$,
% this is not a proof.  In particular, these simulation results
% cannot rule out the possibility that O-SERENAde cannot achieve 100\% throughput when $N$ becomes
% much larger, and/or when it operates under certain pathological load matrices.
% There is indeed another strong evidence that O-SERENAde
% is stable under all admissible workloads:
% %can achieve 100\% throughput under all load matrices.
% As shown earlier, a simple
% O-SERENAde variant has much better delay performance than C-SERENAde, and C-SERENAde is provably stable due to it being C-degenerative.

% Proving the stability of O-SERENAde appears to be hard.  For one thing, Theorem ? above, including its strongest
% extension we are aware of at this moment, cannot be applied to O-SERENAde because it is not C-degenerative.  In fact, it can be shown that
% O-SERENAde could decide on a sub-matching (say the green one) in a non-ouroboros cycle that is lighter than the red sub-matching by up
% to a constant fraction of the weight of the red sub-matching.  Even though this situation happens arguably with a tiny probability,
% so far we are not able to estimate or bound this probability, which could be an important step in this proof.

% In fact, we can let this stability issue go away by imposing the following ``bounded support" condition on O-SERENAde:
% O-SERENAde is used on a non-ouroboros cycle if the red or green weight of every edge is upper-bounded by a large constant $\mu$,
% and C-SERENAde is used otherwise.  O-SERENAde with this ``bounded support" is provably stable because it is C-degenerative.
% Furthermore, in practice, this threshold $\mu$ can be made so large that it will not be reached with high probability, in which case
% O-SERENAde with ``bounded support" should have almost the same delay performance as that without.  However, we believe
% proving the stability of the original O-SERENAde has significant theoretical importance.  For example, it may lead us to new stability
% proof techniques that can be used to solve other hard stability analysis problems.

% The second problem we would like to investigate is to explore the full design space of O-SERENAde.   As explained earlier, each vertex
% $i$ on a non-ouroboros cycle knows $2 \log_2 N + 2$ different ``weights":  $w_g()$ and $w_r()$, for ? = ...
% However, the simple variant we described earlier uses only two weights:
% ... and ...  We plan to study whether there are better decision rules that, by making good use of also other weights, deliver a better tradeoff
% between delay performance and the computational complexity of the decision rule.  Readers may understandably question whether
% this pursuit is necessary because as we have shown earlier, the delay performance of this simple
% O-SERENAde variant is very close to SERENA already, under the four aforementioned load matrices
% when $N = 32$.  We note, however, that it is not known, whether this will continue to be the case
% under other load matrices, and/or when $N$ becomes much larger, so it is important to explore
% this design space fully.

% The third problem we would like to study is the cycle decomposition analysis.

% % to identify one or more robust variants that deliver

% % and/or when this O-SERENAde variant operates , whether this delay performance can continue to be close to SERENA's.


% %uses more information than just

% %(comparing $w_g(i\leadsto \sigma^{N}(i))$)

% %It is important to prove this stability result for the following reason.


% However, again this is not a proof.

% appears to  a more attractive scheduling algorithm
% than

% and C-SERENAde


% creating a negative drift


% so wrong that the weight of the new matching
% can be smaller than the old matching by


% Proving this result is


% The evidence is mounting

% without a proof, we cannot say definitively

% this is not a proof.




% %, or achieves only around 62.5\% of the throughput that


% ``remainder arc"

% each vertex $i$ learns the identities of the leaders in the walks ..., ...., ...  respectively.  Through up to $2 + \log_2 N$ additional iterations, this vertex
% $i$

% performs

% on a non-ouroboros cycle knows the leader

% {\bf A $O(\log N)$ Parallel Exact-Merge Algorithm.}
% %The above two algorithms could only approximate the merge operation. Now in this algorithm, we aim at figuring out the exact weight of a cycle in the cases where its length is not nice (\emph{i.e.,} $2^m$ or divisors of $2^m \pm 2^n$).
% The above two algorithms complete the merge operation by approximating the total weight of a cycle, $\psi$. In this algorithm, we figure out the length of the cycle $\psi$ exactly when it is not equal to $2^m$ or one divisor of $2^{m_1} \pm 2^{m_2}$.


% The underlying idea is indeed very natural, binary search.
% First, we assume there exists a vertex $v$ such that any other vertex
% can determine the relative position (using the leader as reference) and the leader knows the total
% weights from $v$ to the leader. We will show the existence of such a vertex later. Based on the assumption,
% we only need to get the total weight of the path from the leader to $v$.
% Since every other vertex knows the relative position, it is clear that
% we can use a binary search to get such weights.
% Now we will show the existence of such a vertex. Define $L$ be the leader,
% and $v_0$ be the vertex such that $v_0 \rightarrow L$ is an edge of the cycle.
% Let $m_0 = \min\{m \geq 0: L_m(v_0) = L\}$.
% We claim that $v_1 = P^{-1}_{m_0-1}(v_0)$, \emph{i.e.,} $P_{m_0-1}(v_1) = v_0$ is such a vertex.
% First, the leader can learn the total weights of the path from $v_1$ to $L$. Second, for any vertex $v$ between $v_1$ and $v_0$ including
% $v_0$, we have $L_{m_0-1}(v) > L$, \emph{i.e.,} it does not learn the
% true leader yet. And the rest vertexes (not including $v_1$) have
% already learned the true leader. Therefore, by checking whether the
% vertex has learned the true leader or not until the $m_0-1$ iteration,
% any vertex can determine the relative position.
% Hence, by using extra $2 + \log N$ iterations ($2$ for learning the weight of the path from $v_1$ to $L$,
% $\log N$ for learning that from $L$ to $v_1$), the leader $L$ can learn the
% exact total weight of the cycle.





% Each input port sends out 2 messages are sent


% For example, in Figure ?(a), output port 5 will send a message
% ...



% %tentatively to be matched with

% It means in the last time slot, output port $\pi_2(i)$ received the packet from input port $\pi^{-1}(i)$. After Step 1, each input port $i$ obtains $\pi(i),q_{\pi(i)}^{(2)}$. And combining the VOQ length $q_{i}^{(1)}$, input port $i$ can compute $D_{i}(0)$ based on~\ref{firstterm}, then send $i$ and $D_{i}(0)$ to input port $\pi(i)$. Afterwards, each input port $i$ obtains $\pi^{-1}(i)$ and $D_{i}(-1)$. So far, each input port $i$ has $\pi^1(i)$, $\pi^{-1}(i)$, $D_{i}(0)$ and $D_{i}(-1)$.

% The rest of preparation process is to recursively get $\pi^{2^k}(i)$, $\pi^{-2^k}(i)$, $D_{i}(2^k-1)$ and $D_{i}(-2^k)$ for $k=1,\cdots,\left\lceil\log N\right\rceil$. Specifically, assuming we have $\pi^{2^{k-1}}(i)$, $\pi^{-2^{k-1}}(i)$, $D_{i}(2^{k-1}-1)$ and $D_{i}(-2^{k-1})$ after the the $(k-1)$th round. Then in the $k$th round, we first let each input port $i$ send $\pi^{-2^{k-1}}(i),D_{i}(-2^{k-1})$ to input port $\pi^{2^{k-1}}(i)$. Each input port $i$ get $\pi^{-2^{k-1}}\big{(}\pi^{-2^{k-1}}(i)\big{)}=\pi^{-2^k}(i)$ and $D_{\pi^{-2^{k-1}}(i)}(-2^{k-1})$ afterwards. Secondly, combining $D_{i}(-2^{k-1})$, each input port $i$ computes $D_{i}(-2^{k})$ based on~\ref{recursion}, and send $i$ and $D_{i}(-2^{k})$ back to input port $\pi^{-2^k}(i)$. After that, each input port $i$ has $\pi^{2^k}(i)$, $\pi^{-2^k}(i)$, $D_{i}(2^k-1)$ and $D_{i}(-2^k)$. Note that the total number of transmission of Algorithm~\ref{firststep} is $2\left\lceil\log N\right\rceil+3$.



==> sections/serenade-algorithms/serenade_discussion.tex <==
\subsection{Discussion: Why Three Variants}
\label{subsec: why-three-variants}

\addedHL{In this work, we present three variants of SERENADE instead of just one (say E-SERENADE) mainly for two reasons.
First, C-SERENADE and O-SERENADE have to be included, since they represent two 
extremes (conservative vs. opportunistic) in the design space, and neither is strictly better in all aspects.  
%C-SERENADE is lower in both time and message complexities, but O-SERENADE
%has better delay performance, as we will show in ...
Second, E-SERENADE has to be included, because
it is by no means obvious that SERENA can be exactly emulated through only $O(\log N)$ distributed iterations,
and because it provably stabilizes both C-SERENADE and O-SERENADE, as we will elaborate next.  Overall, among the three SERENADE variants, 
O-SERENADE achieves the best tradeoff between delay performance and (time and message) complexities, as our evaluation results in~\autoref{sec:evaluation} will show.} 
